RTL Verification for Secure Speculation Using Contract Shadow Logic

Modern out-of-order processors face speculative execution attacks. Despite various proposed software and hardware mitigations to prevent such attacks, new attacks keep arising from unknown vulnerabilities. Thus, a formal and rigorous evaluation of the ability of hardware designs to deal with speculative execution attacks is urgently desired. This paper proposes a formal verification technique called Contract Shadow Logic that can considerably improve RTL verification scalability while being applicable to different defense mechanisms. In this technique, we leverage computer architecture design insights to improve verification performance for checking security properties formulated as software-hardware contracts for secure speculation. Our verification scheme is accessible to computer architects and requires minimal formal-method expertise. We evaluate our technique on multiple RTL designs, including three out-of-order processors. The experimental results demonstrate that our technique exhibits a significant advantage in finding attacks on insecure designs and deriving complete proofs on secure designs, when compared to the baseline and two state-of-the-art verification schemes, LEAVE and UPEC.

==> Artifact.tex <==
\section{Artifact Appendix}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Abstract}

Our artifact is the infrastructure for verifying the two software-hardware contracts on four processors listed in \cref{tab:eval:setup}.
It includes the baseline verification scheme using four copies of processors and our verification scheme using contract shadow logic.
This artifact can be used to reproduce the verification results, including the time it takes and the attacks it finds, shown in \cref{tab:eval:all}, \cref{tab:eval:compare-defense}, and \cref{fig:eval:size-time}.

\subsection{Artifact check-list (meta-information)}

{\small
\begin{itemize}
  \item {\bf Run-time environment: } JasperGold and Dask.
  \item {\bf Hardware: } A >16-core machine with 4GB memory per core.
  \item {\bf Output: } Terminal outputs and a figure. Example results are included.
  \item {\bf Experiments: } Running the provided scripts will reproduce the results. Results will vary due to the performance of the machine and the randomness in JasperGold's solving engines.
  \item {\bf How much disk space required (approximately)?: } 1GB.
  \item {\bf How much time is needed to prepare workflow (approximately)?: } 20 minutes.
  \item {\bf How much time is needed to complete experiments (approximately)?: } On a >16-core machine, it takes $\sim$3 hours to complete most ($\sim$42 out of 54) experiments and 7 days to complete all experiments.
  \item {\bf Publicly available?: } Yes.
  \item {\bf Code licenses (if publicly available)?: } MIT license.
  \item {\bf Archived (provide DOI)?: } To Be Assigned.
\end{itemize}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Description}

\subsubsection{How to access}

\url{https://github.com/qinhant/ShadowLogicArtifact}.

\subsubsection{Hardware dependencies}

The experiments only require CPU and memory resources.
When running the experiment of a specific configuration, it will take $\sim$1.2 cores.
We provide scripts to run experiments of many configurations in parallel and thus recommend a >16-core machine to finish them in a shorter time.
4GB memory per core is recommended to avoid out-of-memory errors.

\subsubsection{Software dependencies}

JasperGold FPV by Cadence~\cite{website:jaspergold} is required to run the experiments.
It is a commercial hardware verification tool that requires a license to use.
Our scripts assume JasperGold can be launched through \texttt{jg} commands from the terminal.
Dask~\cite{Dask} is used to launch multiple experiments in parallel, it can be installed with \texttt{python3 -m pip install "dask[complete]"}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Installation}

Download the artifact folder to the machine and make two copies of it, which will be used to launch two batches of experiments.
No other installation is required.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Experiment workflow}

This artifact is used to reproduce the verification results on various tasks shown in \cref{tab:eval:all}, \cref{tab:eval:compare-defense}, and \cref{fig:eval:size-time}.

For each verification task, the verilog source code is located in the \texttt{src} folder, including four processors (\texttt{Sodor}, \texttt{SimpleOoO}, \texttt{Ridecore}, and \texttt{BOOM}).
Each processor has its corresponding top module to conduct baseline verification scheme and our verification scheme using contract shadow logic under both sandboxing and constant-time contracts.
The JasperGold scripts to launch each verification task are located in the \texttt{verification} folder.

The users of this artifact can use scripts provided in the \texttt{results} folder to launch batches of verification tasks.
When the batches are running, the user can check the results of finished tasks by using the provided scripts to parse the log files and print out a summary of all verification results.
A plotting script is provided to reproduce \cref{fig:eval:size-time}.





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Evaluation and expected results}

\paragraph{Reproduce \cref{tab:eval:all} and \cref{tab:eval:compare-defense}}
In the first copy of the artifact folder, we first initialize a cluster of 12 worker threads with:

\begin{minipage}{\columnwidth}
\begin{lstlisting}[]
(python3 -u scripts/dask/initCluster.py 12 \
         > & initCluster.log &)
\end{lstlisting}
\end{minipage}
Then, launch the batch of verification tasks with:

\begin{minipage}{\columnwidth}
\begin{lstlisting}[]
(python3 -u results/CompareTable/run.py \
         > & run.log &)
\end{lstlisting}
\end{minipage}

When the verification tasks are running, they will produce \texttt{my\_proj\_*} folders as JasperGold's project folder, \texttt{terminal\_*.log} files as JasperGold's terminal output files, and \texttt{my\_jdb\_*} files saving the attacks found.
Users can run the following commands to parse JasperGold's terminal output files and print out a summary of verification results on finished tasks:

\begin{minipage}{\columnwidth}
\begin{lstlisting}[]
python3 results/CompareTable/summary.py
python3 results/CompareTable/print.py
\end{lstlisting}
\end{minipage}
The commands can be repeated as more tasks are finished.

The summary is listed processor-by-processor.
\texttt{results/CompareTable/example.log} is an example of it.
For each processor, there will be three arrays:

\begin{itemize}[leftmargin=*]
\item
The first array is the names of the verification tasks with the following naming convention:
\texttt{sandbox} and \texttt{ct} represents the sandboxing and constant-time contracts.
\texttt{4copy} and \texttt{2copy} represents the baseline verification scheme and our scheme.
For the \texttt{SimpleOoO}, the array includes six versions of the processor, including the insecure version with no defense scheme followed by the five versions with defense augmentation listed in \cref{tab:eval:compare-defense}.

\item
The second array indicates whether the processor under test is secure.
\texttt{1} indicates the processor is secure, \texttt{0} indicates an attack is found, and \texttt{-1} indicates the experiment has not finished.
You could further open JasperGold's GUI to check the attacks found with:

\begin{minipage}{\columnwidth}
\begin{lstlisting}[]
jg -command "restore -jdb my_jdb_{expName}"
\end{lstlisting}
\end{minipage}

\item
The third array includes the time it takes for the verification tasks to finish in the unit of seconds.
\texttt{-1.0} indicates the experiment has not finished.
\end{itemize}

It takes $\sim$3 hours to complete most ($\sim$25 out of 34) tasks and 7 days to complete all experiments.
The summary is used to fill in the information in \cref{tab:eval:all} and \cref{tab:eval:compare-defense}.
Be aware that the results will vary due to the performance of the machine and the randomness in JasperGold's solving engines.




\paragraph{Reproduce \cref{fig:eval:size-time}}
In this batch of experiments, we can share the cluster created for the last batch.
To launch the experiments, move to the second copy of the artifact folder and use similar commands as before:

\begin{minipage}{\columnwidth}
\begin{lstlisting}[language=bash]
(python3 -u results/ScalabilityFigure/run.py \
         > & run.log &)
## Wait ~3 hours to see most results.
python3 results/ScalabilityFigure/summary.py
python3 results/ScalabilityFigure/print.py
## Example print-outs in `example.log`.
\end{lstlisting}
\end{minipage}
The naming convention in the summary further includes \texttt{RF*\_MEMI*\_MEMD*\_ROB*} to indicate the size of register file, data memory, instruction memory, and re-order buffer.
These parameters are scaled up to demonstrate how verification time will increase in \cref{fig:eval:size-time}.

To reproduce the figure, we provide a template script in  \texttt{results/ScalabilityFigure/plot.py}.
The array \texttt{time} in it stores the verification time to be plotted.
The two sub-arrays in it correspond to the sandboxing and constant-time contracts.
Each sub-array contains verification time when varying register, data memory, and re-order buffer sizes among 2, 4, 8, and 16.
Carefully update the array \texttt{time} in it based on the experiment summary (be aware that 3 data points should be omitted because they cannot finished within 7 days in our machine setup) and plot with:

\begin{minipage}{\columnwidth}
\begin{lstlisting}[]
python3 results/ScalabilityFigure/plot.py
\end{lstlisting}
\end{minipage}

Finally, terminate the cluster by finding the \texttt{PID} of the thread and kill it:

\begin{minipage}{\columnwidth}
\begin{lstlisting}[]
ps -ef | grep initCluster.py
kill XXXX
\end{lstlisting}
\end{minipage}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Methodology}

Submission, reviewing and badging methodology:

\begin{itemize}
  \item \url{https://www.acm.org/publications/policies/artifact-review-badging}
  \item \url{http://cTuning.org/ae/submission-20201122.html}
  \item \url{http://cTuning.org/ae/reviewing-20201122.html}
\end{itemize}

==> Formulation.tex <==
\cameraready{

\section{Formulation}
\label{sec:formal}


\subsection{Property to Prove}

Recall we have the following formula in the background section to define contracts:
\[
\begin{aligned}
&\forall P, M_{pub}, M_{sec}, M_{sec}', \\
\text{\textbf{if}}\quad & O_{ISA}(P,M_{pub},M_{sec})=O_{ISA}(P,M_{pub},M_{sec}') \\
\text{\textbf{then}}\quad & O_{\mu Arch}(P, M_{pub},M_{sec}) = O_{\mu Arch}(P, M_{pub},M_{sec}') & 
\end{aligned}
\]
% Be aware that $O_{ISA}$ and $O_{\mu Arch}$ are configurable based on:
% \begin{itemize}
%     \item How $ISA$ and $\mu Arch$ simulate the program.
%     \item How they extract observation.
% \end{itemize}
% We will start to think a little more precisely on the first item, ``how $ISA$ and $\mu Arch$ simulate the program''.
% What is the length of the simulations? (For infinite cycles? Until the program terminates?)
% Should $ISA$ and $\mu Arch$ be simulated for the same number of cycles?
% We will remove these ambiguities in the following definition.

We will add a notion of ``cycle'' to this original version.
First, we use notation $O^n_{ISA}$ and $O^n_{\mu Arch}$ to represent ``simulate $ISA$ (or $\mu Arch$) for $n$ cycles''.
Second, we define a function to relate the number of cycle being simulated in $ISA$ and $\mu Arch$.
The function, $\texttt{F-BTC}_{\mu Arch}(P,M_{pub},M_{sec}, n)$, returns the number of fetched bound-to-commit instructions when simulating the $\mu Arch$ for $n$ cycles.
We will use this returned value as the number of cycles to be simulated in the $ISA$.
With these, the property we will prove with our contract shadow logic is:\yuheng{Just keep nBTC and remove F-BTC. And explain how we decide nBTC with text.}
\[
\begin{aligned}
&\forall P, M_{pub}, M_{sec}, M_{sec}', n, \\
% \text{\textbf{let}}\quad & n_{BTC} = Max(\texttt{F-BTC}_{\mu Arch}(P,M_{pub},M_{sec}, n),
\texttt{F-BTC}_{\mu Arch}(P,M_{pub},M_{sec}', n)) \\
\text{\textbf{if}}\quad & O^{n_{BTC}}_{ISA}(P,M_{pub},M_{sec})=O^{n_{BTC}}_{ISA}(P,M_{pub},M_{sec}') \\
\text{\textbf{then}}\quad & O^n_{\mu Arch}(P, M_{pub},M_{sec}) = O^n_{\mu Arch}(P, M_{pub},M_{sec}') & 
\end{aligned}
\]

% We use notation $O^n_{ISA}$ and $O^n_{\mu Arch}$ to represent ``simulate $ISA$ (or $\mu Arch$) by fetching $n$ bound-to-commit instructions and extract the observation''.
% The ``fetching $n$ bound-to-commit instructions'' is subtly defined to align with our ``instruction inclusion requirement''.
% Its subtlety lies in two aspects:
% \begin{itemize}
%     \item For all fetched instructions, only some of them are bound to commit. Others will be squashed.
%     \item For all fetched bound-to-commit instructions, when the simulation finishes, only some of them have been committed. Others will be in the ROB.
% \end{itemize}
% In short, when the simulation finishes, ``committed instructions'' $\subseteq$ ``fetched bound-to-commit instructions'' $\subseteq$ ``fetched instructions''.
% For $ISA$, these 3 sets are equal.
% For $\mu Arch$, based on the implementation, e.g., ROB size, prediction correctness, the 3 sets can be different.
% For now, we assume a memory system with constant 1-cycle read/write latency (because I am not sure how cache pre-fetch will affect our definition).
% \yuheng{TODO: there is one problem about this formulation that for $\mu Arch$, ``fetching $n$ bound-to-commit instructions'' does not constrain how many cycles it will simulate. Then, $O^n_{\mu Arch}$ can have undetermined cycles...}

Compared with the original formula, when $n$ is bounded, this new one might miss some contract assumption constraints and give an invalid attack program.
We say this attack program is invalid because if we do the assumption constrain for an unbounded number of cycles, it will not pass.
When this new one is proved with unbounded $n$, it is equivalent to the original one.

\subsection{Discuss Possible Invalid Attacks}

It would be useful to discuss the source of an invalid attack program when $n$ is bounded.
We will show this is rare and we did not observe them during our experiments.
There are two reasons why we miss some constraints:
\begin{itemize}
    \item Fetched instructions that will be squashed (i.e., not bound-to-commit).
    \item Instruction being touched by the system (e.g., prefetched by cache) while not fetched into the pipeline. (In our experiments, we assume a memory system with constant 1-cycle read/write latency (because I am not sure how cache pre-fetch will affect our definition).)
\end{itemize}

% \yuheng{Work In Progress. Don't Read.}




\subsection{Contract Shadow Logic Prove the Property with Two Assumptions}

\yuheng{I am still ``describing'' our two assumptions and have not used formulas to represent our two assumptions. But maybe this is enough?}

The key reason that motivates us to design the contract shadow logic is that the $ISA$ observation can be extracted from the $\mu Arch$ model.
This can be formalized as the first assumption we use: \textbf{the $\mu Arch$ model correctly implements the $ISA$.}
There are many facts that can be derived from ``correctly implemented''.
For our convenience, we derive a fact from this assumption that for each bound-to-commit instruction, there exist signals in the $\mu Arch$ model at a certain cycle that give the correct operands (either read from register file or immediate value decoded from instruction), the computed memory address (if it is a load/store instruction), and the computed write back data.
We rely on existing functionality verification to give us this assumption.

Our second assumption is that \textbf{the shadow logic is implemented correctly.}
We will now explain the definition of correctness.
Given the first assumption, we know those signals for each instruction exist at a certain line of code and at a certain cycle.
However, we have to dig into the implementation to extract these signals correctly.
Thus, we define the correctness of shadow logic as ``extract the correct signals for the first $n_{BTC}$ instructions from the $\mu Arch$ model and compare the signals when the secret changes.
To achieve this correctness, designers should locate the correct signals at the correct cycle, and follow our description of achieving the instruction inclusion requirement and synchronization requirement.

}

==> Implementation.tex <==
\section{Implementation Details}
\label{sec:implementation}
In this section, we introduce several details that are not mentioned in the previous section and discuss how to handle superscalar processors using our scheme.
\subsection{Bookkeeping ISA Level Information}
In our advanced verification scheme, the ISA level comparison is only done for instructions at commit stage.
However, it is possible that some ISA level information are discarded immediately after being used and will not be available at commit stage.
For example, multiplication operands needed by the constant-time programming contract may only be available before they enter the multiplier.
Thus, to avoid such cases, we have to extend the ROB to keep all the necessary ISA level information until commit stage.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.3\textwidth]{images/ROB_mul.png}
    \caption{Extended ROB to Keep \texttt{mul} Information}
    \label{fig:ROB_mul}
\end{figure}

As shown in Figure~\ref{fig:ROB_mul}, we add two columns to the ROB of each out-of-order processor.
One column tells whether an instruction is a \texttt{mul} instruction and the other colums records the two operands of multiplication.
When an \texttt{mul} instruction enters ROB, the $is\_mul$ column gets a corresponding value, and when an \texttt{mul} instruction enters the multiplier, its two operands are stored into the $mul\_opr$ column in ROB.
In the figure, $inst_1$ is not a multiplication instruction, and thus synchronized comparison will not compare the $mul\_opr$ for $inst_1$ in two out-of-order processors.
Because $inst_2$ is a multiplication instruction, the $mul\_opr$ of $inst_2$ will be compared in the synchronized comparison.


\subsection{Finishing Logic Optimization}
As we introduced earlier, the finishing module will store all the inflight instructions of two out-of-order processors when a microarchitectural deviation is observed.
Intuitively, we can store all the ROB indices of all inflight instructions and wait for all of them to be committed and compared.
To further reduce the overhead, we only store the index of the youngest instruction in the ROB.
Then, if the ROB commits an instruction with this index, we know that it is time to finish the checking.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{images/sqaush.png}
    \caption{Update the Youngest Instruction After Squashing}
    \label{fig:squash}
\end{figure}

However, if this youngest instruction gets squashed and not committed, we have to update the stored index to the youngest instruction that is not squashed.
For example, in Figure~\ref{fig:squash}, assume that at the beginning a deviation of microarchitectural information is observed the and the finishing module recorded the index of the youngest instruction in the ROB, which is $inst_5$.
After a squashing happens and $inst_4, inst_5$ are squashed, the youngest instruction becomes $inst_3$, then we need to update the stored index to $inst_3$ at this time.
After the update, the finishing logic only need to wait for $inst_3$ to be committed.

Besides, the two out-of-order processors may have different youngest instructions in the ROB when the microarchitectural deviation is observed.
For example, the first processor may issue some instruction a few cycles earlier than the second processor due to the secret value.
If a microarchitectural deviation is observed during this time window, the two processors will have different youngest instructions.
However, this youngest instruction in the first processor still needs to be compared because it may have already affected the microarchitectural observation in the first processor.
Thus, the finishing logic will record indices of both youngest instructions in two out-of-processors.
Only when both youngest instructions are committed and compared can the finishing logic set the $finish$ bit.




\subsection{Handle Superscalar Processors}
In Section~\ref{sec:methodology}, we assume a processor that issues and commits at most one instruction in a cycle.
However, modern superscalar processors may have multiple functional units and thus are able to issue and commit multiple instructions in a cycle.
We will discuss how our baseline scheme and the advanced scheme are both able to handle such cases.

First, we assume that the out-of-order processor can issue two instructions but only commits one instruction at a cycle.
In this scenario, the advanced scheme can still work because no matter how many instructions are issued, the finishing logic will guarantee that all inflight instructions will be compared at commit stage after observing a microarchitectural deviation.
However, the original baseline scheme may fail because the single-cycle machine may not be able to execute instructions as fast as the out-of-order processor, which means when a microarchitectural deviation is observed, the ISA level comparison may have not finished for all inflight instructions in the out-of-order processors.
The solution is to add a finishing logic to the baseline scheme.
Two counters will be added to record the numbers of instructions issued in the two out-of-order processors.
When observing a microarchitectural deviation, the larger counter will be compared with the number of cycles that have elapsed (this represents the number of instructions executed and compared in two single-cycle machines).
If the counter number is larger, then the ISA level comparison needs to continue for extra cycles to reach the counter number.
Meanwhile, the microarchitectural level comparison will be stopped.
After that, a $finish$ bit will be set and the model checking can be finished.

Next, let us consider an out-of-order processor that can issue and commits two instructions in a cycle.
In this case, we can modify the baseline scheme in the same way as above because as long as the ISA level comparison covers all instructions issued in the out-of-order processors, the baseline scheme is correct.
However, the original advanced scheme will fail because the synchronization logic assumes that at most one instruction is committed in both processors.
When the out-of-order processor is able to commit two instructions in a cycle, all the following cases need to be considered:
\begin{enumerate}
    \item Both processors commit two instructions at this cycle.
    \item Both processors commit one instructions at this cycle.
    \item Both processors commit zero instructions at this cycle.
    \item One processor commits two instruction but the other commits one instruction at this cycle.
    \item One processor commits two instructions but the other commits zero instruction at this cycle.
    \item One processor commits one instruction but the other commits zero instruction at this cycle.
\end{enumerate}
Among all these six cases, only 2) 3) 6) are considered in the original synchronization logic.
Thus, the synchronization module needs to be modified to cover all the possible cases, set pause signals when two out-of-order processors commit different numbers of instructions in some cycle, and record the instruction information for later comparison.
All the modifications will be based on existing mechanisms and they only increase the complexity of the shadow logic to cover more cases.

The above two examples have shown that our two schemes can be extended to superscala processors.
For processors that can issue and commit more than two instructions, the way to modify our schemes is similar to the case of two instructions and is not discussed in this paper.


==> Insights_old.tex <==

\section{Threat Model}

% \mengjia{I did minor text tweak}

Recall from \cref{sec:background:contract}, security properties for secure speculation can be formulated as software-hardware contracts.
Such contracts explicitly state the responsibilities of the software and the hardware sides to achieve an overall non-interference property~\cite{clarkson2010hyperproperties}.
In this paper, we consider the following threat model.


% Recall from \cref{sec:background:contract}, informally, security properties for secure speculation are software-hardware contracts.
% \mengjia{you said contract is formal in the previous paragraph, then you say it is informal here?}
% Such contracts explicitly state the responsibilities of both the software and the hardware sides to achieve an overall non-interference property~\cite{clarkson2010hyperproperties}. 
% The following threat model is considered by software-hardware contracts:
\begin{enumerate}[leftmargin=*]
    \item We assume a system whose data memory is split into two parts: \emph{public} and \emph{secret}. 
    An attacker cannot directly access the secret region.
    % The attacker cannot directly access the secret region.
    The attacker's goal is to infer any secret value through microarchitectural side-channel attacks.
    Non-digital side-channel attacks, such as power side channels~\cite{hertzbleed, poweranalysisattacks}, are out of the scope.
    
    \item The system runs a program that satisfies certain software constraints.
    These constraints prevent the secret from being leaked via ISA state.
    For example, at the ISA level, the program cannot load secret data into registers (in the sandboxing contract), or it needs to follow the constant-time programming discipline.
    % at observation constraints that protect the secret, i.e., the instruction-level observation of certain architectural variables (specified in a contract), such as the \texttt{rd} value of committed instructions, cannot leak any secret.
    % The attacker is able to run any programs satisfying such constraints. \mengjia{attack's constraint is discussed in item 2}

    \item The attacker is able to gain cycle-level observation of certain micro-architectural variables (specified in a contract) in the system, such as the address sequence transmitted on the memory bus and the commit time of instructions.
    
    % \item The program run on the system must satisfy certain software  observation constraints that protect the secret, i.e., the instruction-level observation of certain architectural variables (specified in a contract), such as the \texttt{rd} value of committed instructions, cannot leak any secret.
    % The attacker is able to run any programs satisfying such constraints.
\end{enumerate}


\section{Motivation and Insights}
\label{sec:insight}

% We propose \name to improve RTL verification for speculative execution vulnerabilities.
In this section, we describe the insights that motivate the design of our verification scheme, \name.
% We start by formally introducing \textbf{security properties}: a family of software-hardware contracts for secure speculation.
{
We start by presenting the threat model considered in this paper.
We then introduce the formal definition of the security properties that we aim to verify, i.e., a family of software-hardware contracts for secure speculation. 
% \mengjia{I did some inline editing}
}
We then present a baseline verification scheme for the security properties and analyze the performance bottlenecks encountered when using this baseline verification scheme.
Finally, we point out the optimization insight that leads us to the design of \name.
% at the end of this section.

% \mengjia{My plan for this section is to 1) explain the sw-hw contract checking procedure; 2) analyze its performance bottleneck; 3) point out an opportunity for optimization}


% \thomas{Should we mention what is not in the threat model? (sometimes people like that as it scopes the work). Here it would be what sometimes people call "no active attackers" (even though it is confusing as the kind of passive attacker we describe, in practice are "active" to make their observation). This might be too confusing}
% \qt{We can say something like 'no analog attack considered.'}
% \mengjia{yes, let's add 1-2 sentences to exclude analog attacks}
% Next, we will formally define the security property that accounts for the above threat model.


\subsection{Checking Software-Hardware Contracts}

% Recall from \cref{sec:background:contract}, informally, security properties for secure speculation are software-hardware contracts.
% Such contracts explicitly state the responsibilities of both the software and the hardware sides to achieve an overall non-interference property~\cite{clarkson2010hyperproperties}. 
% \thomas{I removed the "how they interact": the contract does not mention how they interact, right? simply the responsibilities of both side.}
In the rest of this paper, we name a \emph{security property for secure speculation} (often shortened \emph{security property}) any contract that can be formalized by the following \cref{eq:4trace}:
\begin{equation}    
\begin{aligned}
&\forall P, M_{pub}, M_{sec}, M_{sec}', \\
\text{\textbf{if}}\quad & O_{ISA}(P,M_{pub},M_{sec})=O_{ISA}(P,M_{pub},M_{sec}') \\
\text{\textbf{then}}\quad & O_{\mu Arch}(P, M_{pub},M_{sec}) = O_{\mu Arch}(P, M_{pub},M_{sec}') & 
\end{aligned}
\label{eq:4trace}
\end{equation}
The formula states that when running a program $P$ with public memory $M_{pub}$ and secret memory $M_{sec}$ on a microarchitecture processor $\mu Arch$, if the program $P$ satisfies an indistinguishability software observation constraint, then the actual observation when executed on the hardware remains indistinguishable.
In other words, if the secret was not leaked by the software itself, the formula verifies that the hardware does not leak the secret through microarchitectural side-channel observations. 
\mengjia{can we make the formula one to the background?}
\qt{I'd rather put it here as it is closer to the baseline and our scheme. Readers might want to refer to this formula often when they read those two schemes.}
\mengjia{but it will make our life much easier to say in the background, we can define what uarch is and what ISA constraint is... Also it will be less repetitive...}
\qt{I tried to move it to background, please check.}

The software constraint (line 2 in \cref{eq:4trace}) forces the observations of the program's behavior when executing sequentially (i.e., not speculatively) to be independent of the secret. 
% \thomas{I commented-off a sentence that was confusing me : "the ISA semantics of the processor". }
% Therefore, we denote the software constraint using a function $O_{ISA}$, read as a function to derive the ISA observation trace.
The software constraint uses a function $O_{ISA}$ that computes the ISA observation trace of a program. 
Typically $O_{ISA}$ extracts observations from a simple single-cycle implementation of the ISA \asplosrev{and thus does not involve microarchitectural timing information}. (We use an RTL implementation for practical convenience.)
% \thomas{Small modification $O_{ISA}$ is not itself the software constraint. It is a pair of observations that form the constraint. (Old version kept in comment)}
When the program satisfies the software constraint, line 3 in \cref{eq:4trace} states that the microarchitecture observation traces, computed using $O_{\mu Arch}$, must also be independent of the secret. 
The observations in $O_{ISA}$ will depend on the software-contract. 
The observations in $O_{\mu Arch}$ will depend on the attacker observation model and may include processor state and side channel information such as instruction commit times.

%In \cref{eq:4trace}, all traces include event timing, e.g. the commit time for instructions in the $\mu Arch$ machine, but also the time when each instruction get processed in the ISA machine.
%\mengjia{check. not sure it is the right place. I think the property does not require so, but our baseline scheme does what you describe above.} \sm{Does my sentence above take care of this?}

\mengjia{here we repeat something as in the background. Or maybe a better idea is to merge them?}
\qt{I merged some sentences here to background. If it works, then we can remove the above two paragraphs and the following paragraph.}

Note that \cref{eq:4trace} does not describe a single contract but a large family of contracts.
The equation is parameterized by different observation functions that can formalize various contracts.
For example, in the sandboxing contract, the ISA observation trace consists of the per-cycle content of the register file, which implies the contract assumes the software does not load secrets into registers.
In contrast, in the constant-time programming contract, the ISA observation trace includes both the memory access trace and the program counter trace, as the constant-time programming rule requires those traces to be independent of secrets.

\mengjia{this may be a good opportunity to clarify what exactly we target...}
\qt{Do you mean clarify that we only do two contracts? I think the two scheme are not limited to these two contracts. We are just evaluating using these two contracts.}



\paragraph{Observation}
Verifying a security property requires performing \textit{two} kinds of equivalence checks that involve \textit{four} traces.
%\thomas{Why just 2? TODO double check with everyone}
The equivalence check at line 2 in \cref{eq:4trace} is the \textit{\swcheck} to determine whether a program $P$ needs to be protected (we say that $P$ is valid), and the equivalence check at line 3 is the \textit{\hwcheck} to determine whether the microarchitecture processor $\mu Arch$ has a correct defense mechanism for the given program.
\asplosrev{Intuitively we need to reason about four machines (each accounts for a trace) in parallel to verify such a security property as we will show in the baseline scheme below.
However, our insight later shows that it is possible to only reason about two machines in parallel while still correctly verifying the property, which can greatly reduce the state space and the verification complexity. }
\mengjia{why we add this sentence? how can this sentence help?} \qt{I just want to give a hint about the evolution from the baseline to our scheme.}\mengjia{I think the hint is too subtle. It is better to be either explicit or not mention it.}

% \mengjia{pose condition needs to be agnostic to the source of speculation...}



% Finally, we formally define the speculative-non-interference property related to a contract.
% Given a speculative leakage contract $C$, a program $P$ that executes on a micro-architecture $\mu$ with public memory $M_p$ and secret memory $M_s$, the ISA level observation is $O_{ISA}(C,P,M_p,M_s)$ and the micro-architectural observation is $O_{\mu Arch}(P,M_p,M_s)$, $\mu$ is adhering to $C$ iff.
% \begin{equation}    
% \begin{aligned}
% &\forall P, M_p, M_s, M_s', \\
% & O_{ISA}(C,P,M_p,M_s)=O_{ISA}(C,P,M_p,M_s') \\
% &\rightarrow O_{\mu Arch}(P,M_p,M_s) = O_{\mu Arch}(P,M_p,M_s') & 
% \end{aligned}
% \label{eq:4trace}
% \end{equation}
% This property states that if for a program $P$ the attacker's ISA level observation is the same regardless of the secret ($M_s,M_s'$ are distinct), then the micro-architectural level observation should also be equivalent.
% Otherwise, there is secret information leakage due to speculative execution attacks.

% For the rest of this paper, we will call the $O_{ISA}$ equivalence check in Property~\ref{eq:4trace} Contract Assumption Check, and call the $O_{\mu Arch}$ equivalence check in Property~\ref{eq:4trace} Leakage Assertion Check.



% This scheme can achieve unbounded security proof because we do not set any bounds on the cycles that the model checker should explore, which means any potential attacks that takes any number of cycles can be captured.
% If a counterexample is found, then it must indicate a real attack.
% Because we assume that the out-of-order processor issues at most one instruction in a cycle, the 1-cycle processor always finish the same instruction faster than the out-of-order processor.
% This means whenever there is an deviation between $O_{\mu Arch_1},O_{\mu Arch_2}$, , i.e. a counterexample to Leakage Assertion Check, detected, all the instructions that have been or are being executed by the out-of-order processors have already finished in the 1-cycle processors.
% If any of these instructions violate the ISA level requirement, this trace should have already been filtered out by Contract Assumption Check and the deviation between $O_{\mu Arch_1},O_{\mu Arch_2}$ should not be detected.
% Thus, a counterexample found by our scheme must be caused by a real attack that violates Leakage Assertion Check while still satisfying Contract Assumption Check.



\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{images/baseline.pdf}
    \caption{The baseline verification scheme. Two instances of the single-cycle machine are used for \swcheck and two instances of the out-of-order (OoO) processor are used for \hwcheck.}
    % Both checks are conducted cycle by cycle (marked as $C_1$, $C_2$, $C_3$, ...), which is the same as instruction by instruction for 1-cycle processors (marked as $I_1$, $I_2$, $I_3$, ...).}
    % \mengjia{1. Bold the text for \swcheck and \hwcheck. 2. can we remove C1/C2.. I think the figure is clear without it; 3. add question mark for the cycle-by-cycle equation check} \sm{$C$, and $I$ in the figure are not clear.}
    % \mengjia{use $M_{sec}$ and $M_{pub}$ to match the formula 1}
    % \mengjia{@Qinhan, can you make some minor changes: 1) OOO -> OoO; 2) add a legend for time: an arrow to the right and have text "time" above it}
    \label{fig:baseline}
\end{figure}

% \mengjia{many reviewers do not understand how our shadow logic looks like. How about we show them? it would be better if we show an architecture figure of how the shadow logic being interacted the existing logic, such as ROB etc...}


\subsection{The Baseline Verification Scheme}
\label{sec:insight:baseline}

The security property (\cref{eq:4trace}) can be tentatively verified using the scheme visualized in \cref{fig:baseline}.
First, two copies of a single-cycle machine are instantiated as two separate RTL modules.
The two modules have identical RTL code with the instruction memory and public data memory initialized with the same content ($P$ and $M_{pub}$) and different secret memory ($M_{sec}$) \footnote{\asplosrev{In practice, the instruction memory and data memory do not necessarily need to be separated as long as the secret location can be clearly specified.}}.
% , denoted using different colors.
Note that the scheme includes the instruction memory instead of treating $P$ as input to the system. 
%\sm{Not completely true!} \sm{Single copy of program memory... need to clarify that.}
%\thomas{What does it mean to treat P as input? Was the intended point to say that something along the line off: the 2-4 machines don´t get their response from the instruction memory necessarily at the same time? (from a security persepctive, such a scenario would be seemingly suspicious no?) - need zoom discussion/clarification}
%\mengjia{according to our discussion today, we have that really because that is the memory and we do not want to change the RTL code of the processor, right?}
This is because (i) there could be branch instructions jumping back to old instructions in the program and (ii) all four processors need to run the same program.
% , which cannot be realized without a storage for the program.  \thomas{commenting the "cannot"}
%\sm{And that all processors need to execute the same program.}
%\qt{I add two sentences here to explain why we need instruction memory in the system.}
The two instances of single-cycle machine execute instructions sequentially, finishing one instruction per cycle, which models the ISA semantics of the out-of-order processor being verified.
These two copies execute in a lock-step manner, allowing the verification scheme to derive the $O_{ISA}$ trace at each cycle and compare them for equivalence to perform the \swcheck.

Similarly, the RTL for the out-of-order processor is duplicated to create two instances, which only differ in the secret memory. The program memory $P$ and the initial value of the public data memory $M_{pub}$ is the same as in the single-cycle machine. 
The verification scheme %computes and 
compares the microarchitecture execution traces $O_{\mu Arch}$ from the two machines at each cycle for the \hwcheck.

\asplosrev{In the verification, we assume that \swcheck is never violated and check the assertion that \hwcheck always holds.
If a trace is found to violate our assertion, it must be a valid attack trace that satisfy \swcheck, otherwise it should have already been discarded due to violation of the assumption.}

This scheme runs the \swcheck and \hwcheck in parallel at each cycle, allowing for conducting both bounded and unbounded checking.
Prior work~\cite{yang2023pensieve} first performs the \swcheck to filter out invalid programs and then perform the \hwcheck, which does not support unbounded checking involving traces of unbounded length.

\mengjia{add discussion on how prior work scale }


\subsection{Verification Performance Optimization}

The baseline verification scheme has serious scalability challenges (shown in \cref{sec:eval}).
% \yuheng{Do we have in-order 4-copy result? Check}
Its applicability to RTL verification is limited, as it is even unable to produce unbounded proof of \cref{eq:4trace} for in-order processors within 7 days, let alone for out-of-order processors.
% Its applicability to out-of-order processors is limited, as it is unable to produce unbounded proof of \cref{eq:4trace} within a reasonable timeframe (24 hours).
% \mengjia{I remember they cannot find proof even for in-order processors. I wrote this when I thought they can prove for in-order processors. We can change the text. Maybe remove it.}
% \mengjia{check: is it true? the 4-copy cannot work (including bug-finding) with any out-of-order processors?}
% \qt{4-copy can capture bugs but cannot find any proof}\thomas{The thing is "bug finding" is a tricky one to characterize: there are bugs that are really shallow and easy to find for tools, and there are bugs that are really hard to find. One way might have been to seed a bug ourselves, and show how one method does not find it before timeout, when the other does, but it is not fully convincing neither. (discussion how to navigate this problem)? }
% This limitation raises significant concerns, particularly considering that 
% increasing attention is paid to speculative execution vulnerabilities in out-of-order processors.
%\mengjia{I edit the sentence, because the baseline even cannot prove for in-order processors.}

In this paper, our goal is to tackle the performance issue by significantly reducing the size of the state machines utilized in verification.
Since the baseline verification scheme employs four state machines (for the four processors) and likely entails a non-trivial amount of redundancy among them, we aim to explore the possibility of reducing this redundancy.

One appealing option is to remove the duplicated single-cycle and duplicated out-of-order machines.
However, these duplicated machines were needed to include two different values of the secret in each case ($M_{sec}$ and $M_{sec}'$ in \cref{eq:4trace}), and check for non-interference, i.e., the value of the secret does not impact the observations. 
Prior work~\cite{tiwari2009complete} has proposed to use taint tracking to verify the non-interference property over a single trace. However, this requires a trade-off between precision and the taint-tracking overhead~\cite{hu2011theoretical}. We consider it a promising yet orthogonal research direction (\cref{sec:related}).
\qt{I do think it is unnecessary to mention taint propagation here, because we are just choosing one road to optimize, we do not need to explain why other roads cannot work. I think we can remove the above paragraph and directly present our scheme.}



\mengjia{so many defensive writing early on...}
Alternatively, we propose to remove the two single-cycle machines. 
As mentioned in Section~\ref{sec:intro}, the out-of-order processor needs to be functionally correct for it to be reliably used in checking \cref{eq:4trace}.
\asplosrev{Since functional verification is a separate concern and is a well-studied problem, we do not include it in our scheme.}
For the rest of the paper, we assume that the out-of-order processor is functionally correct and produces results that match the single-cycle ISA semantics.
Consequently, the single-cycle machine's execution trace can be reconstructed from the out-of-order processor's committed instruction sequence.
In other words, the single-cycle machine is contained in the out-of-order machine, including the complex instruction decoding, the execution logic, as well as registers/memory state.
This insight leads to our verification scheme, introducing shadow logic to perform \swcheck directly on the out-of-order processors.
% Note that this technique does not use any knowledge of presumed attack patterns and is general enough to apply to any out-of-order processors without loss of generality.

% \thomas{I moved the paragraph about functional correctness down to discussion}


% {\color{blue}\footnotesize

% \noindent\textbf{sw-hw trace}
% \begin{itemize}
%     \item recall from \cref{sec:background:contract}, software-hardware contract defines how software and hardware coordinate to achieve a security property with regards to speculative execution.
%     \item The different contracts in that section can be formulated as the formula below \cref{eq:4trace}.
%     \item Given a program P, a memory consisting of a public region denoted as Mp and a secret region, denoted as Ms and Ms'. If the program sequentially executes (corresponding to its ISA semantics) generating a trace using the function OISA does not leak secrets, then the hardware needs to ensure the same program executing on an out-of-order processor does not leak secrets via microarchitecture side channels, where all the microarchitecture effects can be summarized in a function Ouarch.
%     \item In formula 1, there exist two "equality check" operations. Heavy...
%     \item The first equality check aims to determine whether the given program satisfies the software constraint.
%     If it does not satisfy the software constraint, for example, if the software program itself has alredy leaked secrets when executing non-speculatively, we require hardware to do nothing.
%     \item If the \swcheck passes, the second equality check becomes relevant, which we refer to as \hwcheck. Examples of hardware traces can be cache access patterns etc.
%     \item In summary, to verify against software-hardware contracts, we will need to perform a \swcheck on a pair of traces generated for the ISA semantics of the out-of-order processor, and a \hwcheck on another pair of traces generated by the out-of-order processors.
% \end{itemize}

% \noindent \textbf{baseline verification scheme}
% \begin{itemize}
%     \item directly translate the security property to the verification scheme as follows
%     \item \cref{fig:method} shows the verification scheme
%     \item two copies of a single-cycle CPU is instantiated (RTL code), both taking the same P (initial state of the instruction memory), and Mp (public memory) but differ in Ms.
%     \item The two copies of single-cycle CPU execute instructions sequentially and execute one instruction per-cycle
%     \item For each cycle, we derive the OISA from the current state of the machine, for example, it could be a function of the register states (the sandboxing context) or the memory sequences (the constant-time context).
%     \item Similarly, we derive the Ouarch from the out-of-order processor, 
%     \item the assertion is written as below:\\
%     \texttt{assume contract\_assumption\_check = True, assert leakage\_assertion\_check = True}
% \end{itemize}

% \noindent \textbf{opportunity}
% \begin{itemize}
%     \item problem: large state machine, in particular, we are aware that the OoO processor is necessary
%     \item reduce the number of copies for each CPU. Challenging: prior work uses taint logic -> cite Tim and Ryan Kaster's work -> heavy (@Sharad, can we comment on more about why it does not work? If too long, may move to related work.)
%     \item the single-cycle CPU can be potentially large... put numbers
%     \item Key observation is that they are encapsulated inside the out-of-order processors
%     \item perform both \swcheck and \hwcheck on the pair of out-of-order processors
% \end{itemize}
% }


==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf \

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> ykfkyxzqqtggdstybhwmzfvqmnwcsnwh/Artifact.tex <==
\section{Artifact Appendix}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Abstract}

Our artifact is the infrastructure for verifying the two software-hardware contracts on four processors listed in \cref{tab:eval:setup}.
It includes the baseline verification scheme using four copies of processors and our verification scheme using contract shadow logic.
This artifact can be used to reproduce the verification results, including the time it takes and the attacks it finds, shown in \cref{tab:eval:all}, \cref{tab:eval:compare-defense}, and \cref{fig:eval:size-time}.

\subsection{Artifact check-list (meta-information)}

{\small
\begin{itemize}
  \item {\bf Run-time environment: } JasperGold and Dask.
  \item {\bf Hardware: } A >16-core machine with 4GB memory per core.
  \item {\bf Output: } Terminal outputs and a figure. Example results are included.
  \item {\bf Experiments: } Running the provided scripts will reproduce the results. Results will vary due to the performance of the machine and the randomness in JasperGold's solving engines.
  \item {\bf How much disk space required (approximately)?: } 1GB.
  \item {\bf How much time is needed to prepare workflow (approximately)?: } 20 minutes.
  \item {\bf How much time is needed to complete experiments (approximately)?: } On a >16-core machine, it takes $\sim$3 hours to complete most ($\sim$42 out of 54) experiments and 7 days to complete all experiments.
  \item {\bf Publicly available?: } Yes.
  \item {\bf Code licenses (if publicly available)?: } MIT license.
  \item {\bf Archived (provide DOI)?: } To Be Assigned.
\end{itemize}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Description}

\subsubsection{How to access}

\url{https://github.com/qinhant/ShadowLogicArtifact}.

\subsubsection{Hardware dependencies}

The experiments only require CPU and memory resources.
When running the experiment of a specific configuration, it will take $\sim$1.2 cores.
We provide scripts to run experiments of many configurations in parallel and thus recommend a >16-core machine to finish them in a shorter time.
4GB memory per core is recommended to avoid out-of-memory errors.

\subsubsection{Software dependencies}

JasperGold FPV by Cadence~\cite{website:jaspergold} is required to run the experiments.
It is a commercial hardware verification tool that requires a license to use.
Our scripts assume JasperGold can be launched through \texttt{jg} commands from the terminal.
Dask~\cite{Dask} is used to launch multiple experiments in parallel, it can be installed with \texttt{python3 -m pip install "dask[complete]"}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Installation}

Download the artifact folder to the machine and make two copies of it, which will be used to launch two batches of experiments.
No other installation is required.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Experiment workflow}

This artifact is used to reproduce the verification results on various tasks shown in \cref{tab:eval:all}, \cref{tab:eval:compare-defense}, and \cref{fig:eval:size-time}.

For each verification task, the verilog source code is located in the \texttt{src} folder, including four processors (\texttt{Sodor}, \texttt{SimpleOoO}, \texttt{Ridecore}, and \texttt{BOOM}).
Each processor has its corresponding top module to conduct baseline verification scheme and our verification scheme using contract shadow logic under both sandboxing and constant-time contracts.
The JasperGold scripts to launch each verification task are located in the \texttt{verification} folder.

The users of this artifact can use scripts provided in the \texttt{results} folder to launch batches of verification tasks.
When the batches are running, the user can check the results of finished tasks by using the provided scripts to parse the log files and print out a summary of all verification results.
A plotting script is provided to reproduce \cref{fig:eval:size-time}.





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Evaluation and expected results}

\paragraph{Reproduce \cref{tab:eval:all} and \cref{tab:eval:compare-defense}}
In the first copy of the artifact folder, we first initialize a cluster of 12 worker threads with:

\begin{minipage}{\columnwidth}
\begin{lstlisting}[]
(python3 -u scripts/dask/initCluster.py 12 \
         > & initCluster.log &)
\end{lstlisting}
\end{minipage}
Then, launch the batch of verification tasks with:

\begin{minipage}{\columnwidth}
\begin{lstlisting}[]
(python3 -u results/CompareTable/run.py \
         > & run.log &)
\end{lstlisting}
\end{minipage}

When the verification tasks are running, they will produce \texttt{my\_proj\_*} folders as JasperGold's project folder, \texttt{terminal\_*.log} files as JasperGold's terminal output files, and \texttt{my\_jdb\_*} files saving the attacks found.
Users can run the following commands to parse JasperGold's terminal output files and print out a summary of verification results on finished tasks:

\begin{minipage}{\columnwidth}
\begin{lstlisting}[]
python3 results/CompareTable/summary.py
python3 results/CompareTable/print.py
\end{lstlisting}
\end{minipage}
The commands can be repeated as more tasks are finished.

The summary is listed processor-by-processor.
\texttt{results/CompareTable/example.log} is an example of it.
For each processor, there will be three arrays:

\begin{itemize}[leftmargin=*]
\item
The first array is the names of the verification tasks with the following naming convention:
\texttt{sandbox} and \texttt{ct} represents the sandboxing and constant-time contracts.
\texttt{4copy} and \texttt{2copy} represents the baseline verification scheme and our scheme.
For the \texttt{SimpleOoO}, the array includes six versions of the processor, including the insecure version with no defense scheme followed by the five versions with defense augmentation listed in \cref{tab:eval:compare-defense}.

\item
The second array indicates whether the processor under test is secure.
\texttt{1} indicates the processor is secure, \texttt{0} indicates an attack is found, and \texttt{-1} indicates the experiment has not finished.
You could further open JasperGold's GUI to check the attacks found with:

\begin{minipage}{\columnwidth}
\begin{lstlisting}[]
jg -command "restore -jdb my_jdb_{expName}"
\end{lstlisting}
\end{minipage}

\item
The third array includes the time it takes for the verification tasks to finish in the unit of seconds.
\texttt{-1.0} indicates the experiment has not finished.
\end{itemize}

It takes $\sim$3 hours to complete most ($\sim$25 out of 34) tasks and 7 days to complete all experiments.
The summary is used to fill in the information in \cref{tab:eval:all} and \cref{tab:eval:compare-defense}.
Be aware that the results will vary due to the performance of the machine and the randomness in JasperGold's solving engines.




\paragraph{Reproduce \cref{fig:eval:size-time}}
In this batch of experiments, we can share the cluster created for the last batch.
To launch the experiments, move to the second copy of the artifact folder and use similar commands as before:

\begin{minipage}{\columnwidth}
\begin{lstlisting}[language=bash]
(python3 -u results/ScalabilityFigure/run.py \
         > & run.log &)
## Wait ~3 hours to see most results.
python3 results/ScalabilityFigure/summary.py
python3 results/ScalabilityFigure/print.py
## Example print-outs in `example.log`.
\end{lstlisting}
\end{minipage}
The naming convention in the summary further includes \texttt{RF*\_MEMI*\_MEMD*\_ROB*} to indicate the size of register file, data memory, instruction memory, and re-order buffer.
These parameters are scaled up to demonstrate how verification time will increase in \cref{fig:eval:size-time}.

To reproduce the figure, we provide a template script in  \texttt{results/ScalabilityFigure/plot.py}.
The array \texttt{time} in it stores the verification time to be plotted.
The two sub-arrays in it correspond to the sandboxing and constant-time contracts.
Each sub-array contains verification time when varying register, data memory, and re-order buffer sizes among 2, 4, 8, and 16.
Carefully update the array \texttt{time} in it based on the experiment summary (be aware that 3 data points should be omitted because they cannot finished within 7 days in our machine setup) and plot with:

\begin{minipage}{\columnwidth}
\begin{lstlisting}[]
python3 results/ScalabilityFigure/plot.py
\end{lstlisting}
\end{minipage}

Finally, terminate the cluster by finding the \texttt{PID} of the thread and kill it:

\begin{minipage}{\columnwidth}
\begin{lstlisting}[]
ps -ef | grep initCluster.py
kill XXXX
\end{lstlisting}
\end{minipage}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Methodology}

Submission, reviewing and badging methodology:

\begin{itemize}
  \item \url{https://www.acm.org/publications/policies/artifact-review-badging}
  \item \url{http://cTuning.org/ae/submission-20201122.html}
  \item \url{http://cTuning.org/ae/reviewing-20201122.html}
\end{itemize}

==> ykfkyxzqqtggdstybhwmzfvqmnwcsnwh/Background.tex <==
%!TEX root = main.tex
\section{Background}
\label{sec:background}

% \mengjia{the term "shadow logic" needs to be given a definition in background.}

\subsection{Speculative Execution Attacks and Defenses}
\label{sec:background:spec}

Speculative execution attacks exploit the microarchitectural side effects of transient instructions.
%, i.e., the instructions that are speculatively executed and squashed later due to misprediction.
Transient instructions can be introduced via a wide range of speculation features, including branch history prediction~\cite{kiriansky2018speculative}, branch target prediction~\cite{Kocher2018spectre}, return address prediction~\cite{koruyeh2018spectre,maisuradze2018ret2spec}, store-to-load forwarding~\cite{horn2018speculative},
% % \thomas{The sentence is slightly wrong: technically no transient instruction is introduced by store-to-load forwarding/value prediction. Maybe we don´t care?}\mengjia{the definition of transient instructions are they are speculatively executed and squashed later. So even store-to-load forwarding/value prediction fits within this definition. Maybe we should bring back the definition of transient instructions.}
value prediction~\cite{vicarte2021opening}, and 4K aliasing~\cite{canella2019fallout}.
The side effects of transient instructions are diverse, including modifying the cache states~\cite{Kocher2018spectre, Lipp2018meltdown,koruyeh2018spectre,maisuradze2018ret2spec,kiriansky2018speculative}, TLBs~\cite{gras2018translation}, Line Fill Buffer~\cite{schwarz2019zombieload}, and DRAMs~\cite{tobah2022spechammer}.
% and Networks-on-chip~\cite{xx}.
% Speculative execution is a micro-architecture feature to improve the performance of modern processors.
% It allows processors to speculatively execute instruction sequences before they can determine the correct sequences specified by the program.
% These speculatively executed instructions will be squashed if they are later found out to be incorrect.
% However, they can leave side effects on various micro-architecture structures and leak information.


% The information leakage of speculative execution are exploited to break many well-studied secure programs.
% The key reason is that the leakage can be introduced by the speculative instruction sequences that mismatch the intention of the program.
% For example, under the speculative execution, the boundary check of an array access can be skipped, which allows the attacker to access an arbitrary memory location~\cite{Kocher2018spectre}.

% \mengjia{the above description of speculative execution attacks can be more concise. 
% + need to talk about various sources of speculation.}

Speculative execution vulnerabilities can be mitigated via software and hardware methods.
In software, existing mitigations typically involve placing \texttt{fence} instructions after sensitive branch instructions to delay the execution of the subsequent instructions until the branch is resolved~\cite{amd2023software,intel2021intel}.
Other software approaches involve replacing branch instructions with \texttt{cmov} instructions and using bit masking of the index used for array lookups~\cite{carruth2018speculative}.
% \mengjia{TODO: maybe mention GLIDE, Spectre era (some of Sanjay's work from UCSD)}
Hardware mitigation mechanisms focus on restricting speculative execution by either selectively delaying the execution of instructions that can potentially transmit secrets via side channels~\cite{sakalis2019efficient,yu2019speculative, loughlin2021dolma, weisse2019nda} 
or making it difficult for attackers to observe the microarchitectural side effects of speculative instructions~\cite{yan2018invisispec,ainsworth2021ghostminion, ainsworth2020muontrap, khasawneh2019safespec}.


% Various micro-architecture defenses are proposed to mitigate such attacks.
% In general, they try to restrict the micro-architecture effects of the speculative instructions such as by delaying them~\cite{sakalis2019efficient,yu2019speculative} or by isolating their effects~\cite{yan2018invisispec,ainsworth2021ghostminion}.
% However, the defenses are frequently found out to be insufficient when new attacks~\cite{behnia2021speculative,fustos2020spectrerewind} are discovered.

% \mengjia{maybe hint here that defenses are achieving different security properties.. rather than saying they are broken...}


\subsection{SW-HW Contracts for Secure Speculation}
% \subsection{Speculative Leakage Contract}
\label{sec:background:contract}


% \mengjia{Ongoing: to make this subsection shorter by removing detailed discussion on the two code snippets}

As speculative execution vulnerabilities can be mitigated via either software or hardware methods, it becomes challenging to cleanly and explicitly reason about security properties a defense should achieve.
% Intuitively, a more aggressive hardware defense scheme usually comes with relatively high performance overhead but can securely execute a large number of programs. 
% In contrast, a more limited defense mechanism can offer better performance but usually can only support a restricted set of programs, or it requires the program to incorporate defensive software mitigations.
% As the software and hardware need to coordinate to achieve a final security property, 
The community has been using \textbf{software-hardware contracts} to define security properties precisely related to speculative execution vulnerabilities.

Guarnieri et al.~\cite{guarnieri2021hardware} proposed the first set of formalized contracts by defining which program executions a side channel adversary can distinguish.
Specifically, a contract states that: ``if a program satisfies a specified \textbf{software constraint}, then the hardware needs to achieve a \textbf{noninterference} property to ensure no secrets are being leaked.''
Formally, a contract can be written as follows:

\begin{equation}    
\begin{aligned}
&\forall P, M_{pub}, M_{sec}, M_{sec}', \\
\text{\textbf{if}}\quad & O_{ISA}(P,M_{pub},M_{sec})=O_{ISA}(P,M_{pub},M_{sec}') \\
\text{\textbf{then}}\quad & O_{\mu Arch}(P, M_{pub},M_{sec}) = O_{\mu Arch}(P, M_{pub},M_{sec}') & 
\end{aligned}
\label{eq:4trace}
\end{equation}

The formula states that when running a program $P$ with public memory $M_{pub}$ and secret memory $M_{sec}$ on a microarchitecture processor $\mu Arch$, if the program $P$ satisfies an indistinguishability software observation denoted by $O_{ISA}$, then the actual observation when executed on the hardware denoted as $O_{\mu Arch}$ remains indistinguishable.
% In other words, if the secret was not leaked by the software itself, the formula requires that the hardware does not leak the secret through microarchitectural side-channel observations.



Note that \cref{eq:4trace} does not describe a single contract but a family of contracts.
The equation is parameterized by different execution modes at the software level and different observation functions.
The scheme proposed in this paper supports the \textit{sequential} execution mode where the software constraint considers traces when executing the program sequentially (i.e., not speculatively).
For example, under a so-called sandboxing contract, the software constraint is that executing the program sequentially will not have secrets loaded into the register file.
The $O_{ISA}$ of sandboxing includes the data written to registers of every committed load.
In contrast, in the constant-time programming contract, the software constraint is that executing the program sequentially will not use secrets as addresses of instruction or data memory accesses or as operands to hardware modules whose timing depends on the input.
% will not emit secret-dependent data and instruction memory accesses.
This matches the constant-time programming discipline~\cite{guarnieri2021hardware}.
The $O_{ISA}$ of this contract includes the branch condition, memory address and multiplication operands of committed instructions.

The microarchitecture observation ($O_{\mu Arch}$) considered in this paper includes the address sequence
at the memory bus and the commit time of every committed instruction, which is commonly used in prior works~\cite{oleksenko2022revizor, yang2023pensieve} to reflect cache and timing side channels.
% \mengjia{what does it mean by commit time of potentially speculatively executed inst? if it is committed, it will not be trasient...}
% \qt{I think we can just say commit time of every committed instruction.}
% \mengjia{sure.}


% {\color{gray}
% \yuheng{Make sure we cover this paragraph in background. Then remove this paragraph.}
% In the sandboxing contract, the \swcheck ensures the committed memory access instructions do not access the secret memory region $M_{sec}$.
% In the constant-time programming contract, the ISA traces consist of the memory addresses of load/store instructions, branch conditions, and multiplication operands.
% In both contracts, the microarchitecture traces consist of the memory addresses being issued from the processor and every instruction's commit cycle id.
% }

% For example, in the sandboxing contract, the ISA observation trace consists of the per-cycle content of the register file, which implies the contract assumes the software does not load secrets into registers.
% In contrast, in the constant-time programming contract, the ISA observation trace includes both the memory access trace and the program counter trace, as the constant-time programming rule requires those traces to be independent of secrets.

% The contract is parametric as a user can specify 1) what the software constraint is, and 2) what the attacker's observable microarchitecture events are to distinguish for noninterference.
% The former question divides contracts to apply to different security scenarios, which we detail shortly.
% The latter question covers broad microarchitecture events, including memory access traces, program counter traces, or termination time.


% Typically $O_{ISA}$ extracts observations from a simple single-cycle implementation of the ISA and thus does not involve microarchitectural information. 
% $O_{\mu Arch}$ depends on the attacker observation model and may include processor microarchitectural state and side channel information such as instruction commit times.



% \mengjia{I copied the discussion of security property from the insights section here... TODO: adjust sentences...}
% The formula states that when running a program $P$ with public memory $M_{pub}$ and secret memory $M_{sec}$ on a microarchitecture processor $\mu Arch$, if the program $P$ satisfies an indistinguishability software observation constraint, then the actual observation when executed on the hardware remains indistinguishable.
% In other words, if the secret was not leaked by the software itself, the formula verifies that the hardware does not leak the secret through microarchitectural side-channel observations. 
% \mengjia{can we make the formula one to the background?}
% \qt{I'd rather put it here as it is closer to the baseline and our scheme. Readers might want to refer to this formula often when they read those two schemes.}
% \mengjia{but it will make our life much easier to say in the background, we can define what uarch is and what ISA constraint is... Also it will be less repetitive...}
% \qt{I tried to move it to background, please check.}


\begin{comment}
The software constraint (line 2 in \cref{eq:4trace}) forces the observations of the program's behavior when executing sequentially (i.e., not speculatively) to be independent of the secret. 
% \thomas{I commented-off a sentence that was confusing me : "the ISA semantics of the processor". }
% Therefore, we denote the software constraint using a function $O_{ISA}$, read as a function to derive the ISA observation trace.
The software constraint uses a function $O_{ISA}$ that computes the ISA observation trace of a program. 
Typically $O_{ISA}$ extracts observations from a simple single-cycle implementation of the ISA \asplosrev{and thus does not involve microarchitectural timing information}. (We use an RTL implementation for practical convenience.)
% \thomas{Small modification $O_{ISA}$ is not itself the software constraint. It is a pair of observations that form the constraint. (Old version kept in comment)}
When the program satisfies the software constraint, line 3 in \cref{eq:4trace} states that the microarchitecture observation traces, computed using $O_{\mu Arch}$, must also be independent of the secret. 
The observations in $O_{ISA}$ will depend on the software-contract. 
The observations in $O_{\mu Arch}$ will depend on the attacker observation model and may include processor state and side channel information such as instruction commit times.

%In \cref{eq:4trace}, all traces include event timing, e.g. the commit time for instructions in the $\mu Arch$ machine, but also the time when each instruction get processed in the ISA machine.
%\mengjia{check. not sure it is the right place. I think the property does not require so, but our baseline scheme does what you describe above.} \sm{Does my sentence above take care of this?}

\mengjia{here we repeat something as in the background. Or maybe a better idea is to merge them?}
\qt{I merged some sentences here to background. If it works, then we can remove the above two paragraphs and the following paragraph.}

Note that \cref{eq:4trace} does not describe a single contract but a large family of contracts.
The equation is parameterized by different observation functions that can formalize various contracts.
For example, in the sandboxing contract, the ISA observation trace consists of the per-cycle content of the register file, which implies the contract assumes the software does not load secrets into registers.
In contrast, in the constant-time programming contract, the ISA observation trace includes both the memory access trace and the program counter trace, as the constant-time programming rule requires those traces to be independent of secrets.

\mengjia{this may be a good opportunity to clarify what exactly we target...}
\qt{Do you mean clarify that we only do two contracts? I think the two scheme are not limited to these two contracts. We are just evaluating using these two contracts.}


% A contract involves two important components.
% First, what is the software constraint?
% The answer to this question divides contracts to apply to different security scenarios, which we detail shortly.
% Second, what are the attacker's observable microarchitecture events?
% These events include memory access traces, program counter traces, or the termination time.

% The community has widely agreed that there are two contracts that have practical and popular usage contexts targeting software sandboxing and constant-time programming, respectively. 
\asplosrev{We describe two common contracts below: sandboxing and constant-time programming, which will be the focus of this paper.}
% {We will also discuss which other contracts can be supported by our approach and which cannot in \cref{sec:discussions}.}
%(Other contracts are discussed in \cref{sec:discussions}.)
The sandboxing and constant-time programming contracts differ in the assumed software constraints.
\asplosrev{They share the same $O_{\mu Arch}$, which includes the address sequence at the memory bus and the commit time of every instruction.}
\cref{fig:contract_code} shows two code snippets to highlight the difference. 

% \mengjia{@Qinhan @Yuheng, could you put the two code snippet side by side and add a caption and put here. Maybe use subfigure?}




\begin{figure}[h]
\centering
    \begin{tabular}{cc}
    % \begin{lstlisting}[style=mystyle, language=mylang, label={lst:future}, caption={Example Code for Mircoarchitectural Deviation Caused by Later-Committed Instructions},captionpos=b]
\begin{lstlisting}[style=mystyle, language=C]    
if (x < size){
  val = mem[x] 
  if (val < size)
    dummy = mem[val]
}
\end{lstlisting} 
    
    % \end{tabular}
    % \end{center}
    % \end{minipage}
\quad \vline
&
    
    % \begin{minipage}{\columnwidth}
    % \begin{center}
    % \begin{tabular}{c}
    % \begin{lstlisting}[style=mystyle, language=mylang, label={lst:future}, caption={Example Code for Mircoarchitectural Deviation Caused by Later-Committed Instructions},captionpos=b]
\begin{lstlisting}[style=mystyle, language=C]
sec = mem[0]  
if (cond)
  dummy = mem[sec]
\end{lstlisting}
\\
    \scalebox{0.9}{(a) Sandboxing} & \scalebox{0.9}{(b) Constant-Time}
    \end{tabular}
    \caption{Example of programs to distinguish two contracts.}
    \label{fig:contract_code}
\end{figure}
\mengjia{TODO: omit this code snippet...}


\paragraph{Contract for Software Sandboxing}
Software sandboxing is a technique to restrict the execution of a potentially malicious program to stay within a predetermined memory region, i.e., a sandbox, disallowing the program to access secret data outside the sandbox.
\asplosrev{$O_{ISA}$ of the sandboxing contract consists of the values written to architectural registers of every instruction, which implies the contract assumes the software does not load secrets into registers.}
For example, \cref{fig:contract_code}(a) lists a Spectre V1 code gadget, where memory locations beyond the \texttt{size} bound contain secrets.
The branch instructions (lines 1 and 3) implement a sandboxing policy by performing bounds check to prevent sandbox escape.
% In this example, assume memory locations beyond the \texttt{size} bound contain secrets.
% \mengjia{check this?}
This contract only accepts programs without out-of-bound load instructions.
% In this program, an out-of-bound load instruction (line 2) should not happen at the software level.
% following ISA semantics.
% When executing this program, an out-of-bound load instruction that loads a secret value into a register (line 2) should not be executed following ISA semantics.
% \thomas{Not just never commit. Here, are we describing the sw restriction (in which case I think we should avoid using the keyword commit) or both the sw and the hw sides?}\mengjia{so will "not on the correct execution path" work better? Or "will not be executed in a sequential machine/following ISA semantics"}
% Hardware mitigations, such as STT~\cite{yu2019speculative} and NDA~\cite{weisse2019nda}, are designed for the sandboxing contract.
% \mengjia{I still feel adding "at the software level" may read better. Though repetitive, but a little bit less confusion.}
% \mengjia{commented out the STT/NDA thing after reading Stella's comments}

\paragraph{Contract for Constant-Time Programming}
Constant-time programming is a widely deployed technique to secure cryptographic libraries against microarchitecture side channels.
Different from the sandboxing contract, the program can access secret values (e.g., cryptographic keys), and can include instructions that load secrets into registers (line 1 in \cref{fig:contract_code}(b)).
% are allowed to execute at software level.

The constant-time programming \rev{discipline}\del{rule} requires the program not to use secret or secret-dependent variables as branch conditions and targets, addresses for memory access instructions, and operands for other variable-time operations such as multiplication.
\asplosrev{These observations are included in the $O_{ISA}$ of the constant-time contract.}
In \cref{fig:contract_code}(b), if \texttt{cond} is always false, then it is a constant-time program because line 3 will never be executed and the secret will not be used as address for memory access.
If \texttt{cond} can be true, then \cref{fig:contract_code}(b) is not a constant-time program.
Since secrets can be loaded into registers, mechanisms designed for the sandboxing contract are insufficient to prevent information leakage for programs considered in the constant-time programming contract.

\asplosrev{Note that verifying an RTL design against the constant-time contract means we are checking if the RTL design is secure against speculative execution attacks when the software running on it follows the constant-time programming discipline.
This is different from checking whether the software or the hardware is `constant-time'~\cite{schmitz2023upec, gleissenthall2019iodine}.}
\end{comment}

% \mengjia{since this is not the main claim of our contribution, I would suggest to remove this paragraph.} \qt{Yeah we should remove it.}
% {\color{gray}
% One of our contributions is the capability to support RTL verification for both contracts, as opposed to an important existing work (UPEC~\cite{fadiheh2020formal}), which is unable to handle the constant-time contract and is limited to the sandboxing contract only. 
% }


\subsection{RTL Verification using Model Checking}
% \subsection{RTL Functional and Security Verification using Model Checking}

% \mengjia{how about remove functional and security so we fit the title in one line?}

Model checking is widely used in verifying hardware designs, including processors~\cite{berezin2002verification} and accelerators~\cite{huang2018instruction}.
It is available as both open-source tools (e.g., AVR~\cite{goel2020avr}) and commercial tools (e.g., Cadence Jaspergold~\cite{website:jaspergold}) that directly work on RTL designs.
These tools are highly automated, where the user only needs to provide the hardware source code instrumented with the property to be checked.
%The tools then automatically translate the source code into a model and check the property on it.
Existing tools have flexible support to express various properties via instrumenting hardware code using a design-friendly language, e.g., System Verilog Assertions (SVA). SVA allows specifying (i)  assumptions (using the \texttt{assume} keyword) that describe system assumptions such as constraints on the inputs and (ii) assertions (using the \texttt{assert} keyword) to specify the property that the model checker is required to check, similar to assertions in C/Python. 

As model checking effectively considers all possible input sequences which can be of unbounded length, it provides an {unbounded-length proof} or a complete proof. 
When the property does not hold at some reachable state, model checking reports an input-sequence trace, a {counterexample}, for which the property fails.
% To address the scalability challenges of model checking, as an alternative, 
{Bounded model checking} (BMC) can be used to perform verification for {all possible input sequences of length bounded by some user-provided parameter $k$} - this effectively checks the property for all states reachable within $k$ steps from the initial state \rev{which is obviously not as strong as an unbounded-length proof}.

% \mengjia{it is a bit weird to put this paragraph here... maybe we should put it in the section when we talk about contract security property?}
The information leakage security property is a hyperproperty, i.e., it needs reasoning over two traces (corresponding to two different values of the secret) to prove or disprove it. This can be handled by constructing a model checking instance with two copies of the design (with different values of the secret), and constructing a property comparing traces over the two copies. 


\subsection{Shadow Logic}
\label{sec:background:shadow}

% \mengjia{TODO: make sure we say somewhere that shadow logic is only for verification purpose, and can be easily removed before synthesis... Also in PL, people also call it ghost state or something like htat}

When verifying complex RTL code, it is often necessary to introduce auxiliary code to assist verification by obtaining or deriving extra information from the current state of the system.
Such auxiliary code is called {shadow logic} (or ghost code in software verification~\cite{leino2010dafny}). 
This logic \textit{monitors} the design and assumes and asserts that certain conditions hold.

For example, consider a verification task that checks whether a processor correctly implements its ISA specification.
For every instruction that updates the register file, we need to check that when the instruction commits, the target register holds the value specified by the ISA. 
However, due to complex renaming logic in out-of-order processors, it is a nontrivial task to determine which register in the physical register file is the target register.
Prior work~\cite{reid2016end} customizes shadow logic according to the renaming logic to correctly locate the target register as part of this checking.

It is important that this shadow logic only \emph{monitors} the design and does \textit{not} make any modifications that change the behavior of the system. 
\cameraready{
It is common practice to implement shadow logic for verification purposes under some macro.
This enables this logic to be stripped out during design compilation and thus, shadow logic is not present in the final production RTL. 
% After the verification, the shadow logic can be easily removed from the code by disabling certain macros and will not be present in the run-time RTL.
}



==> ykfkyxzqqtggdstybhwmzfvqmnwcsnwh/Conclusion.tex <==
\section{Conclusions}
\label{sec:conclusion}
Our paper presents \name, a broadly-applicable approach for performing formal verification of security properties on RTL designs for software-hardware contracts.
Our scheme asks processor designers to construct shadow logic to extract ISA observation traces from processors and enforce the instruction inclusion and synchronization requirements.
Our evaluation shows the strength of our scheme compared with the baseline and two state-of-the-art RTL verification schemes in both finding attacks on insecure designs and deriving unbounded proofs for secure designs.

% \mengjia{TODO: adjust statements}
% Our scheme leverages design insights to reduce the complexity of the formal verification problem without making assumptions about expected attack patterns.
% The flexibility of the method allows us to accommodate multiple security properties, and working directly on the RTL allows us to minimize the risk of overlooking security-critical architectural structures. 
% We demonstrate the strength of our scheme against each of the state-of-the-art approaches along one or more of the dimensions of scalability and applicability.


==> ykfkyxzqqtggdstybhwmzfvqmnwcsnwh/Discussion.tex <==
\section{Limitations and Future Work}
\label{sec:discussions}

Despite being able to achieve significant verification performance improvement compared to the baseline and several related works, we acknowledge this paper has several limitations.
First, one appealing feature of our verification scheme is that the proposed contract shadow logic is \textit{conceptually} reusable across different designs, given that the primary task of the shadow logic is to simply extract committed instruction information.
We must concede that, thus far, constructing and synchronizing the shadow logic for the designs in our evaluation has relied on manual effort.
To further reduce the required manual effort, we want to investigate how to partially automate this process.
Our problem shares similarity to \emph{tandem verification}~\cite{Xing2022Generalizing} for functional correctness, where the same ISA-level information is extracted from RTL implementations. 
Applying techniques similar to~\cite{Xing2022Generalizing} might help in automating part of the effort.
% \thomas{added that because I realize that literally all the design we ever wrote were computing the ISA update. Though interestingly we were computing a "diff" instead of the full new state (because of memory). Maybe it should be in related work}


Second, our scheme does not fully address the scalability issue for verifying out-of-order processors with a realistic ROB size, which is usually above 100.
This scalability issue is a well-known problem in hardware verification.
On the positive side, we believe a reasonably reduced-size out-of-order machine already exhibits the essential security-relevant features of a real-size out-of-order machine, including speculation, resource contention, and instruction reordering.
However, we believe work can be done to further improve the scalability. 
One promising direction is to explore taint propagation techniques like GLIFT~\cite{tiwari2009complete,solt2022cellift}.
As studied in prior work~\cite{hu2011theoretical}, taint propagation requires making a delicate trade-off between precision and verification overhead. 
The taint propagation logic can be customized to the security property and specific hardware design to accomplish this.
We hypothesize that taint propagation techniques could be combined with our scheme to further improve verification performance.
% We consider exploring tainting propagation for verifying software-hardware contracts as a promising but challenging research direction and leave it for future work.

% \paragraph{Scaling Benefits over Baseline Design}
% Tables~\ref{tab:eval:compare-processor} and ~\ref{tab:eval:compare-defense} demonstrate the scaling benefits of our scheme over the baseline method, where we are able to find proofs where the baseline times out. We attribute these benefits to two sources: (i) The size of the reachable state set, and thus the model checking time, can depend exponentially on the number of state bits.
% While the difference in design size between the baseline design-under-verification and that for our scheme is relatively small for all the processors, this can have \emph{exponential} impact on the model checking capability between the baseline and our scheme. 
% (ii) The structure of the logic can provide further scaling benefits. Unlike the Baseline where the the $O_{ISA}$ and $O_{\mu Arch}$ observation variables are from different processors, they come from the same processor in our scheme and thus share significant logic. This potentially makes their comparison easier in the model checking process.


% \paragraph{Reduced-size Design}
% Our optimized scheme does not fully address the scalability issue for verifying out-of-order processors with a realistic ROB size, which is usually above 100.
% However, we consider our verification results on reduced-size designs valuable for reasoning about real-size designs \asplosrev{though verifying with reduced-size ROB may miss attacks requiring a larger speculation window}.
% The reason is that despite the quantitative difference in structural sizes, a reasonably reduced-size out-of-order machine already exhibits the essential security-relevant features in a real-size out-of-order machine, including speculation, resource contention, and instruction reordering.
% Our situation is reminiscent of the verification of concurrent software: 
% while originally people believed that concurrency bugs only occurred in the presence of a high number of concurrent actors, formal verification strategies~\cite{contextbounded2005qadeerrehof} showed that the same bugs often also existed in easier-to-verify reduced-size systems.

% \mengjia{need help here...}
% \thomas{I think you were making 3 different points here: 
% 1. JasperGold performance is a mystery in the best of times. 
% 2. The seeded LEAVE candidate invariants are insufficient. (I think that we understand this part: there are no invariants provided by LEAVE, because all the candidate invariants are false (if I remember what Yuheng said))
% 3. Relation between manually crafted invariants and the invariants of assumes and asserts in the shadowlogic. }

Finally, as we explore the relationship between manually crafted invariants and and the information embedded within our shadow logic, some additional insights emerge.
We speculate that our shadow logic may offer a rich array of invariants to the model checker.
This hypothesis is rooted in the notion that contract constraints, originally designed to constrain software programs, indirectly strongly constrain the set of reachable states of the processor.
However, more investigation is needed to understand the constraining power of the shadow logic and how this influences the performance of the verification procedure.
% Furthermore, while trying to inas we delve into the relationship between manually crafted invariants and those embedded within our shadow logic, intriguing insights emerge.
% We speculate that our shadow logic may offer a rich array of invariants to the model checker.
% This hypothesis is rooted in the notion that contract assumptions, originally designed to constrain software programs, indirectly strongly constrains the set of reachable states of the processor.

% Finally, an intriguing question came to us while working on the project is to understand what factor affects the verification performance of the model-checking tool.

% Besides, why the grammars of invariants provided by LEAVE are insufficient to work on out-of-order processors. \thomas{}


% We have some intuition that maybe our shadow logic presents a rich form of invariants to the model checker, since the contract assumptions, ruling out software programs also indirectly restricts reachable states in the processor.



% \paragraph{Other Contracts}
% We evaluate our scheme on two common contracts.
% Other contracts whose ISA traces can be derived only from the committed instructions can be supported as well.
% Less common contracts which require the software checks to track information of uncommitted instructions~\cite{guarnieri2021hardware} cannot be supported currently.


% \yuheng{Note from meeting: 1) auto generate shadow logic as future work. 2) invariants v.s. shadow logic. Are they transfer-able?}




% \paragraph{Hardware Taint Propagation}
% Taint propagation using techniques like GLIFT~\cite{tiwari2009complete,solt2022cellift} is an information flow checking technique designed to optimize the self-composition~\cite{barthe2011secure} based technique used in our scheme.\yuheng{Removed the word ``Alternative", which made the reviewer think its either Taint Analysis or us. We could actually be combined together. Use ``optimize" instead.}
% It only requires one copy of the system, but needs to add additional taint variables and taint propagation logic. 
% \asplosrev{Taint propagation allows to make the trade-off between precision and complexity and people need to select the right taint propagation rule dependent on the security property and specific hardware design.
% Potentially some taint propagation technique can also be combined with our scheme to further improve the verification performance.
% We consider exploring tainting propagation for verifying software-hardware contracts as a promising but challenging research direction and leave it for future work.}

==> ykfkyxzqqtggdstybhwmzfvqmnwcsnwh/Experiment.tex <==
\section{Experiment Results}
\label{sec:eval}




% \yuheng{Given no publish benchmark. We pick two related work to state where we are in the community. Tell them we are giving the best to evaluate. Let the first subsection to be thorough about related work. and convince them it is thorough to the best possible.}
% \yuheng{Need help with this summary paragraph.}

% \yuhengtext{
% In this section, we will first compare our scheme with the baseline, and two existing schemes, i.e., LEAVE~\cite{x} and UPEC~\cite{x}.
% In addition to the comparison, we further evaluate our scheme regarding how its performance can be affected by two factors, the defense mechanism and the structural sizes of ROB, register file, and memory.
% }






\subsection{Comparison with Baseline and Existing Schemes}
\label{sec:eval:compare}



\begin{table}[t]
  \setlength\tabcolsep{2pt}
  \centering
  \small

  \begin{tabular}{|l|c|c|c|c|c|} \hline
    & \multicolumn{5}{c|}{\textbf{Sandboxing Contract}} \\ \cline{2-6}
                  
    & \multicolumn{1}{c|}{\texttt{Sodor}}   & \multicolumn{1}{c|}{\texttt{SimpleOoO-S}}   & \multicolumn{1}{c|}{\texttt{SimpleOoO}}   & \multicolumn{1}{c|}{\texttt{Ridecore}}   & \multicolumn{1}{c|}{\texttt{BOOM}} \\ \hline\hline
                  
    Baseline
    &\timeout &\timeout &\bug &\bug &\graycell \\ \hline
  
    LEAVE~\cite{wang2023specification}
    &\secure &\falsealert &\falsealert &\graycell &\graycell  \\ \hline
  
    UPEC~\cite{fadiheh2020formal}
    &\graycell &\graycell &\graycell &\graycell &(\bug) \\ \hline
  
    Our Scheme
    &\secure &\secure &\bug &\bug &\bug \\ \hline
  \end{tabular}

  \caption{A summary of comparing the Baseline, LEAVE~\cite{wang2023specification}, UPEC~\cite{fadiheh2020formal}, and our scheme on verifying the sandboxing contract on 5 processors. ``\bug'' indicates valid attacks are found (``(\bug)'' indicates UPEC cannot find all possible attacks on \texttt{BOOM}), ``\secure'' indicates a proof is found, ``\timeout'' indicates a time out on the verification task {after running for 7 days}, ``\falsealert'' indicates false counterexamples are found, and a \colorbox{lightgray}{shaded} entry indicates the experiment is not conducted.}
  
% \thomas{Looking at this table, I think in the rebuttal they will likely ask us to do UPEC for SimpleOoO/Sodor. }
  \label{tab:eval:all}
\end{table}



% \begin{table}[t]
%   \setlength\tabcolsep{2pt}
%   \centering
%   \small
%   \begin{tabular}{|l|R{1.3cm}|R{1.3cm}|R{1.3cm}|R{1.3cm}|} \hline
%                   & \multicolumn{2}{c|}{\textbf{Sandboxing }}
%                   & \multicolumn{2}{c|}{\textbf{Constant-Time }}  \\ \cline{2-5}
                  
%                   & \multicolumn{1}{c|}{\textbf{Baseline}}   & \multicolumn{1}{c|}{\textbf{Our Scheme}}
%                   & \multicolumn{1}{c|}{\textbf{Baseline}}   & \multicolumn{1}{c|}{\textbf{Our Scheme}} \\ \hline\hline
                  
%   \texttt{Sodor}       &--~~~                   &\textcolor{proof}{12min}  &--~~~                   &\textcolor{proof}{11s} \\ \hline
  
%   \texttt{SimpleOoO-S} &--~~~                   &\textcolor{proof}{151min} &--~~~                   &\textcolor{proof}{37min}   \\ \hline
  
%   \texttt{SimpleOoO}   &\textcolor{bug}{1.1s}   &\textcolor{bug}{2s}       &\textcolor{bug}{0.4s}   &\textcolor{bug}{0.5s}      \\ \hline
  
%   \texttt{Ridecore}    &\textcolor{bug}{5.1min} &\textcolor{bug}{10min}    &\textcolor{bug}{1.9min} &\textcolor{bug}{2.5min}       \\ \hline

%   \end{tabular}
%   \caption{Comparing the checking time of the baseline scheme and our \name.
%   The \textcolor{bug}{red entry} indicates a bug is found and the \textcolor{proof}{green entry} indicates a proof is found.
%   ``--'' indicates time out, \rev{i.e., no result within 7 days.}}
%   \mengjia{let's be consistent to use the {\timeout} symbol}
%   \label{tab:eval:compare-processor}
% \end{table}


To better understand how our work compares to the existing techniques, we conduct experiments to compare our scheme with the baseline, LEAVE~\cite{wang2023specification}, and UPEC~\cite{fadiheh2020formal}.
\cameraready{
We also include the baseline scheme, which is directly derived from \cref{eq:4trace}.
% Although the baseline scheme is not used in any previous works, we still include it in the comparison because it directly comes from \cref{eq:4trace} and this comparison can demonstrate the benefit of reducing two ISA machines.
}
We compare the verification results on five processor designs, two secure ones (\texttt{Sodor} and \texttt{SimpleOoO-S}) and three insecure ones (\texttt{SimpleOoO}, \texttt{Ridecore}, and \texttt{BOOM}), regarding two contracts, the sandboxing contract and the constant-time programing contract.
The secure out-of-order core, noted as \texttt{SimpleOoO-S}, delays the issue time of a memory instruction until its commit time if at the time when it enters the pipeline, there is a branch before it in the ROB.

\subsubsection{Comparison Summary}
The comparison results regarding the sandboxing contract are summarized in \cref{tab:eval:all}.
% while detailed in the following subsections.
We observe similar results regarding the constant-time contract except UPEC, which does not support it.
Across all five processors, our scheme can successfully find attacks or proofs within a reasonable amount of time (concrete numbers reported later).

% \thomas{I think we should put the time in the table we say "within a reasonable amount of time" in the text.}
\begin{itemize}[leftmargin=*]
    \item Compared to the baseline, our scheme has a clear advantage in conducting unbounded proofs, where the baseline easily times out on finding proofs on secure designs.
    We observe similar performance in finding attacks between the baseline and our scheme.
    \item Similar to our scheme, LEAVE can find proof on in-order processors (\texttt{Sodor}). 
    More importantly, our scheme performs better than LEAVE on out-of-order processors.
    While LEAVE struggles with \texttt{SimpleOOO} designs, generating false counterexamples for both secure and insecure designs, our approach can find bugs and prove security of these designs.
    % it ends up generating false counterexamples for out-of-order processors (\texttt{SimpleOoO} and \texttt{SimpleOoO-S}), no matter whether the design is secure or not, while our scheme still functions well.
    \item Since UPEC is a highly customized verification scheme and requires advanced formal-method expertise to be adapted to a different design, we only show evaluation results from their paper. Even though it can successfully find attacks on \texttt{BOOM}, the approach falls short in finding all possible attacks, since it can only find attacks whose speculation source is explicitly specified by the user.
    \item \cameraready{Our scheme still cannot scale to fully proving the security of large out-of-order processors such as patched Ridecore and BOOM, nor do other schemes (UPEC can do a partial security proof for BOOM due to their customization).
    }
\end{itemize}

% LEAVE~\cite{wang2023specification} and UPEC~\cite{fadiheh2020formal} are two state-of-the-art verification schemes.
% UPEC, when evaluating \texttt{BOOM}, only finds attacks whose speculation source is explicitly specified during the verification.
% \cref{tab:eval:all} only summarizes the result for the sandboxing contract, we observe similar result while verifying the constant-time contract except UPEC, which does not support it.
% \yuheng{Maybe we do not need to mention "UPEC can also find proofs" here? We have discussions in \cref{sec:eval:compare-upec}}\mengjia{i will do it later. please review.}


We provide a detailed comparison below.

\subsubsection{Comparison to Baseline}
% \mengjia{I deleted many discussions about baseline comparison. @Yuheng, let me know if I missed anything important!}
When verifying a secure design (the first two columns), the baseline scheme times out, unable to generate an answer.
In contrast, our scheme can successfully find the proof within 151 minutes.
\cameraready{
In formal verification, a timeout indicates that the model checker is hitting an exponential wall on the model being verified, i.e., the exponential size of the reachable state space is beyond the reach of the solver.
}
This result highlights that our scheme shows much better scalability of RTL verification for software-hardware contracts compared with the baseline scheme.





\begin{comment}
\paragraph{Comparison to Baseline}
We first compare the verification performance of our \name with the baseline scheme in \cref{tab:eval:compare-processor}.
\asplosrev{Only the first three processors in \cref{tab:eval:setup} are used in this comparison.}
The first two rows show the checking time of finding a proof for two secure designs, the in-order \texttt{Sodor} core and a secure version of the \texttt{SimpleOoO} core.
The secure out-of-order core, noted as \texttt{SimpleOoO-S}, delays the issue time of a memory instruction until its commit time if at the time when it enters the pipeline, there is a branch before it in the ROB.
In both cases, the baseline scheme times out, unable to generate an answer; 
our optimized scheme can successfully find the proof within 151 minutes \footnote{\asplosrev{Note that this does not mean our scheme is over 50x faster than the baseline scheme. In formal verification, a timeout usually means the property construction is not good enough so the model checker can never solve it.}}.
This result highlights that our scheme can significantly improve the scalability of RTL verification for software-hardware contracts \asplosrev{compared with the baseline scheme.}

\mengjia{can we drop the discussion about how long it takes to detect bugs}
The next two rows compare the checking time of detecting leakage on two insecure out-of-order designs, the default \texttt{SimpleOoO} core and the \texttt{Ridecore}.
Both the baseline scheme and our optimized scheme can generate a counterexample within a reasonably short time, less than 10 minutes.
However, our scheme usually takes around 2$\times\!$ of the time compared to the baseline scheme.
The reason is that to achieve the instruction inclusion requirement (\cref{sec:main:twoproperties}), our scheme needs to check the pair of out-of-order processors for additional cycles to include inflight instructions in the \swcheck.
Interestingly, as we show in \cref{sec:eval:defense}, other aspects of our optimized scheme enable it to sometimes perform better than the baseline scheme in finding leakage.
\end{comment}

% \yuheng{I think we can cut next two paragraphs. They look less interesting to me, and stall people from reading the insteresting LEAVE and UPEC.}
% We also observe from the table that, consistently across all designs, verifying for the sandboxing contract takes longer time than for the constant-time programming contract.


% \begin{figure}[t]
%     \centering
%     \includegraphics[width=.95\columnwidth]{images/design_size.pdf}
%     \caption{The number of state bits in the three processors and the total state bits used in the baseline verification scheme (i.e., two copies of the processor and two copies of the ISA machine) and in the optimized scheme (i.e., two copies of the processor and the shadow states). The numbers on the bars of the processors are the absolute values of the bars. The numbers on the bars of the two schemes are their ratios compared to the sizes of their corresponding processors.}
%     \yuheng{Remove it and not mention the data becuase it is misleading.}
%     \label{fig:eval:design-size}
% \end{figure}

% \paragraph{Impact of Processor Complexity}
% We also want to study what aspect of processor complexity plays the primary role in affecting verification scalability.
% \cref{tab:eval:compare-processor} helps answer this question by comparing processors that employ different instruction scheduling mechanisms and have varied design sizes.
% Comparing the \texttt{Sodor} core and the \texttt{SimpleOoO-S} core, the former uses a much simpler instruction scheduling mechanism (i.e., in-order execution), while exhibiting a much larger design size in terms of number of state bits (i.e., 3$\times\!$ larger than \texttt{SimpleOoO} as shown in \cref{fig:eval:design-size}).
% Given that verifying the \texttt{SimpleOoO-S} core takes much longer time, we understand that the complexity of instruction scheduling mechanisms is a key limiting factor for RTL verification, since the model-checking tool needs to explore much more complex interactions between instructions.
% Therefore, it is critically important to scale our verification scheme for out-of-order processors.






\subsubsection{Comparison with LEAVE}
LEAVE uses an inductive approach to verify processors against software-hardware contracts.
Their key contribution is to automatically derive inductive invariants to assist deriving an inductive proof.
These invariants are supposed to capture the reachable states of the state machines being verified.
% \mengjia{here the discussion does not match the table, where we say they generate false counterexample...}
They start with a set of automatically generated or manually written candidate invariants and use a search algorithm to iteratively remove invariants that do not hold.
The expectation is that the final remaining invariants are strong enough to prove security.
Otherwise, {when insufficient invariants are used, the induction procedure will consider \textit{unreachable} states and generate false counterexamples}.
As such, they declare the verification result as \textit{UNKNOWN}.
An UNKNOWN result indicates that either the processor may be secure, but the search algorithm cannot find a good set of invariants to make the proof go through, or the processor may be insecure. 
{As a side note, LEAVE proposes invariants that consider the {instruction inclusion} and {synchronization} requirements (\cref{sec:main:twoproperties}) in a limited way for in-order processors. 
Our scheme is the first to satisfy these two requirements in a general way, supporting out-of-order and superscalar processors.}

LEAVE has only been used to verify in-order processors.
As LEAVE is open-sourced~\cite{wang2023specification-code}, we extend the evaluation of LEAVE to out-of-order processors.
% \mengjia{here is the point that we can refer to table 2}
% Specifically, we use LEAVE to verify two versions of \texttt{SimpleOOO} (Section~\ref{sec:experiment}), one insecure and one secure. 
We use the automatically generated candidate invariants described in LEAVE's paper, i.e., values in corresponding registers are equivalent in the two copies of out-of-order processors.
% \mengjia{I think since we used both Yosys and JasperGold and the bottleneck lies in the search engine, it would be better to just drop the discussion below.}
% {\color{gray}
% LEAVE and our scheme use different backends as the verification engine -- they use Yosys, and we use JasperGold.
% As JasperGold is typically stronger than Yosys, to ensure our comparison is fair,
% once LEAVE has generated its custom invariants and constructed a final verification problem, we send the problem to \textit{both} Yosys and JasperGold to try to find an unbounded proof.
% }


% We evaluated both the sandboxing and constant-time contracts. In the following, we share the observations for the sandboxing contract, these are similar to those for the constant-time contract.
When verifying an insecure version of \texttt{SimpleOoO}, our scheme finds an attack in 2 seconds.
However, we observe LEAVE fails to find a set of invariants to prove security and states that the result is UNKNOWN, i.e., LEAVE cannot tell whether the design is secure or not.
When verifying \texttt{SimpleOOO-S} (the secure version), our scheme is able to complete the proof within 2.5 hours, while LEAVE reports UNKNOWN after searching invariants for 2.1 hours.
During its execution, we observe that LEAVE's invariant-search algorithm continuously removes invariants from the candidate sets until there are none left.
The reason is that the automatically generated candidate invariants are insufficient to cover reachable states for even simple out-of-order processors.
In these cases, LEAVE will require additional effort to improve the invariant generation algorithm or ask the user to manually write invariants, both posing open research challenges.

% \mengjia{I moved the summary to the beginning of this subsection. I added one sentence to say they need manual effort at the end of the last paragraph. Check.}
% {\color{gray}
% \paragraph{Summary}
% % \mengjia{maybe we should move the summary ahead...}
% The experiment results above show that our scheme performs better than LEAVE on out-of-order processors.
% While LEAVE struggles with \texttt{SimpleOOO} designs, our approach can both find bugs and prove security of such designs.
% We would like to further highlight that our scheme is automatic once the shadow logic is in place, while LEAVE requires additional effort to improve the invariant generation algorithm or ask the user to manually write invariants to achieve the level of usability of our scheme.
% \yuheng{We could mention our new introduction's idea: invariants must be done by experts.}
% }








\subsubsection{Comparison with UPEC}
% \label{sec:eval:compare-upec}
UPEC uses an inductive verification approach, assisted with substantial manual invariants {by formal-method experts}, to verify complex out-of-order processors including \texttt{BOOM}.
As discussed in \cref{sec:intro}, UPEC's unbounded proof of secure designs is closely coupled with the defense scheme to be verified. 
% \qt{We use the original word in the UPEC paper to describe the defense they verified.}
{Specifically, they verified a defense scheme that prevents speculative load instructions to execute before all preceding branch instructions in the ROB are resolved.
With such a defense, under the sandboxing contract, the secret data never propagates to any other gates in the design.
Their induction procedure finds that this invariant holds for arbitrary initial states and they can complete an unbounded proof by proving an induction step that only involves 1 cycle of symbolic execution.
% that secret data does not reach new gates, an invariant taking any number of steps,  and take a single step to realize the invariant 
% enter the processor pipeline under the sandboxing contract.
% This fact plays a significantly important role in their unbounded proof as it greatly lowers the difficulty of induction.
}
% \mengjia{is this statement correct?}
However, this invariant does not hold for most defenses proposed in the computer architecture community where speculative states do spread in a complex manner inside the processor, as with DoM~\cite{sakalis2019efficient}, STT~\cite{yu2019speculative}, and others.
% As a result, if using UPEC to verify these defense schemes, the user needs to redo the verification and spend hours figuring out a different set of invariants, which poses significant challenges.


In addition, we find their approach achieves high scalability at the cost of losing generality and completeness.
Specifically, UPEC's verification procedure requires the user to provide information on \textit{the source of speculation} in the processor.
Their open-source prototype uses branch misprediction as the sole source of speculation, and their manual invariants were developed based on this assumption.


% In evaluating our scheme against UPEC, we focus on comparing i) the completeness of the verification scheme, and ii) whether the scheme can work on complex out-of-order cores, such as \texttt{BOOM}~\cite{zhaosonicboom}.



To compare our scheme with UPEC, we implemented our \name on \texttt{BOOM} for both sandboxing and constant-time contracts (UPEC only handles the sandboxing contract).
We use the \texttt{SmallBOOM} configuration and directly use the data cache and instruction cache as the memory with the virtual memory module turned off.
Both cache sizes are configured to 256 bytes.



Our experiment results show that our scheme can find multiple attacks on \texttt{BOOM} exploiting different speculation sources.
First, we find an attack for the sandboxing contract in 120 minutes and a similar attack for the constant-time contract in 36.6 minutes.
In these two attacks, mis-speculation is triggered by exceptions due to memory address misalignment:
\begin{minipage}{\columnwidth}
\begin{center}
\begin{tabular}{c}
\begin{lstlisting}[style=mystyle, language=mylang, label={lst:future}]
lui r6, 65536 //set addr to a legal range
lhu r14, 1221(r6) //mis-alignment in addr
lh r0, r14    //use secret as load addr
\end{lstlisting}
\end{tabular}
\end{center}
\end{minipage}
In the above code snippet, the second instruction loads the secret into \texttt{r14} and the third instruction uses the secret as memory address, thus violating the \hwcheck.
Since the second instruction triggers an exception due to address misalignment, the second and third instructions will not be committed, and thus will satisfy the \swcheck. 
Note that, these attacks were not reported by UPEC on \texttt{BOOM} as they only consider branch misprediction as the speculation source. 
% \thomas{Yuheng, this is where we could inject, if we are sure, that this bug would also exist in their "secure" version}\yuheng{Check the paragraph below. I start to agree Mengjia by not include it since it is too strong statement.}

% \yuheng{
% \mengjia{I hope we can be cautious to make this statement. Maybe we drop it because we do not have the actual results?}
% Regarding finding proofs, UPEC can provide a security proof on a modified version of \texttt{BOOM} where load instructions are delayed until all preceding branch instructions are resolved.
% However, their proof only consider branch miprediction as the speculation source and misses the attack shown above, where no branch instruction is used.
% It would be useful to extend their security proof whenever new speculation sources are found to be vulnerable.
% }



Second, we can continue to search for other attacks following the standard practice in formal verification.
We add an assumption to exclude the first attack that we found.
The added assumption ensures the input program does not involve memory accesses using misaligned addresses.
Running the verification procedure for the sandboxing contract leads us to the discovery of a new attack exploiting exceptions due to illegal memory accesses.
The verification for the constant-time contract generates an attack exploiting branch misprediction.
The former case takes 8.7 hours, and the latter case takes 1.4 hours.

Finally, we further continue the experiments to exclude the two attacks.
The verification tasks time out after 24 hours.


% \paragraph{Summary}
% \mengjia{tune down this statement, since we already said the problem is they need new invariants...}
The above experiments show that our scheme can scale to find attacks on complex out-of-order cores, such as \texttt{BOOM}.
In addition, 
% we show that the attack-agnostic nature\yuheng{Are we still using the word "attack-agnostic"?} of
our scheme finds unknown attacks on processors without specifying the source of speculation and ends up finding multiple attacks that UPEC was unable to find.
% Indeed, the current version of UPEC does not offer completeness since it narrowly assumes the branch mis-prediction as the only source of speculation.





% \asplosrev{
% Regarding finding proofs, UPEC can provide a security proof for one specific source of mis-speculation on a secure version of \texttt{BOOM} while our security proof cannot scale to such large processors.
% However, it is important to note the following facts: 1) UPEC proves a simple defense (i.e. no speculative load is issued) which does not require complex manual invariants to prove. 2) Our scheme is trying to find a proof that covers all possible sources of mis-speculation, which is a much more challenging goal.
% In practice, when the source of mis-speculation is unknown, our attack-agnostic approach is much more general than UPEC's attack-specific approach.
% Intrinsically UPEC cannot be extended to match the attack-agnostic capability of our scheme since there is no known comprehensive list of sources of mis-speculation that they could go through one by one.
% \yuheng{Wait, given boom indeed has other source of speculation, if we run their defense, we can easily find an attack.}
% \yuheng{I really want to add "the proof provided by UPEC targets a relatively simple defense where secret will not be speculative accessed due to branch mis-prediction. UPEC also assumes that secret will not be speculative accessed due to other source of speculation, and only considers the sandboxing contract where secret will not be non-speculatively accessed, either. It is unclear how easy it is to construct manual invarants when applying UPEC to general proof tasks under different assumptions.", but it is too aggressive.}
% }


% {\color{gray}
% \yuheng{Following gray text is the older version of the paragraph above in CCS submission.}
% While UPEC does provide a proof for one specific source of mis-speculation and we are unable to provide an attack-agnostic proof that covers all sources of mis-speculation, it is important to note the difference in the goals of the two approaches.
% Our attack-agnostic approach is much more general than UPEC's attack-specific goal and is what is needed in practice when the attack source is unknown.
% It is unclear how UPEC could be extended to match the attack-agnostic capability of our scheme.
% Potentially, they could attempt their attack-specific proof methodology individually to other sources of mis-speculation.
% First, it is unclear if their proofs would be complete for those sources.\yuheng{What does this mean? When UPEC specify a source, why the proof for that source could be incomplete?}
% Second, there is no known comprehensive list of sources of mis-speculation that they could go through.
% Thus, this attack-specific approach is intrinsically non-extensible to be attack agnostic.
% }

% {\color{gray}
% Regarding finding proofs, UPEC can provide a security proof for a secure version of \texttt{BOOM} while our security proof cannot scale to such large processors.
% One important reason is that while UPEC applies an assumption that branch mis-prediction is the only source of speculation, it is hard for our scheme to prove this assumption.
% % Specifically, it targets a specific source of mis-speculation (i.e., branch mis-prediction), targets a simple defense scheme where no data will be loaded when it follows an uncommitted branch, and targets a specific contract where secret will never be loaded non-speculatively.
% % Specifically, it targets a simple defense scheme where no data will be speculative loaded and targets a specific contract where secret will never be non-speculatively loaded.
% % This task makes it very easy to manually write invariants for the system.
% }






\subsection{Impact of Defense Mechanisms}
\label{sec:eval:defense}

\begin{table}[t]
  \setlength\tabcolsep{2pt}
  \small
  \centering
  
  % \begin{tabular}{|l|R{1.2cm}|R{1.2cm}|R{1.2cm}|R{1.2cm}|} \hline
  %                 & \multicolumn{2}{c|}{\textbf{Sandboxing }}
  %                 & \multicolumn{2}{c|}{\textbf{Constant-Time }}  \\ \cline{2-5}
                  
  %                 & \multicolumn{1}{c|}{\textbf{Baseline}}   & \multicolumn{1}{c|}{\textbf{Our Scheme}}
  %                 & \multicolumn{1}{c|}{\textbf{Baseline}}   & \multicolumn{1}{c|}{\textbf{Our Scheme}} \\ \hline\hline
                  
  % $\mathsf{NoFwd_{futuristic}}$ &\timeout &\textcolor{proof}{66min}  &\textcolor{bug}{0.1s}  &\textcolor{bug}{0.4s} \\ \hline
  
  % $\mathsf{NoFwd_{spectre}}$    &\timeout &\textcolor{proof}{45h}    &\textcolor{bug}{1.1s}  &\textcolor{bug}{0.1s}   \\ \hline
  
  % $\mathsf{Delay_{futuristic}}$ &\timeout &\textcolor{proof}{21min}  &\timeout               &\textcolor{proof}{10min}      \\ \hline
  
  % $\mathsf{Delay_{spectre}}$    &\timeout &\textcolor{proof}{151min} &\timeout               &\textcolor{proof}{37min}   \\ \hline
  
  % $\mathsf{DoM_{spectre}}$      &\textcolor{bug}{31min{\color{black}\footnotemark[4]}}
  %                                         &\textcolor{bug}{6.5min{\color{black}\footnotemark[4]}}
  %                                                                    &\textcolor{bug}{36min} &\textcolor{bug}{5.9min}       \\ \hline

  % \end{tabular}
  
  \begin{tabular}{|l|R{2.2cm}|R{2.2cm}|} \hline
                  & \multicolumn{1}{c|}{\textbf{Sandboxing}} & \multicolumn{1}{c|}{\textbf{Constant-Time}}  \\ \hline\hline
                  
  $\mathsf{NoFwd_{futuristic}}$ &\textcolor{proof}{66min}  &\textcolor{bug}{0.4s}     \\ \hline
  
  $\mathsf{NoFwd_{spectre}}$    &\textcolor{proof}{45h}    &\textcolor{bug}{0.1s}     \\ \hline
  
  $\mathsf{Delay_{futuristic}}$ &\textcolor{proof}{21min}  &\textcolor{proof}{10min}  \\ \hline
  
  $\mathsf{Delay_{spectre}}$    &\textcolor{proof}{151min} &\textcolor{proof}{37min}  \\ \hline
  
  $\mathsf{DoM_{spectre}}$      &\textcolor{bug}{6.5min{\color{black}\footnotemark[2]}}
                                                           &\textcolor{bug}{5.9min}   \\ \hline

  \end{tabular}
  
  
  \caption{Verification time using our scheme on \texttt{SimpleOoO} augmented with different defenses. The \textcolor{bug}{red entry} indicates an attack is found and the \textcolor{proof}{green entry} indicates a proof is found.}
  % We use the same annotation as \cref{tab:eval:all}.}
  \label{tab:eval:compare-defense}
\end{table}

\footnotetext[2]{These two attacks are found using an 8-entry ROB instead of the default 4-entry ROB because these attacks require more concurrent instructions.}


{We now study how various factors can affect the verification time of our scheme.
We start with the influence of defense mechanisms on verification time.}
% We next study how different defense mechanisms affect verification time.
We extend the \texttt{SimpleOoO} core with five microarchitecture defenses from the literature~\cite{sakalis2019efficient,yu2019speculative,weisse2019nda}.
Note that we can directly reuse the shadow logic we developed for \texttt{SimpleOoO}, highlighting the reusability of our approach.
% \yuheng{We can still use the same shadow logic!}
We note this is the \textit{first} time for many of these defense proposals to be evaluated as RTL designs, in contrast to high-level abstract models~\cite{guarnieri2021hardware, yang2023pensieve, trippel2018checkmate} or via gem5 simulation~\cite{gem5}.


\paragraph{Defenses}
The following two mechanisms share similarities with the defenses described in STT~\cite{yu2019speculative} and NDA~\cite{weisse2019nda}.
% They target the sandboxing contract.
\begin{itemize}[leftmargin=*]
  \item $\mathsf{NoFwd_{futuristic}}$: Do not forward the data of a load instruction to younger instructions until its commit time.
  \item $\mathsf{NoFwd_{spectre}}$: Do not forward the data of a load instruction to younger instructions until its commit time, if 
  when the load enters the pipeline, there is a branch before the load in the ROB.
\end{itemize}
The difference between the two mechanisms is that $\mathsf{NoFwd_{futuristic}}$ considers all possible sources of speculation, while $\mathsf{NoFwd_{spectre}}$ only considers branch prediction as the source of speculation.


The next three defenses work by delaying load instructions at different points in their lifetime.
\begin{itemize}[leftmargin=*]
  \item $\mathsf{Delay_{futuristic}}$: Delay the issue time of a memory instruction until its commit time.
  \item $\mathsf{Delay_{spectre}}$: Delay the issue time of a memory instruction until its commit time, if at the time when it enters the pipeline, there is a branch before it in the ROB.
  It is noted as \texttt{SimpleOoO-S} in \cref{sec:eval:compare}.
  \item $\mathsf{DoM_{spectre}}$: This models a simplified version of the Delay-on-Miss defense~\cite{sakalis2019efficient}.
  It always speculatively issues a load instruction. If the load hits the L1 cache, return the data to the core and proceed.
  If the load misses the L1 cache, delay the load from being sent to the main memory if at the time when the load enters the pipeline, there is a branch before the load in the ROB.
  We model a cache with a single cache entry with a 1-cycle hit and a 3-cycle miss.
\end{itemize}
$\mathsf{Delay_{futuristic}}$ and $\mathsf{Delay_{spectre}}$ are secure on \texttt{SimpleOoO} for both the sandboxing contract and constant-time contract, while $\mathsf{DoM_{spectre}}$ is not secure.
The vulnerability of $\mathsf{DoM_{spectre}}$ has been discovered in prior work~\cite{behnia2021speculative,fustos2020spectrerewind}.


\paragraph{Evaluation Results}
\cref{tab:eval:compare-defense} compares the checking time of verifying the five defenses.
For all the cases where we are supposed to find a proof, i.e., when the designs are secure, our scheme can find a proof \rev{for all of them within 45 hours, with most completing in about an hour.}
We note in all the cases, the baseline scheme times out (not shown in the table). 
% Further, our scheme also performs better than the baseline scheme in bug-finding when verifying $\mathsf{DoM_{spectre}}$.


Comparing the checking time for different defenses, we observe that defenses have a non-trivial impact on checking time.
First, it takes much longer to find the proof in secure designs (above 10 minutes) than to find an attack in insecure designs (below 10 minutes).
% This matches our observation in \cref{sec:eval:compare}.
Second, it takes less time to find a proof on a relatively more conservative defense mechanism.
Comparing the pair of \texttt{NoFwd} and the pair of \texttt{Delay} defenses, the futuristic version takes much less time to verify.






\subsection{Impact of Structure Sizes}
\label{sec:eval:size}

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{images/performance.pdf}
    \caption{Verification time when varying the size of the register file, data memory, and re-order buffer. }
    \label{fig:eval:size-time}
\end{figure}

Finally, we study how structure sizes of re-order buffer, register file, and memory affect  verification time.
\cref{fig:eval:size-time} shows the checking time for verifying $\mathsf{NoFwd_{futuristic}}$ defense for the sandboxing contract and $\mathsf{Delay_{spectre}}$ defense for the constant-time contract.
The default configuration consistently uses 4 entries for the register file, ROB, and data memory.
The three lines in the plot are derived by changing one of the three structures and keeping the other two unchanged.


Overall, the size of the register file has negligible impact on verification time.
The size of data memory has a limited impact on proving the sandboxing contract but has a larger impact on proving the constant-time contract.
Note that the size of ROB has a significant impact (y-axis is log scale).
When we increase the ROB size, the verification time increases exponentially.
The ROB size determines the number of inflight instructions, and the space of possible interactions between instructions grows quickly with ROB size, taking a much longer time to check.




%=======================================================
%========== MOVE a 2-Column Figure here BEGIN ==========
%=======================================================

% \begin{table*}[t]
% \small
% \centering
% % \resizebox{2\columnwidth}{!} {
% \color{black}\begin{tabular}[\aboverulesep=0ex, \belowrulesep=0ex]{@{\extracolsep{0pt}}|c|c|c|c|c|c|c|c|}
% \hline
% &Target Specu- & Support & No Manual  &No Assumed &Scale to & Unbounded &\multirow{2}{*}{Case Study}  \\
% &lation Attacks & RTL &Invariant & Attack Pattern &OoO Processor &Check & \\
% \hline\hline
% Iodine~\cite{gleissenthall2019iodine} & \cross & \tick &\tick &\tick &  \cross & \tick &
% \multirow{3}{*}{\shortstack{In-order processor,\\ arithmetic unit,\\ or crypto accelerator}}  \\ 
% % \hline
% \cline{1-7}

% Xenon~\cite{v2021solver} & \cross & \tick & \tick & \tick & \cross   &  \tick & \\
% % % \multirow{2}{*}{Only support in-order processors or acclerators.} 
% % \\
% % & & & & & &  \\
% \cline{1-7}
% Knox~\cite{athalye2022verifying} & \cross & \tick & \cross& \tick& \cross& \tick & \\

% \hline\hline
% CheckMate~\cite{trippel2018checkmate} & \tick & \cross &\tick &\cross & \tick & \cross & \multirow{3}{*}{Abstract OoO model}  \\
% \cline{1-7}
% Guarnieri et al.~\cite{guarnieri2021hardware} & \tick & \cross  &\tick & \tick & \tick & \tick &   \\ 
% \cline{1-7}
% Pensieve~\cite{yang2023pensieve} & \tick & \cross & \tick & \tick & \tick & \cross &  \\
% \hline\hline
% \multirow{2}{*}{UPEC~\cite{fadiheh2020formal}} & \multirow{2}{*}{\tick} & \multirow{2}{*}{\tick} & \multirow{2}{*}{\cross} & \multirow{2}{*}{\cross} & \multirow{2}{*}{\tick} & \multirow{2}{*}{\tick} &In-order processor   \\
% & & & & & & & Complex OoO processor   \\ 
% \hline
% LEAVE~\cite{wang2023specification} & \tick & \tick  &\cross & \tick & \cross & \tick & In-order processor  \\ 
% \hline
% \multirow{2}{*}{Our Scheme} & \multirow{2}{*}{\tick} & \multirow{2}{*}{\tick} & \multirow{2}{*}{\tick} & \multirow{2}{*}{\tick} & \multirow{2}{*}{\tick} & \multirow{2}{*}{\tick} &In-order processor,   \\
% & & & & & & & Complex OoO processor   \\ 
% \hline
% % & & & & &\multirow{2}{*}{In-order processor} &  \multirow{3}{*}{\parbox{5.2cm}{While it is the only one to handle OoO processors without assuming any attack patterns, it cannot prove practical-size OoO processors.}} \\
% % \multirow{1}{*}{Our Scheme}&\multirow{1}{*}{\tick} &\multirow{1}{*}{\tick} &\multirow{1}{*}{\tick} & \multirow{1}{*}{\tick}& \multirow{2}{*}{Simple OoO processor} & \\
% % & & & & & & 
% %  \\
% % \multirow{1}{*}{Our Scheme} & \multirow{1}{*}{\tick} & \multirow{1}{*}{\tick} & \multirow{1}{*}{\tick} & \multirow{1}{*}{\tick} & \multirow{1}{*}{In-Order Processor} &   \\ 
% % & & & & & \multirow{1}{*}{Simple OoO Processor} & \\
% \end{tabular}
% % }
% \caption{\rev{Comparison between different hardware verification schemes.}\yuheng{TODO: remove it}}
% \label{table:compare_scheme}
% \end{table*}

%=====================================================
%========== MOVE a 2-Column Figure here END ==========
%=====================================================




==> ykfkyxzqqtggdstybhwmzfvqmnwcsnwh/ExperimentSetup.tex <==
\section{Experiment Setup}
\label{sec:experiment}

\begin{table}[t]
  \setlength\tabcolsep{4pt}
  \small
  \centering
  \begin{tabular}{|c|L{6.7cm}|} \hline
  % Processor & Configuration \\ \hline\hline
  \multirow{6}{*}{\begin{tabular}{@{}c@{}}\texttt{Sodor}\\\cite{website:sodor}\end{tabular}}
    &Open-source in-order processor \\ %\cline{2-4}
    &ISA: the full suite of RV32I \\
    &Configuration: 2-stage pipeline, 1-cycle memory \\
    & Code size: 700 lines of Chisel (2,700 lines of Verilog)\\
    & \qquad\qquad\space $\sim$90 lines of Verilog for shadow logic\\
    & \qquad\qquad\space $\sim$3h manual effort for shadow logic\\
    % & \asplosrev{Design size: 1.4K bits, 27K gates }\\
    % & \asplosrev{\qquad\qquad\quad\space 8 bits, 2.0K gates for shadow logic}\\
    
  \hline
  
  \multirow{7}{*}{\begin{tabular}{@{}c@{}}\texttt{Simple} \\\texttt{OoO}\end{tabular}}
    &Our in-house minimal out-of-order processor \\
    &ISA: 4 customized insts (loadimm, ALU, load, branch) \\
    &Configuration: 4-stage pipeline,  4-entry ROB  \\
    &\qquad\qquad\qquad\space commit bandwidth is 1 inst/cycle \\
    % &\qquad\quad 1-cycle multiplier \\
    % &\qquad\quad 1-cycle memory \\
    % & Out-of-order scheme: all in-flight data in the ROB \\
    & Code size: 1,000 lines of Verilog\\
    & \qquad\qquad\space $\sim$100 lines of Verilog for shadow logic\\
    & \qquad\qquad\space $\sim$5h manual effort for shadow logic\\
    % & \asplosrev{Design size: 450 bits, 5.4K gates}\\
    % & \asplosrev{\qquad\qquad\quad\space 12 bits, 740 gates for shadow logic}\\
  \hline
  
  \multirow{7}{*}{\begin{tabular}{@{}c@{}}\texttt{Ride}\\\texttt{core}\\\cite{website:ridecore}\end{tabular}} 
    &Open-source out-of-order processor \\
    &ISA: 35 instructions in RV32IM \\
    &Configuration: 6-stage pipeline, 8-entry ROB \\
    &\qquad\qquad\qquad\space commit bandwidth is 2 inst/cycle\\
    % &\qquad\quad 4-cycle non-pipelined multiplier \\
    % &\qquad\quad 2-cycle pipelined memory \\
    % &Out-of-order scheme: full-fledged support with \\
    % &register renaming using unified physical register \\
    % &file and instruction scheduling information distributed in ROB and per-FU reservation stations\\
    & Code size: 8,100 lines of Verilog\\
    & \qquad\qquad\space $\sim$400 lines of Verilog for shadow logic\\
    & \qquad\qquad\space $\sim$10h manual effort for shadow logic\\
    % & \asplosrev{Design size: 10K bits, 123K gates}\\
    % & \asplosrev{\qquad\qquad\quad\space 350 bits, 9.9K gates for shadow logic}\\
  \hline
  \multirow{7}{*}{\begin{tabular}{@{}c@{}}\texttt{BOOM}\\\cite{zhaosonicboom}\end{tabular}} 
    &Open-source out-of-order processor \\
    &ISA: RV64GC \\
    &Configuration: SmallBoomConfig \\
    &\qquad\qquad\qquad\space 32-entry ROB \\
    &\qquad\qquad\qquad\space commit bandwidth is 1 inst/cycle \\
    % &\qquad\quad independent integer/floating point pipelines \\
    & Code size: 19k lines of Chisel (136k lines of Verilog)\\
    & \qquad\qquad\space $\sim$240 lines of Verilog for shadow logic\\
    & \qquad\qquad\space $\sim$8h manual effort for shadow logic\\
    \hline
  \end{tabular}
  \caption{Detailed processor configurations.}
  \label{tab:eval:setup}
\end{table}




% We evaluate our scheme and the baseline verification scheme over three processors, including one in-order processor and two out-of-order processors, with varied complexity.
% We list their detailed configurations in \cref{tab:eval:setup}.
% The default configuration uses a 4-entry data memory, a 16-entry instruction memory, and a 4-entry ROB (in out-of-order processors).
% The data memory and instruction memory are distinct in all processors, so the instruction memory cannot be overwritten by memory write instructions.
% \texttt{Sodor} and \texttt{SimpleOoO} are configured to use a simple 4-entry register file, and \texttt{Ridecore} uses a more realistic 32-entry register file.
% We will show how these configurations affect verification time in \cref{sec:eval:size}.


We implement shadow logic for verifying the sandboxing contract and the constant-time contract (\cref{sec:background:contract}) on four processors as shown in \cref{tab:eval:setup}.
Other than the three open-source processors, SimpleOoO is a toy out-of-order processor developed by us that has the basic out-of-order execution behaviors, and we augment it with different defense mechanisms.
In \cref{tab:eval:setup}, we compare the code size for each processor that we verified and the code size and manual effort for the shadow logic.
Note that although BOOM is much larger than Ridecore, its shadow logic is less complex because it only commits one instruction every cycle while Ridecore is a superscalar processor that can commits two instructions per cycle.
This shows that the complexity of our shadow logic does not necessarily grow as the processor gets larger.
% \asplosrev{These four processors will be used our experimental evaluation to compare our scheme with the baseline scheme or related works.}
% For single-commit processors, the shadow logic takes around 100 LoC (line of code), and for superscalar processors, such as \texttt{Ridecore}, the shadow logic is more complex, taking around 400 LoC.
% Overall, the shadow logic is relatively simple compared to the core, and can be carefully reviewed for correctness.


% \qt{We've decided to remove Fig.5 and only mention the size comparison when comparing with the baseline.}
% \cref{fig:eval:design-size} compares the sizes of the three processors, the baseline verification scheme, and the optimized scheme.
% Overall, the number of the state bits used in the optimized scheme is around twice the size of the processor with 1-3\% overhead due to additional shadow states.
% This is on average 31\% smaller than the size of the baseline scheme.
% We also observe a similar decrease in the number of logic gates in the optimized scheme.
% These align with our intuition to reduce the total size of state machines involved in verification.


Here is the overview of our verification workflow:
\begin{enumerate}[leftmargin=*]
    \item[1.] Implement the \name that extracts and compares the information from two out-of-order processors.
    The design under verification (DUV) includes both processors and the shadow logic.
    \item[2.] Initialize the instruction memories in two out-of-order processors to have symbolic values, so all possible programs will be explored in model checking.
    \item[3.] Write assumptions (constraints) including: (1) the two out-of-order processors have the same initial state except that the secret in memory has different initial values; (2) the \swcheck must always hold.
    \item[4.] Model check the DUV with the above assumptions and the assertion that \hwcheck holds.
\end{enumerate}







We perform verification tasks using the commercial model checking tool, JasperGold~\cite{website:jaspergold}.
We use its \texttt{Mp} and \texttt{AM} solving engines to find proofs, and use the \texttt{Ht} engine to detect leakage.
The performance results were obtained on a server with an Intel Xeon E5-4610 processor running at 2.4 GHz.
We set 7 days as the time-out period for each verification task.




% \mengjia{copied from intro... }

% \begin{itemize}[leftmargin=*]

% \item
% Second, our verification scheme needs to be \textit{attack-agnostic}, which means we want to \textit{avoid} using prior knowledge of attack patterns and guiding the verification to only search for specific templated attack patterns while leaving out other potential attack patterns.
% Though effective in guaranteeing the absence of known attacks like Spectre V1~\cite{Kocher2018spectre}, such approaches cannot be used to tackle the extensive security verification that we focus on in this paper.
% For example, considering branch misprediction as the only source of speculation can easily miss vulnerabilities due to other speculation sources, such as store-to-load forwarding.'
% \mengjia{we can mention this in the related work/comparison, but I do not think it is a strong claim...}

% \item 
% Finally, we expect our verification scheme to be used for both bug-finding, i.e., identifying attacks on insecure designs, and deriving security proofs
% for secure designs.
% In contrast, often existing work either only focuses on finding bugs, e.g., Pensieve~\cite{yang2023pensieve} and CheckMate~\cite{trippel2018checkmate}, or on finding proofs, e.g., LEAVE~\cite{wang2023specification}.
% \mengjia{I think we can mention this later.. but it is more like something given by JasperGold, not something we achieve...}

% \end{itemize}




==> ykfkyxzqqtggdstybhwmzfvqmnwcsnwh/Formulation.tex <==
\cameraready{

\section{Formulation}
\label{sec:formal}


\subsection{Property to Prove}

Recall we have the following formula in the background section to define contracts:
\[
\begin{aligned}
&\forall P, M_{pub}, M_{sec}, M_{sec}', \\
\text{\textbf{if}}\quad & O_{ISA}(P,M_{pub},M_{sec})=O_{ISA}(P,M_{pub},M_{sec}') \\
\text{\textbf{then}}\quad & O_{\mu Arch}(P, M_{pub},M_{sec}) = O_{\mu Arch}(P, M_{pub},M_{sec}') & 
\end{aligned}
\]
% Be aware that $O_{ISA}$ and $O_{\mu Arch}$ are configurable based on:
% \begin{itemize}
%     \item How $ISA$ and $\mu Arch$ simulate the program.
%     \item How they extract observation.
% \end{itemize}
% We will start to think a little more precisely on the first item, ``how $ISA$ and $\mu Arch$ simulate the program''.
% What is the length of the simulations? (For infinite cycles? Until the program terminates?)
% Should $ISA$ and $\mu Arch$ be simulated for the same number of cycles?
% We will remove these ambiguities in the following definition.

We will add a notion of ``cycle'' to this original version.
First, we use notation $O^n_{ISA}$ and $O^n_{\mu Arch}$ to represent ``simulate $ISA$ (or $\mu Arch$) for $n$ cycles''.
Second, we define a function to relate the number of cycle being simulated in $ISA$ and $\mu Arch$.
The function, $\texttt{F-BTC}_{\mu Arch}(P,M_{pub},M_{sec}, n)$, returns the number of fetched bound-to-commit instructions when simulating the $\mu Arch$ for $n$ cycles.
We will use this returned value as the number of cycles to be simulated in the $ISA$.
With these, the property we will prove with our contract shadow logic is:\yuheng{Just keep nBTC and remove F-BTC. And explain how we decide nBTC with text.}
\[
\begin{aligned}
&\forall P, M_{pub}, M_{sec}, M_{sec}', n, \\
% \text{\textbf{let}}\quad & n_{BTC} = Max(\texttt{F-BTC}_{\mu Arch}(P,M_{pub},M_{sec}, n),
\texttt{F-BTC}_{\mu Arch}(P,M_{pub},M_{sec}', n)) \\
\text{\textbf{if}}\quad & O^{n_{BTC}}_{ISA}(P,M_{pub},M_{sec})=O^{n_{BTC}}_{ISA}(P,M_{pub},M_{sec}') \\
\text{\textbf{then}}\quad & O^n_{\mu Arch}(P, M_{pub},M_{sec}) = O^n_{\mu Arch}(P, M_{pub},M_{sec}') & 
\end{aligned}
\]

% We use notation $O^n_{ISA}$ and $O^n_{\mu Arch}$ to represent ``simulate $ISA$ (or $\mu Arch$) by fetching $n$ bound-to-commit instructions and extract the observation''.
% The ``fetching $n$ bound-to-commit instructions'' is subtly defined to align with our ``instruction inclusion requirement''.
% Its subtlety lies in two aspects:
% \begin{itemize}
%     \item For all fetched instructions, only some of them are bound to commit. Others will be squashed.
%     \item For all fetched bound-to-commit instructions, when the simulation finishes, only some of them have been committed. Others will be in the ROB.
% \end{itemize}
% In short, when the simulation finishes, ``committed instructions'' $\subseteq$ ``fetched bound-to-commit instructions'' $\subseteq$ ``fetched instructions''.
% For $ISA$, these 3 sets are equal.
% For $\mu Arch$, based on the implementation, e.g., ROB size, prediction correctness, the 3 sets can be different.
% For now, we assume a memory system with constant 1-cycle read/write latency (because I am not sure how cache pre-fetch will affect our definition).
% \yuheng{TODO: there is one problem about this formulation that for $\mu Arch$, ``fetching $n$ bound-to-commit instructions'' does not constrain how many cycles it will simulate. Then, $O^n_{\mu Arch}$ can have undetermined cycles...}

Compared with the original formula, when $n$ is bounded, this new one might miss some contract assumption constraints and give an invalid attack program.
We say this attack program is invalid because if we do the assumption constrain for an unbounded number of cycles, it will not pass.
When this new one is proved with unbounded $n$, it is equivalent to the original one.

\subsection{Discuss Possible Invalid Attacks}

It would be useful to discuss the source of an invalid attack program when $n$ is bounded.
We will show this is rare and we did not observe them during our experiments.
There are two reasons why we miss some constraints:
\begin{itemize}
    \item Fetched instructions that will be squashed (i.e., not bound-to-commit).
    \item Instruction being touched by the system (e.g., prefetched by cache) while not fetched into the pipeline. (In our experiments, we assume a memory system with constant 1-cycle read/write latency (because I am not sure how cache pre-fetch will affect our definition).)
\end{itemize}

% \yuheng{Work In Progress. Don't Read.}




\subsection{Contract Shadow Logic Prove the Property with Two Assumptions}

\yuheng{I am still ``describing'' our two assumptions and have not used formulas to represent our two assumptions. But maybe this is enough?}

The key reason that motivates us to design the contract shadow logic is that the $ISA$ observation can be extracted from the $\mu Arch$ model.
This can be formalized as the first assumption we use: \textbf{the $\mu Arch$ model correctly implements the $ISA$.}
There are many facts that can be derived from ``correctly implemented''.
For our convenience, we derive a fact from this assumption that for each bound-to-commit instruction, there exist signals in the $\mu Arch$ model at a certain cycle that give the correct operands (either read from register file or immediate value decoded from instruction), the computed memory address (if it is a load/store instruction), and the computed write back data.
We rely on existing functionality verification to give us this assumption.

Our second assumption is that \textbf{the shadow logic is implemented correctly.}
We will now explain the definition of correctness.
Given the first assumption, we know those signals for each instruction exist at a certain line of code and at a certain cycle.
However, we have to dig into the implementation to extract these signals correctly.
Thus, we define the correctness of shadow logic as ``extract the correct signals for the first $n_{BTC}$ instructions from the $\mu Arch$ model and compare the signals when the secret changes.
To achieve this correctness, designers should locate the correct signals at the correct cycle, and follow our description of achieving the instruction inclusion requirement and synchronization requirement.

}

==> ykfkyxzqqtggdstybhwmzfvqmnwcsnwh/Implementation.tex <==
\section{Implementation Details}
\label{sec:implementation}
In this section, we introduce several details that are not mentioned in the previous section and discuss how to handle superscalar processors using our scheme.
\subsection{Bookkeeping ISA Level Information}
In our advanced verification scheme, the ISA level comparison is only done for instructions at commit stage.
However, it is possible that some ISA level information are discarded immediately after being used and will not be available at commit stage.
For example, multiplication operands needed by the constant-time programming contract may only be available before they enter the multiplier.
Thus, to avoid such cases, we have to extend the ROB to keep all the necessary ISA level information until commit stage.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.3\textwidth]{images/ROB_mul.png}
    \caption{Extended ROB to Keep \texttt{mul} Information}
    \label{fig:ROB_mul}
\end{figure}

As shown in Figure~\ref{fig:ROB_mul}, we add two columns to the ROB of each out-of-order processor.
One column tells whether an instruction is a \texttt{mul} instruction and the other colums records the two operands of multiplication.
When an \texttt{mul} instruction enters ROB, the $is\_mul$ column gets a corresponding value, and when an \texttt{mul} instruction enters the multiplier, its two operands are stored into the $mul\_opr$ column in ROB.
In the figure, $inst_1$ is not a multiplication instruction, and thus synchronized comparison will not compare the $mul\_opr$ for $inst_1$ in two out-of-order processors.
Because $inst_2$ is a multiplication instruction, the $mul\_opr$ of $inst_2$ will be compared in the synchronized comparison.


\subsection{Finishing Logic Optimization}
As we introduced earlier, the finishing module will store all the inflight instructions of two out-of-order processors when a microarchitectural deviation is observed.
Intuitively, we can store all the ROB indices of all inflight instructions and wait for all of them to be committed and compared.
To further reduce the overhead, we only store the index of the youngest instruction in the ROB.
Then, if the ROB commits an instruction with this index, we know that it is time to finish the checking.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{images/sqaush.png}
    \caption{Update the Youngest Instruction After Squashing}
    \label{fig:squash}
\end{figure}

However, if this youngest instruction gets squashed and not committed, we have to update the stored index to the youngest instruction that is not squashed.
For example, in Figure~\ref{fig:squash}, assume that at the beginning a deviation of microarchitectural information is observed the and the finishing module recorded the index of the youngest instruction in the ROB, which is $inst_5$.
After a squashing happens and $inst_4, inst_5$ are squashed, the youngest instruction becomes $inst_3$, then we need to update the stored index to $inst_3$ at this time.
After the update, the finishing logic only need to wait for $inst_3$ to be committed.

Besides, the two out-of-order processors may have different youngest instructions in the ROB when the microarchitectural deviation is observed.
For example, the first processor may issue some instruction a few cycles earlier than the second processor due to the secret value.
If a microarchitectural deviation is observed during this time window, the two processors will have different youngest instructions.
However, this youngest instruction in the first processor still needs to be compared because it may have already affected the microarchitectural observation in the first processor.
Thus, the finishing logic will record indices of both youngest instructions in two out-of-processors.
Only when both youngest instructions are committed and compared can the finishing logic set the $finish$ bit.




\subsection{Handle Superscalar Processors}
In Section~\ref{sec:methodology}, we assume a processor that issues and commits at most one instruction in a cycle.
However, modern superscalar processors may have multiple functional units and thus are able to issue and commit multiple instructions in a cycle.
We will discuss how our baseline scheme and the advanced scheme are both able to handle such cases.

First, we assume that the out-of-order processor can issue two instructions but only commits one instruction at a cycle.
In this scenario, the advanced scheme can still work because no matter how many instructions are issued, the finishing logic will guarantee that all inflight instructions will be compared at commit stage after observing a microarchitectural deviation.
However, the original baseline scheme may fail because the single-cycle machine may not be able to execute instructions as fast as the out-of-order processor, which means when a microarchitectural deviation is observed, the ISA level comparison may have not finished for all inflight instructions in the out-of-order processors.
The solution is to add a finishing logic to the baseline scheme.
Two counters will be added to record the numbers of instructions issued in the two out-of-order processors.
When observing a microarchitectural deviation, the larger counter will be compared with the number of cycles that have elapsed (this represents the number of instructions executed and compared in two single-cycle machines).
If the counter number is larger, then the ISA level comparison needs to continue for extra cycles to reach the counter number.
Meanwhile, the microarchitectural level comparison will be stopped.
After that, a $finish$ bit will be set and the model checking can be finished.

Next, let us consider an out-of-order processor that can issue and commits two instructions in a cycle.
In this case, we can modify the baseline scheme in the same way as above because as long as the ISA level comparison covers all instructions issued in the out-of-order processors, the baseline scheme is correct.
However, the original advanced scheme will fail because the synchronization logic assumes that at most one instruction is committed in both processors.
When the out-of-order processor is able to commit two instructions in a cycle, all the following cases need to be considered:
\begin{enumerate}
    \item Both processors commit two instructions at this cycle.
    \item Both processors commit one instructions at this cycle.
    \item Both processors commit zero instructions at this cycle.
    \item One processor commits two instruction but the other commits one instruction at this cycle.
    \item One processor commits two instructions but the other commits zero instruction at this cycle.
    \item One processor commits one instruction but the other commits zero instruction at this cycle.
\end{enumerate}
Among all these six cases, only 2) 3) 6) are considered in the original synchronization logic.
Thus, the synchronization module needs to be modified to cover all the possible cases, set pause signals when two out-of-order processors commit different numbers of instructions in some cycle, and record the instruction information for later comparison.
All the modifications will be based on existing mechanisms and they only increase the complexity of the shadow logic to cover more cases.

The above two examples have shown that our two schemes can be extended to superscala processors.
For processors that can issue and commit more than two instructions, the way to modify our schemes is similar to the case of two instructions and is not discussed in this paper.


==> ykfkyxzqqtggdstybhwmzfvqmnwcsnwh/Insights.tex <==

\section{Threat Model}

% \mengjia{I did minor text tweak}

Recall from \cref{sec:background:contract}, security properties for secure speculation can be formulated as software-hardware contracts.
Such contracts explicitly state the responsibilities of the software and the hardware sides to achieve an overall non-interference property~\cite{clarkson2010hyperproperties}.
In this paper, we consider the following threat model.


% Recall from \cref{sec:background:contract}, informally, security properties for secure speculation are software-hardware contracts.
% \mengjia{you said contract is formal in the previous paragraph, then you say it is informal here?}
% Such contracts explicitly state the responsibilities of both the software and the hardware sides to achieve an overall non-interference property~\cite{clarkson2010hyperproperties}. 
% The following threat model is considered by software-hardware contracts:
\begin{enumerate}[leftmargin=*]
    \item We assume a system whose data memory is split into two parts: \emph{public} and \emph{secret}. 
    An attacker cannot directly access the secret region.
    % The attacker cannot directly access the secret region.
    The attacker's goal is to infer any secret value through microarchitectural side-channel attacks.
    Non-digital side-channel attacks, such as power side channels~\cite{hertzbleed, poweranalysisattacks}, are out of the scope.
    
    \item The system runs a program that satisfies certain software constraints.
    These constraints prevent the secret from being leaked via ISA state.
    For example, at the ISA level, the program cannot load secret data into registers (in the sandboxing contract), or it needs to follow the constant-time programming discipline.
    % at observation constraints that protect the secret, i.e., the instruction-level observation of certain architectural variables (specified in a contract), such as the \texttt{rd} value of committed instructions, cannot leak any secret.
    % The attacker is able to run any programs satisfying such constraints. \mengjia{attack's constraint is discussed in item 2}

    \item The attacker is able to gain cycle-level observation of certain micro-architectural variables in the system, including the address sequence transmitted on the memory bus and the commit time of instructions.
    
    % \item The program run on the system must satisfy certain software  observation constraints that protect the secret, i.e., the instruction-level observation of certain architectural variables (specified in a contract), such as the \texttt{rd} value of committed instructions, cannot leak any secret.
    % The attacker is able to run any programs satisfying such constraints.
\end{enumerate}


\section{Motivation and Insights}
\label{sec:insight}


In this section, we describe the insights that motivate the design of our verification scheme.
We start by presenting a baseline verification scheme for secure speculation and we analyze the performance bottlenecks encountered.
We then point out the optimization insight that is architecture-friendly and leads us to the design of \name.


% \subsection{Checking Software-Hardware Contracts}

\subsection{The Baseline Verification Scheme}
\label{sec:insight:baseline}


Verifying the software-hardware contract described in Section~\ref{sec:background:contract} requires performing \textit{two} kinds of equivalence checks that involve \textit{four} traces.
The equivalence check at line 2 in \cref{eq:4trace} is the \textit{\swcheck} to determine whether a program $P$ needs to be protected (we say that $P$ is valid).
The equivalence check at line 3 is the \textit{\hwcheck} to determine whether the microarchitecture processor $\mu Arch$ has a correct defense mechanism for the given program.
% \asplosrev{Intuitively we need to reason about four machines (each accounts for a trace) in parallel to verify such a security property as we will show in the baseline scheme below.
% However, our insight later shows that it is possible to only reason about two machines in parallel while still correctly verifying the property, which can greatly reduce the state space and the verification complexity. }
% \mengjia{why we add this sentence? how can this sentence help?} \qt{I just want to give a hint about the evolution from the baseline to our scheme.}\mengjia{I think the hint is too subtle. It is better to be either explicit or not mention it.}

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{images/overview_new.pdf}
    \caption{Overview of \name.}
    \label{fig:overview}
\end{figure}


% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\columnwidth]{images/baseline.pdf}
%     \caption{The baseline verification scheme. Two instances of the single-cycle machine are used for \swcheck and two instances of the out-of-order (OoO) processor are used for \hwcheck.}
%     \label{fig:baseline}
% \end{figure}



The security property (\cref{eq:4trace}) can be tentatively verified using the scheme visualized in \cref{fig:overview}(a).
% \mengjia{TODO: we may change the figure, so the text will also be adjusted...}
First, two copies of a single-cycle machine are instantiated as two separate RTL modules.
The two modules have identical RTL code with the instruction memory and public data memory initialized with the same content ($P$ and $M_{pub}$) and different secret memory ($M_{sec}$), i.e., two secret memories differ in at least one location.
% \footnote{\asplosrev{In practice, the instruction memory and data memory do not necessarily need to be separated as long as the secret location can be clearly specified.}}.
% Note that the scheme includes the instruction memory instead of treating $P$ as input to the system. 
% This is because (i) there could be branch instructions jumping back to old instructions in the program and (ii) all four processors need to run the same program.
The two instances of single-cycle machines execute instructions sequentially, finishing one instruction per cycle.
These two copies execute in a lock-step manner, allowing the verification scheme to derive the $O_{ISA}$ trace at each cycle and compare them for equivalence to enforce the \swcheck.
\cameraready{The comparison results serve as a constraint to filter out invalid programs for the out-of-order processor being verified.
The model checker will discard the programs that generate the traces violating the constraint.}
% \cameraready{As a result, any invalid programs will not be involved in the \hwcheck. 


Similarly, the RTL for the out-of-order processor is duplicated to create two instances, which only differ in the secret memory.
The program memory $P$ and the initial value of the public data memory $M_{pub}$ are the same as in the single-cycle machine. 
The verification scheme compares the microarchitecture execution traces $O_{\mu Arch}$ from the two machines at each cycle for the \hwcheck.

% \asplosrev{In the verification, we assume that \swcheck is never violated and check the assertion that \hwcheck always holds.
% If a trace is found to violate our assertion, it must be a valid attack trace that satisfy \swcheck, otherwise it should have already been discarded due to violation of the assumption.}
% \mengjia{what does this paragraph try to say?}
% \qt{Just to show how will the verification with baseline work. We can remove it if it is already clear enough.}

This scheme runs the \swcheck and \hwcheck in parallel at each cycle, allowing for conducting both bounded and unbounded checking.
% Prior work~\cite{yang2023pensieve} first performs the \swcheck to filter out invalid programs and then performs the \hwcheck, which does not support unbounded checking involving traces of unbounded length.

\begin{comment}
\subsection{Challenges: Reusability and Scalability}

\mengjia{I know I am repeating the intro here... TODO: we can try to make this version shorter by just refer back to the intro.}
\thomas{I think this section is a bit too much repetition + defensive/related work. I think some part of this section should be put in related work}
\mengjia{sounds good. indeed a lot of repetition.}

\mengjiatext{
The baseline verification scheme faces scalability issues.
% Its applicability to RTL verification is limited.
For example, it is unable to produce unbounded proof of software-hardware contracts for in-order processors within 7 days (shown in \cref{sec:eval:compare}), let alone for out-of-order processors.

There are two attempts to address this scalability issue in RTL verification of software-hardware contracts, both requiring formal-method expertise.
UPEC~\cite{fadiheh2020formal} uses an inductive verification approach, assisted with substantial manual invariants, to verify complex out-of-order processors.
Their approach can achieve high scalability, showcased via their proof of a defense scheme on the BOOM processor.
However, the unbounded proof is closely coupled with the defense scheme to be verified.

Specifically, they verified a defense scheme that delays memory instructions until they reach the head of ROB, and their proof is customized towards this defense by stating an invariant that none of the secret data will spread among any gates inside the processor pipeline.
This invariant plays a significantly important role in their unbounded proof.
However, this invariant does not hold for most defenses proposed in the computer architecture community where speculative states do spread in a complex manner inside the processor, considering DoM, STT, and others.
As a result, if using UPEC to verify these defense schemes, the user needs to redo the verification and spend hours figuring out a different set of invariants, which poses significant challenges.

On the other hand, LEAVE attempts to reduce the amount of manual effort in verifying software-hardware contracts of RTL designs by searching for invariants in a set of candidates invariants automatically.
They show their approach works effectively on in-order pipeline processors.
Despite offering a rich idea, their approach is still quite limited in terms of scalability.
We use their approach to verify a toy out-of-order processor in Section~\ref{sec:eval:compare}.
It turns out that their search algorithm cannot find useful invariants, and they end up running into the same issue as UPEC, that is, requiring users to provide manual invariants.

To summarize, the community faces serious challenges in coming up with verification schemes that are both reusable for verifying different defense designs and, meanwhile, scalable enough to be able to verify out-of-order processors.
}
\end{comment}

\subsection{Architecture-driven Insights for Verification}

As discussed in \cref{sec:intro}, the community faces serious challenges in coming up with verification schemes that are both reusable for verifying different defense designs and, meanwhile, scalable enough to be able to verify out-of-order processors.
In this paper, we aim to tackle the research challenge of designing a reusable verification scheme while achieving reasonable scalability, where the verification scheme can handle some out-of-order processors without requiring to come up with custom inductive invariants. 
% The key idea is to augment the by significantly reducing the size of the state machines utilized in verification.
A baseline verification scheme employs four state machines (for the four processors) which entails a non-trivial amount of redundancy among them, we aim to explore the possibility of reducing this redundancy.

As mentioned in Section~\ref{sec:intro}, if an out-of-order processor functionally correctly implements its ISA specification, the ISA trace can be reconstructed from the out-of-order processor's committed instruction sequence.
% \asplosrev{Since functional verification is a separate concern and is a well-studied problem, we do not include it in our scheme.}
% For the rest of the paper, we assume that the out-of-order processor is functionally correct and produces results that match the single-cycle ISA semantics.
% Consequently, the single-cycle machine's execution trace can be reconstructed from the out-of-order processor's committed instruction sequence.
In other words, the single-cycle machine is contained in the out-of-order machine, including the complex instruction decoding, the execution logic, as well as registers/memory state.
This insight leads to our verification scheme, introducing shadow logic to implement the \swcheck directly on the out-of-order processors, as shown in \cref{fig:overview}(b).
With this, we can reduce a four-machine verification problem (the baseline) to a two-machine problem with some additional shadow logic -- this reduction in logic could potentially lead to better scalability.







% \mengjia{so many defensive writing early on...}
% Alternatively, we propose to remove the two single-cycle machines. 
% As mentioned in Section~\ref{sec:intro}, the out-of-order processor needs to be functionally correct for it to be reliably used in checking \cref{eq:4trace}.
% \asplosrev{Since functional verification is a separate concern and is a well-studied problem, we do not include it in our scheme.}
% For the rest of the paper, we assume that the out-of-order processor is functionally correct and produces results that match the single-cycle ISA semantics.
% Consequently, the single-cycle machine's execution trace can be reconstructed from the out-of-order processor's committed instruction sequence.
% In other words, the single-cycle machine is contained in the out-of-order machine, including the complex instruction decoding, the execution logic, as well as registers/memory state.
% This insight leads to our verification scheme, introducing shadow logic to perform \swcheck directly on the out-of-order processors.


==> ykfkyxzqqtggdstybhwmzfvqmnwcsnwh/Insights_old.tex <==

\section{Threat Model}

% \mengjia{I did minor text tweak}

Recall from \cref{sec:background:contract}, security properties for secure speculation can be formulated as software-hardware contracts.
Such contracts explicitly state the responsibilities of the software and the hardware sides to achieve an overall non-interference property~\cite{clarkson2010hyperproperties}.
In this paper, we consider the following threat model.


% Recall from \cref{sec:background:contract}, informally, security properties for secure speculation are software-hardware contracts.
% \mengjia{you said contract is formal in the previous paragraph, then you say it is informal here?}
% Such contracts explicitly state the responsibilities of both the software and the hardware sides to achieve an overall non-interference property~\cite{clarkson2010hyperproperties}. 
% The following threat model is considered by software-hardware contracts:
\begin{enumerate}[leftmargin=*]
    \item We assume a system whose data memory is split into two parts: \emph{public} and \emph{secret}. 
    An attacker cannot directly access the secret region.
    % The attacker cannot directly access the secret region.
    The attacker's goal is to infer any secret value through microarchitectural side-channel attacks.
    Non-digital side-channel attacks, such as power side channels~\cite{hertzbleed, poweranalysisattacks}, are out of the scope.
    
    \item The system runs a program that satisfies certain software constraints.
    These constraints prevent the secret from being leaked via ISA state.
    For example, at the ISA level, the program cannot load secret data into registers (in the sandboxing contract), or it needs to follow the constant-time programming discipline.
    % at observation constraints that protect the secret, i.e., the instruction-level observation of certain architectural variables (specified in a contract), such as the \texttt{rd} value of committed instructions, cannot leak any secret.
    % The attacker is able to run any programs satisfying such constraints. \mengjia{attack's constraint is discussed in item 2}

    \item The attacker is able to gain cycle-level observation of certain micro-architectural variables (specified in a contract) in the system, such as the address sequence transmitted on the memory bus and the commit time of instructions.
    
    % \item The program run on the system must satisfy certain software  observation constraints that protect the secret, i.e., the instruction-level observation of certain architectural variables (specified in a contract), such as the \texttt{rd} value of committed instructions, cannot leak any secret.
    % The attacker is able to run any programs satisfying such constraints.
\end{enumerate}


\section{Motivation and Insights}
\label{sec:insight}

% We propose \name to improve RTL verification for speculative execution vulnerabilities.
In this section, we describe the insights that motivate the design of our verification scheme, \name.
% We start by formally introducing \textbf{security properties}: a family of software-hardware contracts for secure speculation.
{
We start by presenting the threat model considered in this paper.
We then introduce the formal definition of the security properties that we aim to verify, i.e., a family of software-hardware contracts for secure speculation. 
% \mengjia{I did some inline editing}
}
We then present a baseline verification scheme for the security properties and analyze the performance bottlenecks encountered when using this baseline verification scheme.
Finally, we point out the optimization insight that leads us to the design of \name.
% at the end of this section.

% \mengjia{My plan for this section is to 1) explain the sw-hw contract checking procedure; 2) analyze its performance bottleneck; 3) point out an opportunity for optimization}


% \thomas{Should we mention what is not in the threat model? (sometimes people like that as it scopes the work). Here it would be what sometimes people call "no active attackers" (even though it is confusing as the kind of passive attacker we describe, in practice are "active" to make their observation). This might be too confusing}
% \qt{We can say something like 'no analog attack considered.'}
% \mengjia{yes, let's add 1-2 sentences to exclude analog attacks}
% Next, we will formally define the security property that accounts for the above threat model.


\subsection{Checking Software-Hardware Contracts}

% Recall from \cref{sec:background:contract}, informally, security properties for secure speculation are software-hardware contracts.
% Such contracts explicitly state the responsibilities of both the software and the hardware sides to achieve an overall non-interference property~\cite{clarkson2010hyperproperties}. 
% \thomas{I removed the "how they interact": the contract does not mention how they interact, right? simply the responsibilities of both side.}
In the rest of this paper, we name a \emph{security property for secure speculation} (often shortened \emph{security property}) any contract that can be formalized by the following \cref{eq:4trace}:
\begin{equation}    
\begin{aligned}
&\forall P, M_{pub}, M_{sec}, M_{sec}', \\
\text{\textbf{if}}\quad & O_{ISA}(P,M_{pub},M_{sec})=O_{ISA}(P,M_{pub},M_{sec}') \\
\text{\textbf{then}}\quad & O_{\mu Arch}(P, M_{pub},M_{sec}) = O_{\mu Arch}(P, M_{pub},M_{sec}') & 
\end{aligned}
\label{eq:4trace}
\end{equation}
The formula states that when running a program $P$ with public memory $M_{pub}$ and secret memory $M_{sec}$ on a microarchitecture processor $\mu Arch$, if the program $P$ satisfies an indistinguishability software observation constraint, then the actual observation when executed on the hardware remains indistinguishable.
In other words, if the secret was not leaked by the software itself, the formula verifies that the hardware does not leak the secret through microarchitectural side-channel observations. 
\mengjia{can we make the formula one to the background?}
\qt{I'd rather put it here as it is closer to the baseline and our scheme. Readers might want to refer to this formula often when they read those two schemes.}
\mengjia{but it will make our life much easier to say in the background, we can define what uarch is and what ISA constraint is... Also it will be less repetitive...}
\qt{I tried to move it to background, please check.}

The software constraint (line 2 in \cref{eq:4trace}) forces the observations of the program's behavior when executing sequentially (i.e., not speculatively) to be independent of the secret. 
% \thomas{I commented-off a sentence that was confusing me : "the ISA semantics of the processor". }
% Therefore, we denote the software constraint using a function $O_{ISA}$, read as a function to derive the ISA observation trace.
The software constraint uses a function $O_{ISA}$ that computes the ISA observation trace of a program. 
Typically $O_{ISA}$ extracts observations from a simple single-cycle implementation of the ISA \asplosrev{and thus does not involve microarchitectural timing information}. (We use an RTL implementation for practical convenience.)
% \thomas{Small modification $O_{ISA}$ is not itself the software constraint. It is a pair of observations that form the constraint. (Old version kept in comment)}
When the program satisfies the software constraint, line 3 in \cref{eq:4trace} states that the microarchitecture observation traces, computed using $O_{\mu Arch}$, must also be independent of the secret. 
The observations in $O_{ISA}$ will depend on the software-contract. 
The observations in $O_{\mu Arch}$ will depend on the attacker observation model and may include processor state and side channel information such as instruction commit times.

%In \cref{eq:4trace}, all traces include event timing, e.g. the commit time for instructions in the $\mu Arch$ machine, but also the time when each instruction get processed in the ISA machine.
%\mengjia{check. not sure it is the right place. I think the property does not require so, but our baseline scheme does what you describe above.} \sm{Does my sentence above take care of this?}

\mengjia{here we repeat something as in the background. Or maybe a better idea is to merge them?}
\qt{I merged some sentences here to background. If it works, then we can remove the above two paragraphs and the following paragraph.}

Note that \cref{eq:4trace} does not describe a single contract but a large family of contracts.
The equation is parameterized by different observation functions that can formalize various contracts.
For example, in the sandboxing contract, the ISA observation trace consists of the per-cycle content of the register file, which implies the contract assumes the software does not load secrets into registers.
In contrast, in the constant-time programming contract, the ISA observation trace includes both the memory access trace and the program counter trace, as the constant-time programming rule requires those traces to be independent of secrets.

\mengjia{this may be a good opportunity to clarify what exactly we target...}
\qt{Do you mean clarify that we only do two contracts? I think the two scheme are not limited to these two contracts. We are just evaluating using these two contracts.}



\paragraph{Observation}
Verifying a security property requires performing \textit{two} kinds of equivalence checks that involve \textit{four} traces.
%\thomas{Why just 2? TODO double check with everyone}
The equivalence check at line 2 in \cref{eq:4trace} is the \textit{\swcheck} to determine whether a program $P$ needs to be protected (we say that $P$ is valid), and the equivalence check at line 3 is the \textit{\hwcheck} to determine whether the microarchitecture processor $\mu Arch$ has a correct defense mechanism for the given program.
\asplosrev{Intuitively we need to reason about four machines (each accounts for a trace) in parallel to verify such a security property as we will show in the baseline scheme below.
However, our insight later shows that it is possible to only reason about two machines in parallel while still correctly verifying the property, which can greatly reduce the state space and the verification complexity. }
\mengjia{why we add this sentence? how can this sentence help?} \qt{I just want to give a hint about the evolution from the baseline to our scheme.}\mengjia{I think the hint is too subtle. It is better to be either explicit or not mention it.}

% \mengjia{pose condition needs to be agnostic to the source of speculation...}



% Finally, we formally define the speculative-non-interference property related to a contract.
% Given a speculative leakage contract $C$, a program $P$ that executes on a micro-architecture $\mu$ with public memory $M_p$ and secret memory $M_s$, the ISA level observation is $O_{ISA}(C,P,M_p,M_s)$ and the micro-architectural observation is $O_{\mu Arch}(P,M_p,M_s)$, $\mu$ is adhering to $C$ iff.
% \begin{equation}    
% \begin{aligned}
% &\forall P, M_p, M_s, M_s', \\
% & O_{ISA}(C,P,M_p,M_s)=O_{ISA}(C,P,M_p,M_s') \\
% &\rightarrow O_{\mu Arch}(P,M_p,M_s) = O_{\mu Arch}(P,M_p,M_s') & 
% \end{aligned}
% \label{eq:4trace}
% \end{equation}
% This property states that if for a program $P$ the attacker's ISA level observation is the same regardless of the secret ($M_s,M_s'$ are distinct), then the micro-architectural level observation should also be equivalent.
% Otherwise, there is secret information leakage due to speculative execution attacks.

% For the rest of this paper, we will call the $O_{ISA}$ equivalence check in Property~\ref{eq:4trace} Contract Assumption Check, and call the $O_{\mu Arch}$ equivalence check in Property~\ref{eq:4trace} Leakage Assertion Check.



% This scheme can achieve unbounded security proof because we do not set any bounds on the cycles that the model checker should explore, which means any potential attacks that takes any number of cycles can be captured.
% If a counterexample is found, then it must indicate a real attack.
% Because we assume that the out-of-order processor issues at most one instruction in a cycle, the 1-cycle processor always finish the same instruction faster than the out-of-order processor.
% This means whenever there is an deviation between $O_{\mu Arch_1},O_{\mu Arch_2}$, , i.e. a counterexample to Leakage Assertion Check, detected, all the instructions that have been or are being executed by the out-of-order processors have already finished in the 1-cycle processors.
% If any of these instructions violate the ISA level requirement, this trace should have already been filtered out by Contract Assumption Check and the deviation between $O_{\mu Arch_1},O_{\mu Arch_2}$ should not be detected.
% Thus, a counterexample found by our scheme must be caused by a real attack that violates Leakage Assertion Check while still satisfying Contract Assumption Check.



\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{images/baseline.pdf}
    \caption{The baseline verification scheme. Two instances of the single-cycle machine are used for \swcheck and two instances of the out-of-order (OoO) processor are used for \hwcheck.}
    % Both checks are conducted cycle by cycle (marked as $C_1$, $C_2$, $C_3$, ...), which is the same as instruction by instruction for 1-cycle processors (marked as $I_1$, $I_2$, $I_3$, ...).}
    % \mengjia{1. Bold the text for \swcheck and \hwcheck. 2. can we remove C1/C2.. I think the figure is clear without it; 3. add question mark for the cycle-by-cycle equation check} \sm{$C$, and $I$ in the figure are not clear.}
    % \mengjia{use $M_{sec}$ and $M_{pub}$ to match the formula 1}
    % \mengjia{@Qinhan, can you make some minor changes: 1) OOO -> OoO; 2) add a legend for time: an arrow to the right and have text "time" above it}
    \label{fig:baseline}
\end{figure}

% \mengjia{many reviewers do not understand how our shadow logic looks like. How about we show them? it would be better if we show an architecture figure of how the shadow logic being interacted the existing logic, such as ROB etc...}


\subsection{The Baseline Verification Scheme}
\label{sec:insight:baseline}

The security property (\cref{eq:4trace}) can be tentatively verified using the scheme visualized in \cref{fig:baseline}.
First, two copies of a single-cycle machine are instantiated as two separate RTL modules.
The two modules have identical RTL code with the instruction memory and public data memory initialized with the same content ($P$ and $M_{pub}$) and different secret memory ($M_{sec}$) \footnote{\asplosrev{In practice, the instruction memory and data memory do not necessarily need to be separated as long as the secret location can be clearly specified.}}.
% , denoted using different colors.
Note that the scheme includes the instruction memory instead of treating $P$ as input to the system. 
%\sm{Not completely true!} \sm{Single copy of program memory... need to clarify that.}
%\thomas{What does it mean to treat P as input? Was the intended point to say that something along the line off: the 2-4 machines don´t get their response from the instruction memory necessarily at the same time? (from a security persepctive, such a scenario would be seemingly suspicious no?) - need zoom discussion/clarification}
%\mengjia{according to our discussion today, we have that really because that is the memory and we do not want to change the RTL code of the processor, right?}
This is because (i) there could be branch instructions jumping back to old instructions in the program and (ii) all four processors need to run the same program.
% , which cannot be realized without a storage for the program.  \thomas{commenting the "cannot"}
%\sm{And that all processors need to execute the same program.}
%\qt{I add two sentences here to explain why we need instruction memory in the system.}
The two instances of single-cycle machine execute instructions sequentially, finishing one instruction per cycle, which models the ISA semantics of the out-of-order processor being verified.
These two copies execute in a lock-step manner, allowing the verification scheme to derive the $O_{ISA}$ trace at each cycle and compare them for equivalence to perform the \swcheck.

Similarly, the RTL for the out-of-order processor is duplicated to create two instances, which only differ in the secret memory. The program memory $P$ and the initial value of the public data memory $M_{pub}$ is the same as in the single-cycle machine. 
The verification scheme %computes and 
compares the microarchitecture execution traces $O_{\mu Arch}$ from the two machines at each cycle for the \hwcheck.

\asplosrev{In the verification, we assume that \swcheck is never violated and check the assertion that \hwcheck always holds.
If a trace is found to violate our assertion, it must be a valid attack trace that satisfy \swcheck, otherwise it should have already been discarded due to violation of the assumption.}

This scheme runs the \swcheck and \hwcheck in parallel at each cycle, allowing for conducting both bounded and unbounded checking.
Prior work~\cite{yang2023pensieve} first performs the \swcheck to filter out invalid programs and then perform the \hwcheck, which does not support unbounded checking involving traces of unbounded length.

\mengjia{add discussion on how prior work scale }


\subsection{Verification Performance Optimization}

The baseline verification scheme has serious scalability challenges (shown in \cref{sec:eval}).
% \yuheng{Do we have in-order 4-copy result? Check}
Its applicability to RTL verification is limited, as it is even unable to produce unbounded proof of \cref{eq:4trace} for in-order processors within 7 days, let alone for out-of-order processors.
% Its applicability to out-of-order processors is limited, as it is unable to produce unbounded proof of \cref{eq:4trace} within a reasonable timeframe (24 hours).
% \mengjia{I remember they cannot find proof even for in-order processors. I wrote this when I thought they can prove for in-order processors. We can change the text. Maybe remove it.}
% \mengjia{check: is it true? the 4-copy cannot work (including bug-finding) with any out-of-order processors?}
% \qt{4-copy can capture bugs but cannot find any proof}\thomas{The thing is "bug finding" is a tricky one to characterize: there are bugs that are really shallow and easy to find for tools, and there are bugs that are really hard to find. One way might have been to seed a bug ourselves, and show how one method does not find it before timeout, when the other does, but it is not fully convincing neither. (discussion how to navigate this problem)? }
% This limitation raises significant concerns, particularly considering that 
% increasing attention is paid to speculative execution vulnerabilities in out-of-order processors.
%\mengjia{I edit the sentence, because the baseline even cannot prove for in-order processors.}

In this paper, our goal is to tackle the performance issue by significantly reducing the size of the state machines utilized in verification.
Since the baseline verification scheme employs four state machines (for the four processors) and likely entails a non-trivial amount of redundancy among them, we aim to explore the possibility of reducing this redundancy.

One appealing option is to remove the duplicated single-cycle and duplicated out-of-order machines.
However, these duplicated machines were needed to include two different values of the secret in each case ($M_{sec}$ and $M_{sec}'$ in \cref{eq:4trace}), and check for non-interference, i.e., the value of the secret does not impact the observations. 
Prior work~\cite{tiwari2009complete} has proposed to use taint tracking to verify the non-interference property over a single trace. However, this requires a trade-off between precision and the taint-tracking overhead~\cite{hu2011theoretical}. We consider it a promising yet orthogonal research direction (\cref{sec:related}).
\qt{I do think it is unnecessary to mention taint propagation here, because we are just choosing one road to optimize, we do not need to explain why other roads cannot work. I think we can remove the above paragraph and directly present our scheme.}



\mengjia{so many defensive writing early on...}
Alternatively, we propose to remove the two single-cycle machines. 
As mentioned in Section~\ref{sec:intro}, the out-of-order processor needs to be functionally correct for it to be reliably used in checking \cref{eq:4trace}.
\asplosrev{Since functional verification is a separate concern and is a well-studied problem, we do not include it in our scheme.}
For the rest of the paper, we assume that the out-of-order processor is functionally correct and produces results that match the single-cycle ISA semantics.
Consequently, the single-cycle machine's execution trace can be reconstructed from the out-of-order processor's committed instruction sequence.
In other words, the single-cycle machine is contained in the out-of-order machine, including the complex instruction decoding, the execution logic, as well as registers/memory state.
This insight leads to our verification scheme, introducing shadow logic to perform \swcheck directly on the out-of-order processors.
% Note that this technique does not use any knowledge of presumed attack patterns and is general enough to apply to any out-of-order processors without loss of generality.

% \thomas{I moved the paragraph about functional correctness down to discussion}


% {\color{blue}\footnotesize

% \noindent\textbf{sw-hw trace}
% \begin{itemize}
%     \item recall from \cref{sec:background:contract}, software-hardware contract defines how software and hardware coordinate to achieve a security property with regards to speculative execution.
%     \item The different contracts in that section can be formulated as the formula below \cref{eq:4trace}.
%     \item Given a program P, a memory consisting of a public region denoted as Mp and a secret region, denoted as Ms and Ms'. If the program sequentially executes (corresponding to its ISA semantics) generating a trace using the function OISA does not leak secrets, then the hardware needs to ensure the same program executing on an out-of-order processor does not leak secrets via microarchitecture side channels, where all the microarchitecture effects can be summarized in a function Ouarch.
%     \item In formula 1, there exist two "equality check" operations. Heavy...
%     \item The first equality check aims to determine whether the given program satisfies the software constraint.
%     If it does not satisfy the software constraint, for example, if the software program itself has alredy leaked secrets when executing non-speculatively, we require hardware to do nothing.
%     \item If the \swcheck passes, the second equality check becomes relevant, which we refer to as \hwcheck. Examples of hardware traces can be cache access patterns etc.
%     \item In summary, to verify against software-hardware contracts, we will need to perform a \swcheck on a pair of traces generated for the ISA semantics of the out-of-order processor, and a \hwcheck on another pair of traces generated by the out-of-order processors.
% \end{itemize}

% \noindent \textbf{baseline verification scheme}
% \begin{itemize}
%     \item directly translate the security property to the verification scheme as follows
%     \item \cref{fig:method} shows the verification scheme
%     \item two copies of a single-cycle CPU is instantiated (RTL code), both taking the same P (initial state of the instruction memory), and Mp (public memory) but differ in Ms.
%     \item The two copies of single-cycle CPU execute instructions sequentially and execute one instruction per-cycle
%     \item For each cycle, we derive the OISA from the current state of the machine, for example, it could be a function of the register states (the sandboxing context) or the memory sequences (the constant-time context).
%     \item Similarly, we derive the Ouarch from the out-of-order processor, 
%     \item the assertion is written as below:\\
%     \texttt{assume contract\_assumption\_check = True, assert leakage\_assertion\_check = True}
% \end{itemize}

% \noindent \textbf{opportunity}
% \begin{itemize}
%     \item problem: large state machine, in particular, we are aware that the OoO processor is necessary
%     \item reduce the number of copies for each CPU. Challenging: prior work uses taint logic -> cite Tim and Ryan Kaster's work -> heavy (@Sharad, can we comment on more about why it does not work? If too long, may move to related work.)
%     \item the single-cycle CPU can be potentially large... put numbers
%     \item Key observation is that they are encapsulated inside the out-of-order processors
%     \item perform both \swcheck and \hwcheck on the pair of out-of-order processors
% \end{itemize}
% }


==> ykfkyxzqqtggdstybhwmzfvqmnwcsnwh/Introduction.tex <==
%!TEX root = main.tex
\section{Introduction}
\label{sec:intro}


{Speculative execution} in modern out-of-order (OoO) processors has given rise to various speculative execution {attacks}, including Spectre~\cite{Kocher2018spectre}, Meltdown~\cite{Lipp2018meltdown}, L1TF~\cite{website:l1tf_intel}, and LVI~\cite{van2020lvi}. 
These attacks exploit the microarchitectural side effects of transient instructions, i.e., the instructions that are executed speculatively due to misspeculation and squashed later.
Prior work has demonstrated that speculative execution attacks can leak secrets via a wide range of microarchitectural structures, including caches~\cite{Kocher2018spectre, kiriansky2018speculative, koruyeh2018spectre}, TLBs~\cite{gras2018translation}, branch predictors~\cite{chowdhuryy2021leaking} and functional units~\cite{bhattacharyya2019smotherspectre}.

Even worse, as the microarchitecture becomes ever more complex, anticipating
speculative execution {vulnerabilities} seems to pose a Sisyphean challenge. 
For example, Foreshadow~\cite{van2018foreshadow} identified the L1TF vulnerability, showcasing cross-domain leakage of data residing in the L1 cache.
Though the L1TF vulnerability was quickly patched by Intel by flushing L1 data cache upon context switch~\cite{website:l1tf_intel}, such mitigation was insufficient to block small variations of the attack, due to the existence of various other structures inside the L1, including the line fill buffer, the store buffer, the load port, etc.
These structures were exploited to leak information by a batch of follow-on attacks called Microarchitecture Data Sampling Attacks (MDS)~\cite{schwarz2019zombieload, van2019ridl}.
The cat-and-mouse game described above calls for rigorous approaches to ensure %formal and extensive 
the security of processors.





% To this end, this paper aims to develop a formal verification scheme for secure speculation
% on out-of-order processors working at the \textit{Register Transfer Level (RTL)}, as opposed to higher-level abstract models, such as Pensieve~\cite{yang2023pensieve}, CheckMate~\cite{trippel2018checkmate}, and in Guarnieri et al.~\cite{guarnieri2021hardware}.
% Higher-level models are prone to overlooking small but crucial processor structures, like the buffers exploited by the MDS attacks. 
% Given the significance of those details in the security of complex microarchitecture designs, such oversight can result in misleading verification outcomes. 
% \cameraready{In fact, verification on higher-level models and RTL should be used in different design stages.
% The prior one can be used to find bugs at a early design stage while the latter one is needed in a later stage after all micro-architectural details are implemented.}
% \mengjia{I feel the flow in this paragraph changes twice, which feels a bit unnatural. My new attempt below.} \sm{Like Mengjia's para below, lets go with it.}

To this end, this paper aims to develop a formal verification scheme for secure speculation
on out-of-order processors working at the \textit{Register Transfer Level (RTL)}.
% , as opposed to higher-level abstract models, such as Pensieve~\cite{yang2023pensieve}, CheckMate~\cite{trippel2018checkmate}, and in Guarnieri et al.~\cite{guarnieri2021hardware}.
\cameraready{
As hardware design is a lengthy procedure and involves multiple steps, including early-stage high-level modeling and later-stage Register Transfer Level (RTL) implementation, we need verification tools at each stage to offer security guarantees.
Several prior work, such as Pensieve~\cite{yang2023pensieve}, CheckMate~\cite{trippel2018checkmate}, and in Guarnieri et al.~\cite{guarnieri2021hardware}, focus on higher-level abstract models to assist security verification at early design stage.
However, higher-level models are prone to overlooking small but crucial processor structures, like the buffers exploited by the MDS attacks. 
Thus, we aim to design verification tools that can operate at the RTL level at a later design stage when all microarchitectural details are in place.
We envision our tool can work complementarily with existing early-stage verification tools for the whole hardware design flow.
}



% Of course, the undesirable consequence of working at the RTL level is the scalability challenge due to the large design state space. 



% \subsection{Goal: Reusable and Scalable RTL Verification}
\subsection{Blueprint for Systematic and Scalable RTL Security Verification}
% \thomas{Added "systematic" because we had lost the "reusable" part}
% \thomas{What is reusable?Maybe we could say "A blueprint for RTL security verification"}
% \mengjia{I think you roughly get what i want to say... blueprint may work!}


Existing RTL formal verification schemes for secure speculation pose scalability challenges.
Most techniques only work effectively on simple designs such as in-order processors, but struggle to cope with architecturally complex designs like out-of-order processors, leading to timeout.
Making a verification scheme work on an out-of-order processor requires the verification engineer to spend significant manual effort to customize security specifications of subcomponents and try to find invariants that help the unbounded proof to go through. 
This process is very challenging, especially as it requires the engineers to have security expertise and in-depth knowledge of formal methods, computer architecture, and the specifics of the design studied.
% \mengjia{what is security experience ? property?}\thomas{it was typo, security expertise, does it work?}\mengjia{good.}
Moreover, the verification harness that works on one design cannot be easily transferred to another design without requiring new creative insights. 
% \thomas{I think we are also target of that critic}
% \qt{I agree.}
% \thomas{I now understand why we say that here. Because for different defense we can reuse.}
% \mengjia{I think it is not only manual effort, but also intelligence effort. Is there an English for intelligence effort?}
% \thomas{Requiring creative insights?}
% \mengjia{good I like it!}
% Therefore, we end up paying significant and tedious manual verification efforts, again and again for different designs.
% Even worse, often we stuck on verifying new designs.
% \mengjia{now we should say we stuck for different ... TODO: fix English.}

For example, the state-of-the-art verification work UPEC~\cite{fadiheh2020formal} successfully proves a secure speculation scheme on BOOM~\cite{zhaosonicboom}, highlighting a breakthrough along this research direction.\footnote{There are multiple versions of UPEC dealing with different security issues~\cite{schmitz2023upec, deutschmann2023scalable}.
In this paper, unless otherwise stated, we refer to \cite{fadiheh2020formal} which tackles speculative vulnerabilities in RTL implementations.}
However, a careful examination of their scheme shows that the verification methodology
is depending on the specific conservative defense mechanism being verified (which is to prevent speculative load instructions to execute before all preceding branch instructions in the ROB are resolved).
To verify other defenses such as DoM~\cite{sakalis2019efficient} and STT~\cite{yu2019speculative}, a UPEC user will face extensive challenges and need to invest additional effort to extend the set of invariants. 

Alternatively, recent work (LEAVE~\cite{wang2023specification}) proposed to reduce the amount of manual effort needed for RTL verification of secure speculation schemes using automatic invariant search techniques.
Those techniques demonstrated great effectiveness on certain in-order pipelined processors, however we found that the approach tends to have a hard time on simple out-of-order processors (Section~\ref{sec:eval:compare}).
% As their scalability is still limited, they will again need to seek manual invariants for better performance.

% To summarize, the primary research challenge here is to balance scalability to more evolved architectures and amount of manual and non-reusable efforts required to complete the RTL security verification.
To summarize, the primary research challenge here is to improve verification scalability to more evolved architectures and reduce the amount of manual and non-reusable efforts required to complete the RTL security verification.

In this paper, we try to make progress towards reusable and more scalable verification schemes by leveraging computer architecture insights.
Our verification approach gets the computer architects who design the processor involved in the formal verification loop: we are asking them to design the shadow logic machinery instrumental to our verification task, from which we can call the verification tools to formally check the security property.
Compared to writing logical invariants, writing this shadow logic machinery is a task much closer to the standard activity of computer architects.
% which very few prior manage to do so, given the existing gap between the two research communities. 


\subsection{This Paper: Contract Shadow Logic}



% , that can improve the prevalent existing RTL security verification method for secure speculation. 
% It uses computer architecture design insights to improve the scalability of current verification procedures for secure speculation RTL designs.
The security property to be checked in secure speculation is expressed as a software-hardware contract~\cite{guarnieri2021hardware, cauligi2022sok},
% \mengjia{TODO: there is an SOK paper extends it to include more contracts..} \qt{Added.}
which states, ``if a software program satisfies a constraint, then the hardware ensures executing the program will not leak secrets.''
Checking this statement involves two operations.
We refer to the operation that checks the software against a constraint as the \textbf{\swcheck}, and refer to the operation that checks the hardware for detecting {information leakage} as the \textbf{\hwcheck}.
Each of the two checks is performed on a pair of state machines (or machines for short). 
% \mengjia{I try to be more implicit about one-inst}
The \swcheck compares the executions of two simple machines which implement the ISA and execute each instruction in one-cycle (henceforth referred to as {single-cycle machines} or {ISA machines}).
% with identical implementation but different secret input values. 
Similarly the \hwcheck compares the executions of two copies of the out-of-order processor to check for secret leakage.
% leakage of the secret.
The baseline verification scheme examines the \textit{four} state machines cycle by cycle.


% We propose to reduce the security checking time via reducing the overall size of the state machines involved in the check.
We propose a verification scheme, called {\name}.
The key insight is that we can \textit{perform both the \swcheck and the \hwcheck on a single pair of out-of-order machines}, and thus eliminate the pair of single-cycle machines in the verification scheme.
Specifically, assuming the out-of-order processor is correctly implementing the ISA semantics, the single-cycle machine's execution trace can be recovered from the out-of-order processor's \textit{committed} instruction sequences.
We implement this ISA trace extraction mechanism as shadow logic (which is added to assist verification, does not interfere with the original design, and can be safely removed before synthesis).

% As a highlight, different from prior verification work, implementing this shadow logic only requires computer architects' knowledge of the design without needing extra formal-method expertise.
%\thomas{this insight hass been tentatively included earlier}




We have implemented our verification scheme using the commercial RTL verification tool, JasperGold~\cite{website:jaspergold} and use it to verify one in-order processor, three out-of-order processors, and five defense augmentations.
% This marks a milestone in the scalability of security proofs of RTL designs \asplosrev{for secure speculation} \qt{The word `milestone' may sound too strong.}.\mengjia{let's drop this sentene.}
% We also provide a detailed performance evaluation to characterize how our security verification time scales with various factors including instruction scheduling mechanism (i.e., in-order or out-of-order), ISA complexity, defense mechanisms, and microarchitecture structure sizes.
We provide experimental results to compare our scheme with the baseline and two state-of-the-art verification schemes, LEAVE~\cite{wang2023specification} and UPEC~\cite{fadiheh2020formal}.
\cameraready{Through our results, we demonstrate the following:}
First, across all secure designs, the baseline scheme cannot provide any security proofs within 7 days, while, our scheme can prove the security for all of them.
Second, while LEAVE cannot automatically find bugs or prove security for our in-house simplified out-of-order processor, our new scheme is able to do so.
Third, we show the ability of our method to find attacks arising from different mis-speculation sources on the BOOM~\cite{zhaosonicboom} processor, while UPEC can only detect attacks caused by pre-identified mis-speculation sources.
\cameraready{However, we would like to point out that scalability continues to be a challenge in formally verifying secure speculation of hardware designs, and one will need additional architectural insights to assist formal verification to scale to more complex out-of-order processors.}

% \mengjia{TODO: adjust the statement later}



In summary, this paper makes the following contributions:
\begin{enumerate}[leftmargin=*]
    \item We propose a verification scheme, called \name.
    Our scheme leverages computer architecture insights to improve the scalability of RTL security verification for secure speculation while maintaining broad applicability (\cref{sec:insight}).
    \item We identify two important requirements to construct correct shadow logic for checking software-hardware contracts (\cref{sec:main}).
    % \thomas{maybe we could talk about the two requirements as a contribution (those are interesting principles/insights into the design of shadow logic for hw/sw contracts)}\mengjia{good. added.}
    \item We demonstrate the efficacy of our scheme on four processors and conduct a detailed comparison to showcase the advantages of our scheme compared to the baseline and two state-of-the-art verification schemes, i.e., LEAVE and UPEC (\cref{sec:eval}).
   % Our approach can provide security proofs for an in-order processor and a simple out-of-order processor that were not possible with the baseline scheme.
    % \item We compare the performance of our scheme with two state-of-the-art verification schemes (LEAVE and UPEC) and demonstrate its advantage along one or more of the dimensions of scalability and attack-agnostic capability. \mengjia{TODO: adjust this statement later. } 
\end{enumerate}



==> ykfkyxzqqtggdstybhwmzfvqmnwcsnwh/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf \

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> ykfkyxzqqtggdstybhwmzfvqmnwcsnwh/Methodology.tex <==
\section{\name}
\label{sec:main}

% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=\textwidth]{images/method_new.png}%     \caption{Transferring from baseline Scheme to advanced Scheme. (a) shows a baseline verification scheme. (b) shows the intuition to get rid of two ISA machines. (c) shows the shadow logic and mechanisms needed to implement the advanced scheme.}
%     \mengjia{to illustrate the synchronization problem, I hope we can add timeline to showcase the cycle-by-cycle check. see something like Figure 9 (last page) here: https://arxiv.org/pdf/2006.03841.pdf}
%     \label{fig:method}
% \end{figure*}


% We now present our technique: adding \name to improve verification scalability by reducing the number of state machines involved in verification.
% Specifically, we perform the \swcheck directly on the out-of-order processor, reducing a four-machine verification problem (the baseline) to a two-machine problem with some additional shadow logic.
{
In this section, we present the main components of \name. 
We first describe the basic component of our shadow logic that extracts the ISA traces from out-of-order processors.
We then discuss the challenges in making the shadow logic correctly verify software-hardware contracts, and finally provide our solution adressing these challenges.
% Finally, we cover implementation details.
}


\subsection{Shadow Logic to Extract ISA Traces}


An important task of the shadow logic is to monitor the commit stage of the out-of-order processor and extract information for every committed instruction to derive the ISA trace.
The shadow logic needs to be implemented according to the observation function ($O_{ISA}$).
% Depending on what the observation function is, the ISA trace may require extra information than what already exists in the ROB.
For example, if checking for the constant-time contract, the \swcheck needs to compare the addresses of committed memory access instructions and the condition values of committed branch instructions.
Different processor implementations may store this information in different places.
In the best case, the information is already present in the ROB and can be directly obtained.
% The pseudocode for the shadow logic can be as simple as below.
% \mengjia{@Qinhan, is the code below correct? feel free to improve it}

% \mengjia{why the first one is assert and the other is assume?}
% \qt{we can all use assert. I just want to show the reader that there are both assert and assume.}
% \thomas{Hmm, I am not sure that I understand this specific contract/shadow logic.
% (is it the case that this is not meaningful pseudocode?)}
% % \begin{minipage}{\columnwidth}
% % \begin{center}
% % \begin{tabular}{c}
% % \begin{lstlisting}[style=mystyle, language=mylang, label={lst:future}, caption={Example Code for Mircoarchitectural Deviation Caused by Later-Committed Instructions},captionpos=b]
% \begin{lstlisting}[style=mystyle, language=mylang, label={lst:future}]
% assert(cpu1.ROB[head].opcode
%       ==cpu2.ROB[head].opcode);
% case cpu1.ROB[head].opcode:
%   BRANCH: assume(cpu1.ROB[head].cond
%                 ==cpu2.ROB[head].cond);
%   MEM: assume(cpu1.ROB[head].addr
%               ==cpu2.ROB[head].addr);
% \end{lstlisting}
% % \end{tabular}
% % \end{center}
% % \end{minipage}


In more complex cases, the information may be spread across multiple modules, such as inside the register files and load/store queues, and in some cases the information might not even be readily available at commit-time anymore.
{
This is the place where we can leverage and involve the architect's knowledge and expertise.
}
Specifically, to handle these cases, the user needs to extend the existing ROB structure with shadow metadata state to record the information needed to reconstruct the ISA trace.
For example, instead of extracting this information from across modules, we can record the opcode type with the instruction when it enters the ROB and its operand values when it finishes execution.
If the instruction commits later, we can directly obtain the information for the \swcheck.
% Our approach is simple, compatible with almost all observation functions, and easy to implement for out-of-order processors as long as they have ROBs.


Nonetheless, even though the shadow logic needs to be customized for different processor designs, the task of deriving shadow logic to extract ISA traces is straightforward for the processor designers to carry out.
% Notably, the shadow logic required by our scheme can be designed by computer architects who have limited formal-method expertise but 
% are familiar with the design of the processor.
We think this presents an important advantage of our scheme compared to related work, as our scheme can get the designers involved in the verification loop and make the formal tools more accessible to architects.
Moreover, our verification scheme is reusable across different design variations, defenses and contracts, as we only need to swap in different ISA trace extraction logic without requiring to search for new invariants as needed by existing work.
% \thomas{the point about reusability is repeated several times (5.1 and here)}
% }
% \thomas{I think at that point they don't yet know the solution we are proposing, so I fear we are repeating the intro with not enough new knowledge for the reader.}\mengjia{sure. let's think about where to put this paragraph...}
% \qt{I think we can just merge it 5.1. Shrink it into a few sentences and put it as the last paragraph.}
% \thomas{The point that needs to be brought again (because intro was long time ago) is bringing architects in the loop. I thikn usability is ok in 5.1}

Remarkably, there's a scenario where no additional engineering effort is required for tackling different designs. 
Imagine a hardware designer integrating security measures like STT and DoM onto an initially insecure processor.
The shadow logic, initially integrated for the insecure design, seamlessly transfers to the secure design without alteration.
Indeed, all the necessary signals for the shadow logic remain intact within the processor when adding the defense mechanism. 
We use this observation in \cref{sec:eval:defense}, where we assess different defense schemes employing precisely the same shadow logic.

% Excitingly, there exists a case when we do not need to repay any extra engineering efforts for different designs.
% Consider a hardware designer implements a secure defense, such as STT and DoM, upon an insecure processor.
% The shadow logic we put in for the insecure design will be left untouched when ported to the secure design, since with a secure speculation scheme, all the signals needed by the shadow logic are still there in the processor.
% Indeed, in \cref{sec:eval:defense}, we evaluate different defense schemes using the exactly same shadow logic. 

% \mengjia{@Yuheng and @Qinhan, need to make sure the last statement is correct!}
% \qt{I changed a few words now I think it is correct.}

% \asplosrev{Rewriting the shadow logic for a different observation function is also simple because a different observation function only needs to compare different shadow metadata states in ROB.
% For example, to check the sandboxing contract, we need to compare the data value of every committed load instruction between two out-of-order processors.
% When switching to the constant-time contract, the shadow metadata states to be compared are the branch conditions, program counters, multiplication operands and addresses for memory instructions.
% All these shadow metadata can be added to the ROB code in one shot and controlled by macros corresponding to different observation functions.
% To use a specific observation function, we only need to enable its macro and change the shadow metadata states in the comparison expression.
% }



\subsection{Challenges: Two Requirements}
\label{sec:main:twoproperties}

% \mengjia{@Thomas and @Sharad, please check Section 4.1 and Section 4.2}

% \mengjia{shall we re-order the two requirements?}

Enforcing the \swcheck needs comparing two ISA-level traces.
% Intuitively, such traces can be derived from the commit stage of the out-of-order processor.
However, naively introducing shadow logic to extract committed instruction information is insufficient to verify software-hardware contracts since it will violate what we name the \textbf{instruction inclusion requirement} and the \textbf{synchronization requirement}.
% We will first explain these two requirements, and then describe the additional shadow logic it takes to enforce them when the two copies of the single-cycle machine are removed. 



\subsubsection{Instruction Inclusion Requirement}

Recall from \cref{eq:4trace}: the \swcheck and the \hwcheck examine the same program $P$.
This leads to the instruction inclusion requirement: ``\textit{if an instruction's microarchitecture side effects have been considered in the \hwcheck and it will eventually commit, this instruction must also be examined by the \swcheck}.''


The baseline verification scheme assumes the out-of-order processor fetches at most one instruction per cycle and the ISA processor executes one instruction per cycle.
The instruction inclusion requirement is automatically fulfilled as the ISA processor is always running ahead of the out-of-order processor.


% \mengjia{somehow, I feel the text below is verbose... there is some space for improvement. @Thomas @Sharad}
However, when switching to our optimized verification scheme, enforcing the instruction inclusion requirement requires additional work.
Indeed, intuitively, in the out-of-order machines, the \swcheck is checked at commit time, because the \swcheck only examines committed instructions. 
This is a bit behind the \hwcheck, meaning we may miss the instructions that are still in their execution or even the fetch stage. 
Thus, we need to make sure that any violation of the \hwcheck is not related to a failure of \swcheck that has not occurred yet, \cameraready{i.e., the violation of the \hwcheck is not for a program that should have been filtered out by the \swcheck}.




\begin{comment}
For example, consider the scenario below.

\begin{minipage}{\columnwidth}
\begin{center}
\begin{tabular}{c}
% \begin{lstlisting}[style=mystyle, language=mylang, label={lst:future}, caption={Example Code for Mircoarchitectural Deviation Caused by Later-Committed Instructions},captionpos=b]
\begin{lstlisting}[style=mystyle, language=mylang, label={lst:future}]
mul r1, r2, r2  //commit at cycle x
lw r_sec, r3   
lw r4, r_sec    //issue load at cycle x
\end{lstlisting}
\end{tabular}
\end{center}
\end{minipage}

Assume at cycle \texttt{x}, the out-of-order processor commits the multiplication instruction (line 1) and speculatively issues the load instruction using a secret-dependent address (line 3).
The \hwcheck detects the deviation of microarchitecture traces at cycle \texttt{x} due to the speculative secret-dependent load.
The \swcheck performed at the same cycle reports the ISA traces match since it checked the instruction at line 1 (indicating the program under test is valid), and thus the verification claims to have detected an attack counterexample.
However, this is a false counterexample,
because the program is actually invalid, as the load instruction at line 3 will eventually commit and cause ISA trace deviation due to the secret dependency.
The example indicates that \swcheck needs to \textit{look ahead} of the execution of the out-of-order processor, requiring extra shadow logic. 
\end{comment}

\paragraph{Solution}
Our solution to enforce the instruction inclusion requirement is to structure the verification logic into two phases.
In the first phase, we perform the \swcheck and \hwcheck on a pair of out-of-order processors cycle by cycle.
Upon detecting microarchitecture trace deviation, we switch to the second phase, where the \swcheck is applied to all the inflight and bound-to-commit instructions in the pipeline, satisfying the instruction inclusive requirement.

\subsubsection{Synchronization Requirement}

In the baseline verification scheme, for each pair of machines, the two machines in the pair execute in a lock-step manner. 
Hence, the scheme can %simply 
perform both the \swcheck and the \hwcheck by comparing the corresponding states in each pair at \emph{each cycle}.
Because the ISA machine executes exactly one instruction per cycle, the check on ISA traces ($O_{ISA}$) is equivalent to comparing states instruction after instruction.

However, comparing at each cycle the new elements of the ISA traces derived from the two out-of-order processors will not be an equivalent check.
This is because the out-of-order machines might run out of synchronization when the two processors commit their instructions at different time.
Consider the case when the two processors try to commit a load instruction with different addresses, which can happen because of different values of the secret.
One of the processors commits the load in one cycle as the load hits the L1 cache, while the other processor suffers a cache miss and commits the load after the result returns from DRAM, potentially after a hundred cycles.
Because the instruction commits at different cycles, the ISA trace derived from the first processor is no longer cycle-aligned with the ISA trace derived from the second processor.

\paragraph{Solution}
To perform the same check for the \swcheck in the baseline scheme, we first need to \textit{realign} the derived ISA traces.
We achieve this by introducing shadow logic to the second phase of our verification scheme to synchronize the out-of-order processors to commit instructions at the same speed.
% Note that this piece of shadow logic operates in the second phase of our verification logic.


% \begin{figure}[t]
\begin{lstlisting}[style=mystyle, language=mylang, basicstyle=\ttfamily\linespread{0.85}\small, label={fig:contract_code}, caption={Verilog-Style Pseudo-code for Shadow Logic. },captionpos=b] 
cpu cpu1 (.clk(pause1 ? 0: clk), .rst(rst)); 
cpu cpu2 (.clk(pause2 ? 0: clk), .rst(rst));

always @(posedge clk) begin
  // shadow logic to compare traces
  uarch_diff = (O_uarch(cpu1)!=O_uarch(cpu2));
  isa_diff   = (O_ISA(cpu1)  !=O_ISA(cpu2));
  
  // phase-1
  initial uarch_diff_phase1 <= 0;
  if (uarch_diff_phase1==0 && uarch_diff) then
    uarch_diff_phase1 <= 1;
    tail1 <= cpu1.tail;
    tail2 <= cpu2.tail;
  endif
 
  // phase-2
  if uarch_diff_phase1 then
    // Requirement 1: inst inclusion
    drained = (tail1==cpu1.head-1) &&
              (tail2==cpu2.head-1);
    
    // Requirement 2: realign ISA traces
    if (cpu1.commit==cpu2.commit)
        pause1 <= 0;
        pause2 <= 0;
    else if (cpu1.commit)
        pause1 <= 1;
    else if (cpu2.commit)
        pause2 <= 1;
  endif

  // contract assumption check
  assume (isa_diff==0); 
  // leakage assertion check
  assert (!(uarch_diff_phase1 && drained)); 
end
\end{lstlisting} 
% \end{figure}

% \begin{figure}[h]
% \centering
    % \end{tabular}
    % \end{center}
    % \end{minipage}
% \quad \vline
%     \caption{Verilog-Style Pseudo-code for Shadow Logic.}
%     \label{fig:contract_code}
% \end{figure}

\subsection{Solution: Two-Phase Shadow Logic}
\label{sec:main:overview}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\columnwidth]{images/our_scheme.pdf}
%     \caption{Coordinating the execution timeline of two instances of out-of-order processors using shadow logic.}
%     \label{fig:our_scheme}
% \end{figure}

\cref{fig:contract_code} shows the pseudocode of our two-phase shadow logic written in Verilog style.
Given an out-of-order processor to be verified, we create two instances of the processor, named \texttt{cpu1} and \texttt{cpu2} (lines 1-2).
We then introduce shadow logic to drive and monitor the microarchitecture traces and ISA traces of the two instances cycle by cycle (lines 5-7).

    

The remaining shadow logic uses the trace comparison results and operates differently in two phases.
In Phase 1, upon a microarchitecture trace deviation, we record the deviation by setting the variable \texttt{uarch\_diff\_phase1} to true and also record the tail of the ROB of each cpu instance.
The goal of recording the tail is to assist the shadow logic in Phase 2 to determine when the \swcheck is completed to satisfy the instruction inclusion requirement.

In Phase 2, since a microarchitecture trace deviation has already happened, the responsibility of the remaining shadow logic is to ensure the \swcheck is sound, satisfying both the instruction inclusion requirement and the synchronization requirement.
Specifically, the shadow logic tracks whether the two instances have committed the instruction that was recorded at the end of Phase 1 (lines 19-21).
Note that the actual shadow logic implementation also accounts for the case when the recorded tail is squashed due to mis-speculation, which we do not show in \cref{fig:contract_code} for brevity.
Besides, the shadow logic also re-aligns the ISA observation traces whenever the two instances go out of synchronization.
The re-alignment operation is achieved by manipulating the input \texttt{clk} signal to the two cpu instances, involving no code modifications inside the cpu code (see lines 23-30 and how \texttt{pause} is used in lines 1-2).

Note that the re-alignment operation only happens in Phase 2 because the commit signal is included in the $O_{\mu arch}$ trace, which is a common practice in contracts targeting timing side channels.
\cameraready{This example shows a machine (the cpu instance) with one clock domain.
In the case that the machine has multiple clock domains, e.g., using different clocks for the processor and caches, all the clocks need to be paused and resumed simultaneously.}


Finally, we use SVA to explicitly express the \swcheck and \hwcheck in lines 33-36.




\paragraph{Model Checking with \name}
Given the cpu state machines and the shadow logic, model-checking techniques check for all possible input states that satisfy the assumption ($M_{pub}$ and $M_{sec}$) and answer the question whether any of the input states can trigger the assertions.
We expect three possible outcomes:
\begin{itemize}[leftmargin=*]
    \item[1)] the model checker finds a counterexample, which reassembles an attack code that satisfies the software constraints but will introduce distinguishable microarchitecture traces running on the cpu;
    \item[2)] the model checker declares a successful unbounded proof to indicate the processor under verification does satisfy the software-hardware contract for unbounded number of cycles;
    \item[3)] the model check hits a scalability bottleneck and cannot produce a result within a reasonable amount of time, which we refer to as ``time out.''
\end{itemize}


\paragraph{\rev{Validity} of the Synchronization Operation}
% \yuheng{@Mengjia}
% \mengjia{the previous paragraph title reads as a claim, so I changed it. Does it make sense to you?}\sm{I like this.}
% \mengjia{missing links}
As discussed in \cref{sec:background:shadow}, shadow logic should only passively monitor operations and never modify the design under verification.
However, the shadow logic we introduce does have a limited influence on the design when the ``\texttt{pause}'' signal freezes the clock. 
Strictly speaking, this logic is no longer just monitoring the design.
\rev{
We claim our shadow logic is still valid for two reasons.
First, the shadow logic performs the ``\texttt{pause}'' operation in Phase 2.
At the beginning of Phase 2, the timing-dependent microarchitectural traces deviation has already been detected, thus Phase 2 only focuses on comparing traces of committed instructions, i.e. ISA traces, which only involve the execution results of committed instructions and does not include any microarchitectural timing information.
Second, the ``\texttt{pause}'' signal only freezes the clock signal of the processor and thus does not affect the execution results of committed instructions.
Thus, it will not influence the ISA traces, nor will it affect the ISA trace comparison results.
}



% \paragraph{Phase 1}
% The shadow logic monitors the ISA traces and microarchitecture traces of the two out-of-order processors and performs the two cycle-by-cycle equivalence checks.
% The shadow logic for \hwcheck is identical to what already exists in the baseline scheme.
% Depending on the contract, we define the observation function for the traces, e.g., the addresses of the memory requests issued by the core.
% To perform the \swcheck, we augment the commit stage of the processor with shadow logic to record in shadow state information corresponding to every committed instruction.
% \rev{In the first phase, the verification is searching all reachable states for states that can lead to a deviation between the two ISA traces or the two microarchitecture traces.}

% This first phase has three possible outcomes:
% \rev{
% (1) the verification finds that for all reachable states, no deviation is detected on the ISA traces or the microarchitecture traces;
% }
% (2) the ISA traces deviate and (3) the microarchitecture traces deviate while the ISA traces do not.
% In case (1) and (2), the security property holds since no secret is leaked via speculative execution.
% In case (3), we still need to examine whether the inflight instructions pass the \swcheck or not, requiring Phase 2 for this case.

% \paragraph{Phase 2}
% \rev{
% If the verification in Phase-1 finds reachable states that can cause a deviation of microarchitecture traces, it continues with Phase-2 to focus on \swcheck of the ISA traces to determine whether the program is valid.
% }


% To tackle the synchronization requirement discussed in \cref{sec:main:twoproperties}, we need to synchronize the two processors for each instruction they commit to align the extracted ISA traces.
% We synchronize the two machines by introducing a ``\texttt{pause}'' signal to each instance.
% The \texttt{pause} signal freezes the input clock signal of the state machine, pausing any state changes during the pause. We pause the one copy that commits in some cycle while the other does not, and let it continue after the other copy commits.
% The pausing shadow logic introduced is simple and agnostic to the processor's implementation.
% \rev{
% Note that our Phase-2 check only involves \swcheck on the ISA traces, which do not include any timing information.
% Therefore, the ``\texttt{pause}'' signal will not interfere with our check results.}

% To preserve the instruction inclusion requirement, the shadow logic needs to include all the inflight and bound-to-commit instructions in the \swcheck.
% \cref{fig:our_scheme} has an illustrative example to show how the shadow logic coordinates the execution of two processor instances that commit maximally one instruction per cycle.
% At \texttt{t3}, we detect a deviation of the microarchitecture traces, and the shadow logic switches to focus on \swcheck on ISA traces to determine whether the program is valid.
% The goal is to include all the instructions already in the pipeline at the deviation timepoint (\texttt{t3}) in the \swcheck.
% Therefore, we let the two processors progress and use the synchronization logic to align their ISA traces.


% This then raises the question: when 
% to \textit{terminate} the \swcheck?
% {
% Since we only want to include the inflight instructions at the deviation time point, one option is to continue to check the assumption for an upper-bound of the number of cycles it takes to fully drain the ROB.
% However, this upper-bound can be very large (consider the worst case where each instruction in the ROB has a long latency and depends on the previous instruction), which will introduce many redundant checks and make it unpractical even for finding simple attacks.
% }

% Alternatively, we choose to record a small amount of information in shadow state 
% to help determine the end of the ISA trace.
% Specifically, we record the tail of the ROB entry at the deviation point (\texttt{t3} in \cref{fig:our_scheme}).
% We consider \swcheck to be complete when the marked tails in both instances reach the head of ROB.
% In the case when a marked tail is squashed (i.e., it cannot reach the head of ROB), we update the marked tail to the youngest unsquashed entry based on the squash signal. 


% \subsection{Implementation Details}
% \label{sec:detail}

% \mengjia{TODO: we will make this part very concise and short...}

% Our \name is widely applicable and allows the verification of different security properties, depending on the observation functions chosen. It also supports superscalar machines, a common architectural optimization present in many out-of-order processors.
% In this section, we elaborate on details necessary to support both of these aspects.



\paragraph{Supporting Superscalar Processors}
% The baseline scheme supports verifying superscalar processors that fetch more than one instruction per cycle as long as the corresponding single-cycle ISA machine's completion speed can match the out-of-order processor, e.g., by computing instructions two by two. 
The pseudocode in \cref{fig:contract_code} assumes the processor commits maximally one instruction at a cycle.
Our scheme can be adapted for superscalar processors, where multiple instructions can be committed at each cycle.
The problem that we need to tackle is that the pausing granularity is determined by how many instructions the processor commits.
We will need to add shadow logic to break the atomicity of \swcheck by supporting partial ISA trace comparison at each cycle and the capability to remember unaligned traces for future comparison.
This approach introduces minimal shadow state overhead as the number of entries for memorizing unmatched ISA traces only needs to match the commit bandwidth of the processor. 
It is constant regardless of the ISA trace length.
However, the complexity of the logic increases with the commit bandwidth because we need to align traces across neighboring cycles.

% Our optimized scheme needs special support for superscalar processors.
% As shown in \cref{fig:our_scheme}, the synchronization shadow logic works well with processors that commit at most one instruction per cycle.
% As they commit 0 or 1 instruction at each cycle, our pause signal can align the ISA traces with single-instruction granularity.



% However, this scheme needs to be adapted for superscalar processors, where multiple instructions can be committed at each cycle.
% The problem is that the pausing granularity is determined by how many instructions each instance of processor commits, and it can likely be more than one.
% To better understand the problem, 
% Consider the example in \cref{fig:sync}, where the out-of-order processors can commit two instructions per cycle.
% At \texttt{t1}, the first instance commits \texttt{Ix}.
% At \texttt{t2}, the second instance commits two instructions \texttt{Ix} and \texttt{Iy}.
% At \texttt{t3}, the first instance commits \texttt{Iy} and \texttt{Iz}.
% If we continue in this way, no matter how the pause operation is performed, we will never be able to fully align the ISA traces at any cycle.

% We address the above issue by regaining single-instruction granularity with minimal shadow logic overhead.
% We break the atomicity of \swcheck by supporting partial ISA trace comparison at each cycle and the capability to remember unaligned traces for future comparison.
% \cref{fig:sync} shows how our scheme works.
% At \texttt{t1}, we inject pause (\circled{1}) to the first processor instance since it runs ahead of the other instance.
% At \texttt{t2}, since the ISA traces for both instances are non-empty, we can perform \swcheck to compare the head of the two traces until we exhaust one of the traces (\circled{2}).
% For the other trace that still has dangling items, we record those items in our shadow logic and forward them to the next cycle.
% In \cref{fig:sync}, the ROB entry for \texttt{Iy} will be recorded at \texttt{t2} (\circled{3}).
% The recorded instruction will be appended to the head of the ISA trace for the next cycle (\circled{4}) and used in the \swcheck (\circled{5}).

% The above approach introduces minimal shadow state overhead as the number of entries for memorizing unmatched ISA traces only needs to match the commit bandwidth of the processor. 
% It is constant regardless of the ISA trace length.
% However, the complexity of the logic to perform \swcheck increases with the commit bandwidth because we need to align traces across neighboring cycles.

\cameraready{
\subsection{Discussion}

\paragraph{Verification Gap.}
Our verification scheme reformulates the contract property in Equation~\ref{eq:4trace} and can potentially introduce a verification gap.
Our proof is conditioned upon the ISA traces stated as the hypothesis in Equation~\ref{eq:4trace} matching the ISA traces extracted from the out-of-order processors, which in turn requires the following assumptions to be satisfied:
1) the shadow logic is assumed to be implemented correctly;
2) the out-of-order processor is assumed to be functionally correct.

First, the definition of the correctness of our shadow logic includes the shadow logic selecting the right signals to extract the ISA trace and the microarchitectural trace, and the shadow logic generating the pause signal at the proper time.
As such, we ensure the derived ISA trace from the out-of-order processor contains the writeback data of each corresponding instruction.


Second, the functional correctness assumption ensures that the commit stage generates the correct ISA instructions and writeback data as the ISA specification.
Together with the shadow logic correctness assumption, we ensure the derived ISA traces in our scheme are equivalent to the ISA hypothesis in the contract property.

}
% \color{gray}{
% \sm{gray text to be dropped?}
% In our scheme, when the model checker provides an unbounded proof, it does not prove the exact same contract defined in Equation \ref{eq:4trace}.
% More specifically, the ISA observation used in our proof is extracted from the out-of-order machine instead of the ISA machine specified in Equation \ref{eq:4trace}.
% We will show how this gap can be filled with \textbf{two assumptions: the shadow logic being correctly implemented and the functional correctness of the out-of-order machine}.

% The first assumption is easier to understand: the shadow logic should be correctly implemented according to our description in \cref{sec:main:overview}.
% This could be enforced through manual examination of the designers.
% For example, when the ISA observation includes the writeback data of each instruction, the designers should pick the correct signal containing the writeback data in the out-of-order machine.
% The designers should also correctly enforce the instruction inclusion requirement and
% the synchronization requirement by pausing the out-of-order machine correctly in Phase 2.

% Even if shadow logic is implemented correctly, there is still one step away from exactly verifying  Equation \ref{eq:4trace}.
% The question left is whether, for example, the writeback signal in the out-of-order machine contains the same value as the writeback signal in the ISA machine.
% This could be enforced by the functional correctness of the out-of-order machine.
% More generally, functional correctness enforces that the signals extracted from the out-of-order machine contain the same value as those extracted from the ISA machine.
% We rely on the existing functional verification process to give us the assumption of functional correctness.
% }



% \mengjia{I reused most text from rebuttal below..}
\cameraready{
\paragraph{Decoupling of security and functional verification.}
Our verification approach leverages the decoupling (i.e., separation) of functional verification and security verification.
Specifically, our approach for verifying a security property generates a verification task that does not embody a proof obligation related to the functional correctness of the out-of-order processor.
Instead, as stated above, we assume the machine has been independently verified to be functionally correct.
Our choice is justified because verification engineers spend significant effort on functional verification, and our approach leverages this and avoids having to redo this effort as a sub-task of security verification, which may explain the significant verification performance improvement obtained with our approach.
Similar decoupling approaches are also used in inductive approaches on verifying contract properties such as LEAVE~\cite{wang2023specification}.
}


% {\color{gray}{
% \paragraph{Decoupling of security and functional verification.}
% \sm{gray text to be dropped.}
% The discussion above also gives us another aspect to understand the benefit of contract shadow logic.
% By making functional correctness a separate assumption, our scheme manages to remove the burden of functional verification from the security verification.
% This decoupling is a high-level explanation of the performance improvement of our scheme.
% Similar decoupling approaches are also used in inductive approaches on verifying contract properties such as LEAVE~\cite{wang2023specification}.
% }




==> ykfkyxzqqtggdstybhwmzfvqmnwcsnwh/RelatedWork.tex <==
\section{Related Work}
\label{sec:related}






% We discuss related work in the order of their proximity to our research.
% \rev{
% \cref{table:compare_scheme} shows the comparison between different hardware verification schemes.
% The first batch, Iodine~\cite{gleissenthall2019iodine}, Xenon~\cite{v2021solver}, and Knox~\cite{athalye2022verifying}, verifies whether a hardware module or in-order processor can take a same amount of time for different inputs.\yuheng{Add UPEC-DIT here?}
% This property is not related to speculative execution vulnerabilities.
% The second batch of work, including CheckMate~\cite{trippel2018checkmate}, Guarnieri et al.~\cite{guarnieri2021hardware}, and Pensieve~\cite{yang2023pensieve}, applies their verification methodologies to abstract hardware models, sacrificing the model precision provided by RTL.
% % \mengjia{we may want to reorder the text in the related work section to match the table.}

Among all related works, UPEC~\cite{fadiheh2020formal} and LEAVE~\cite{wang2023specification} are the closest to us, as they both target speculative execution vulnerabilities and work on RTL.
We have provided detailed comparisons of our scheme, UPEC, and LEAVE in \cref{sec:eval:compare}.
We now discuss other related work.
We identify that previous approaches differ along three axes: 1) verification target, 2) security properties, and 3) checking techniques.
% Compared with them, the table shows that our scheme is the \textit{first} to successfully conduct formal verification of speculation contracts on RTL implementation of out-of-order processors without pre-assuming any attack pattern or using any manual invariants.

% \mengjia{I cut some text and refer to S6.4 for detail.}

% Although the out-of-order processor we try is relatively small and our scheme times-out when proving out-of-order processors with practical size, moving from in-order to out-of-order is already a significant step.
% To bridge the same gap, previous works either sacrificed the model precision provided by RTL, were limited to bounded checks, assumed specific attack patterns, or used manual invariants to speed up the verification.
% \thomas{It is often not just "or" but "and" right?}
% \qt{I think "or" is not exclusive, "either ... or" is exclusive. Maybe we can just remove that "either".}
% Our scheme does not have any of the above limitations.
% \yuheng{Do we want to cut some of the above description of UPEC and LEAVE, also?}
% }
% \subsection{Security Verification Schemes}

% \mengjia{I would like to put a structure in discussing related work.
% 1. We first focus on RTL verification techniques: UPEC and LEAVE (do we have other work or not?) ; Prior work attempts to convert 4-copy to 2-copy, but have the following limitations compared to \name.
% 2. We then talk about other techniques that focus on high-level models; using fuzzing or other attack synthesis techniques (CheckMate); 
% 3. Finally maybe 1-2 sentence about software verification techniques..}\yuheng{USNIEX caraline work}\yuheng{Radu's fuzzing TEExec...}

% \mengjia{@Qinhan, shall we talk about IODINE,.... the sequence of work targeting RTL verification for constant time, but do not check against sw-hw contract?}


% \mengjia{We dropped all the gray text for UPEC and LEAVE...}
% {\color{gray}
% \paragraph{RTL Verification of the Software-Hardware Contract}
% % \yuhengtext{
% UPEC~\cite{fadiheh2020formal} and LEAVE~\cite{wang2023specification} have almost the same verification goal as our work.
% As discussed in \cref{sec:eval:comparison-with-state-of-the-art}, their key difference from us is that they use inductive proofs with manual effort that customized to specific processors or even specific attack patterns.
% In contrast, our shadow logic is designed to be automatic and attack-agnostic and can be applied to different processors through a standard workflow.
% \yuheng{I tried to briefly summarize and pointing to the \cref{sec:eval:comparison-with-state-of-the-art}.}
% % }
% % \thomas{Commented quite a bit here as it seems it was doing the same thing as the new paragraph}
% % Both UPEC~\cite{fadiheh2020formal} and LEAVE~\cite{wang2023specification} share a similar goal as our work to verify RTL designs for secure speculation.
% % At a high level, they also attempt to convert the four-machine verification problem to a two-machine problem.
% % However, they significantly differ from our work in terms of the applicability of their technique.
% % We begin with two RTL verification schemes against speculative execution attacks that can both achieve full coverage (unbounded proof).

% UPEC~\cite{fadiheh2020formal} and LEAVE~\cite{wang2023specification} have almost the same verification goal as our work and also use two copies of the out-of-order processor for the verification, though they make use of invariants rather than shadow logic.
% % However, they do not design shadow logic as we do, but rather use the inductive proof technique.

% % \thomas{the following commented is alreayd in the table}
% % UPEC~\cite{fadiheh2020formal} is a technique to provide unbounded formal proofs for secure speculation mechanisms at RTL level.
% The highlight of UPEC~\cite{fadiheh2020formal} is the demonstration of a proof for a defense mechanism implemented on the open-source BOOM processor~\cite{asanovic2015berkeley}.
% % at the RTL level.
% % Thus, it is the closest to the goals of this paper.
% %\textbf{UPEC}~\cite{fadiheh2020formal} does unbounded formal checks against speculative execution attacks for out-of-order processors at the RTL level.
% % It is able to both capture attacks and prove security under the sandboxing contract, and can scale to large out-of-order processors such as BOOM~\cite{asanovic2015berkeley}.
% %UPEC applies two copies of the out-of-order processor, but starts the verification from an arbitrary state instead of reset state and conducts the proof inductively.
% %Multiple constraints are used to rule out illegal initial states.
% %For example, it assumes that there must be a mis-predicted branch instruction in the ROB at the initial state.
% %In the ROB, the instructions older than branch will be committed while instructions younger than it will be squashed later.
% %To enforce the software constraint of sandboxing, UPEC assumes that any load instruction in the ROB targeting at the secret must be younger than the branch.
% %It initialized two copies of the out-of-order processor to a same initial state except the secret, and check the variables influenced by the secret (the same variable having different values in two copies) after $k$ cycles.
% %$k$ starts from 1 and is incremented by 1 after every check.
% %If it is found that after $k$ cycles, some variable observable to the attacker (such as commit time) is influenced by the secret, then this indicates an attack.
% %On the other hand, if after $k+1$ cycles the secret has not influenced any observable variables and UPEC finds that the secret does not influence more variables compared with the result from $k$ cycles, it will try to prove that the secret will not influence any more variables, thus finishing the security proof.
% However, UPEC is a highly customized technique that has limited applicability.
% First, UPEC only supports the sandboxing contract, while our \name can support multiple software-hardware contracts with sequential execution mode.
% Second, UPEC gains verification performance by leveraging prior knowledge of attack patterns \rev{and encodes them as invariants to be used by the model checker}, which can miss the detection of attacks exploiting unknown speculation sources.
% In contrast, our technique is attack-agnostic.
% Finally, UPEC customizes a proof technique that relies on secret data not speculatively propagating to any microarchitectural state.
% This technique only works for very conservative defenses under a specific contract, i.e., $\mathsf{Delay_{futuristic}}$ under the sandboxing contract, and unlike our work, the technique does not work for other defenses.


% % However, UPEC is not attack-agnostic as it has to assume the speculation source, such as a mispredicted branch instruction in the ROB.
% % Thus, if an attack exploits some unkown speculation source, UPEC is unable to capture it.
% % The usage of prior attack knowledge helps UPEC reduce the total number of states to be explored and greatly improves its performance.
% % % Further, UPEC considers only the sandboxing contract and provides a security proof for a simple defense that prevents issuing any speculative load instructions.
% % % For the sandboxing contract, the secret can never be loaded from memory to any location, which leads to a fast %inductive 
% % % proof in UPEC since the secret \smtext{does not influence processor state}.
% % % It is unclear whether\smtext{/how} UPEC can be adapted to other contracts such as constant-time.
% % %or have as good performance as it achieves for sandboxing.
% % In comparison with UPEC, our \name is attack-agnostic and is applicable to more complex defenses under multiple contracts. 
% % The broader applicability of our technique requires the proof to explore all reachable states which makes it hard to handle processors as large as BOOM.


% LEAVE~\cite{wang2023specification} proposes an inductive approach to prove that RTL designs guarantee different software-hardware contracts. 
% The focus of the algorithm is on finding inductive invariants either automatically or manually, which can help the proof go through. 
% If it cannot find enough inductive invariants, the proof will not go through even if the design is secure.
% % The paper provides limited information about how their shadow logic is implemented, and thus we are unable to provide a concrete comparison.
% However, their practical evaluation only includes in-order processors, such as Sodor 2-stage. 
% Note that inductive invariants for out-of-order processors are more complex, so it is unclear whether LEAVE could find enough invariants to prove security.
% In contrast, our scheme does not require invariants and proves security for both in-order and out-of-order processors.
% }




% we demonstrate multiple applications on out-of-order processors using our \name. \sm{Not clear what you mean by "applications" here.}
% \mengjia{How about "we provide multiple demonstrations of proving security properties on out-of-order processors using \name."} \sm{Yes, this is fine, please go ahead.}
% As a side note, the paper proposed an algorithm to find inductive invariants which serve as lemmas to help proof go through.
% We consider this technique can be used in complementary with our \name. \sm{Do we need the last two sentences?} 
%\qt{It's not clear whether their technique can be combined with ours, but this is an interesting direction.}
%\sm{One point Qinhan made was that LEAVE cannot detect bugs, because when they can't find a proof, it may be because it couldn't find the invariants, or the design was buggy. LEAVE has no way to distinguish between the two. That was the point the original text was making, and that is why the discussion on LEAVE was focused on the invariants.}
%\qt{Maybe we can still mention this point, but not to criticize them, just saying the goal is a bit different from ours.}

%\mengjia{======}
%The software constraint in LEAVE to satisfy \textit{Synchronization Property} and \textit{Instruction Inclusion Property} is realized not through two single-cycle processors, but through the generation of inductive invariants.\mengjia{they also do shadow logic right? why invariant?}
%\mengjia{======}
%\qt{The property to check is $assumption\rightarrow assertion$.
%We build up shadow logic so we can directly check this property.
%What LEAVE does is first try to find as many inductive $invariants$ such that $assumption \rightarrow invariants$ holds, then check if $invariants \rightarrow assertion$ holds.
%In other words, it tries to derive sufficient conditions for $assertion$ from $assumption$.
%The first step is starting with a large set of user-provided invariants and gradually removing invalid ones from it.
%So the invariant learning process is very important in their algorithm, and if finally they fail to prove, the reason might be they do not get enough invariants from the first step.
%I think the key difference is not about using shadow logic or not, it is about the invariants.
%}

% without using knowledge of existing attack patterns.
% The focus of the algorithm is on finding inductive invariants \smtext{which serve as lemmas} to help the proof go through. \smtext{These inductive invariants are constraints on the system states and are automatically generated.}
%At the beginning of the algorithm, a large set of invariants is generated automatically.
%Then, LEAVE iteratively removes those invalid invariants from the set and make sure the remaining invariants are real inductive invariants while satisfying the software constraint of the contract.
%Finally, it checks if this set of invariants are enough to prove the assertion (no leakage on hardware).
% The software constraint in LEAVE to satisfy \textit{Synchronization Property} and \textit{Instruction Inclusion Property} is realized not through two single-cycle processors, but through the generation of inductive invariants.
% %but by adding more constraints during the invariants learning process.
% %Note that our scheme guarantees these two properties by adding shadow logic.
% When the LEAVE algorithm terminates without a proof, it may be due to its inability to find \smtext{inductive} invariants and does not necessarily indicate a real attack.
% \smtext{Thus, it is set up to find proofs rather than attacks. In contrast, UPEC, Pensieve and \name will provide counter-examples which are traces capturing the attack.}
% %which is one of the common application of formal verification schemes. 
% In their practical evaluation, LEAVE demonstrates success with in-order processors such as Sodor 2-stage, but do not present any results for out-of-order processors. 
% \mengjia{I think too much discussion on the proof part, which I consider is orthogonal to our work (more sounds like we are targeting different directions). I really do not think that having a slightly different goal is a limitation of LEAVE.
% Rather, I would like to emphasize two points here: 1) the paper provides no detail on the design of the shadow logic, disallow us to provide a concrete comparison; 
% and 2) adding shadow logic for obtaining ISA traces from out-of-order processors can be much more complex than from in-order processors (according to our practical experience), as we need to handle synchronization granularity issues on superscalar processors}
% Thus, it is unclear if the technique can scale to out-of-order processors because the \smtext{inductive} invariants to prove security of out-of-order processors can be much more complex \smtext{and harder to find} than the in-order processor case.

%By contrast, our \name is able to both find attacks and prove security.
%We experiment with both out-of-order processors and in-order processors, the result of which is a good demonstration of the praticability of our scheme. 

%It can generate full proofs and scale to complex RTL designs. 
%However, its goal is to only prove adherence to contracts and cannot capture violations, thus its algorithm is a proof-searching one rather than an attack-searching one.
%This means it can only help prove the security of a processor but cannot help find attacks because not finding a proof does not mean there exists an attack, it may also be caused by the algorithm setup.

% [reader should be able to understand these easily at this point. We should prepare reader for this with prior sections. Otherwise, directly tell people we are better is too defensive and trigger complaints. Architects is not super familiar with UPEC.]

% [compare with those fuzzing RTL evaluation.]

% [by reading our paper, we should make it easy for other to understand other papers. Because we define a framework to put other papers into category, classify them.]

% Their proof is from arbitrary state and based on induction.
% Explain why they are able to find proof for large CPUs.
% However, this requires prior-knowledge of the attack, and thus cannot find unknown attacks.
% Besides, although they show that they can prove security for large designs, they are not proving for any complex defense mechanism.

% Besides, they only consider one specific contract.

% Their synchronization idea is similar to ours, but they only propose a high-level idea and try on in-order CPUs.
% This is much more complex on out-of-order CPUs.
% Try to find more differences

\paragraph{Targets for Verification of Secure Speculation}
There is a lot of work leveraging formal methods to verify secure speculation properties (variants of software-hardware contracts), but their targets differ from our work, either focusing on abstract processor models or software.

Pensieve~\cite{yang2023pensieve}, Guarnieri et al.~\cite{guarnieri2021hardware}, and CheckMate~\cite{trippel2018checkmate} target abstract processor models (not RTL).
% \paragraph{Verification for Secure Speculation Using Abstract Hardware Models}
Specifically, Pensieve~\cite{yang2023pensieve} does bounded model checking to detect speculative execution vulnerabilities on modular models connected using hand-shaking interfaces.
% It can capture attacks within a bounded number of cycles for abstract models (not RTL), but cannot provide unbounded security checks.
Guarnieri et al.~\cite{guarnieri2021hardware} uses a paper proof to reason about an abstract out-of-order processor model expressed as operational semantics.
CheckMate~\cite{trippel2018checkmate} applies security litmus tests on abstract processor models expressed as $\mu$hb graphs to synthesize exploit patterns, so as to find new attacks through these patterns. 
% This group of works all target abstract processor models.
Although verifying abstract processor models can give designers key insights, this approach unavoidably neglects RTL implementation details, which may cause speculative execution attacks.


On the software side, there are efforts to guarantee that a program does not contain gadgets that can be exploited by different speculative execution attacks~\cite{cauligi2020constant,cheang2019formal,mosier2022axiomatic,wang2019oo7,wu2019abstract,mosier2023serberus}.
For example, Serberus~\cite{mosier2023serberus} detects code patterns, at compile time, in cryptographic primitives that can be exploited by broad ranges of speculative execution attacks.
% \mengjia{todo: spell some of the work out. Also, include caroline's recent SP paper in case she is on the PC.}
This line of work usually assumes a specific hardware model, and then verifies that specific pieces of software satisfy the software constraint component in software-hardware contracts.
The goal is very different from our work, where we verify the hardware's RTL implementation.

\paragraph{Security Properties}
There exist RTL security verification works that target security properties \textit{not} related to speculative execution.
These works target various data-oblivious properties.
For example, Clepsydra~\cite{ardeshiricham2017clepsydra} verifies hardware modules, such as ALUs and Caches, take the same amount of time when executing on different input data.
IODINE~\cite{gleissenthall2019iodine}, Xenon~\cite{v2021solver}, UPEC-DIT~\cite{deutschmann2023scalable} check whether each instruction's execution time is independent of its operands for in-order/out-of-order processors.
% \mengjia{Put Qinhan's CCS paper here..}
Knox~\cite{athalye2022verifying} builds a framework to verify that when a specific program is running on a physically-isolated Hardware Security Module (HSM), its execution time does not leak extra information beyond the functional specification of the program.

\paragraph{Checking Techniques}
% \mengjia{put secVerilog and specVerilog work here...}
% There are also efforts on verifying hardware for partial %(almost fully) 
% coverage of speculative execution attacks through formal verification and testing techniques.
% Pensieve~\cite{yang2023pensieve} does bounded model checking to detect speculative execution vulnerabilities.
% It can capture attacks within a bounded number of cycles for abstract models (not RTL), but cannot provide unbounded security checks.
% \rev{Guarnieri et al.~\cite{guarnieri2021hardware} uses a paper proof to reason about an abstract out-of-order processor model.}
% CheckMate~\cite{trippel2018checkmate} applies security litmus tests on abstract processor models to synthesize exploit patterns, so as to find new attacks through these patterns. 
% \rev{Although verifying abstract processor models can give designers key insights, this approach unavoidably neglects RTL implementation details which may cause speculative execution attacks.}
In addition to leveraging formal-method techniques, fuzzing-based schemes~\cite{ghaniyoun2021introspectre,moghimi2020medusa,xiao2019speechminer,weber2021osiris,oleksenko2022revizor,oleksenko2023hide,hur2022specdoctor}, such as SpecDoctor~\cite{hur2022specdoctor}, check RTL or blackbox hardware for speculative execution vulnerabilities by generating and testing random attack patterns.
Although the above works cannot guarantee full coverage of speculative execution attacks, they can be faster at detecting security bugs when evaluating large designs.

% \newline

\paragraph{Verification of Clean-slate Designs}
Finally, an exciting yet orthogonal line of work focuses on security verification of clean-slate designs.
SecVerilog~\cite{zhang2015hardware} enables hardware programmers to enforce security policies while developing the hardware.
A violation of the security policy would be detected at compile time.
SpecVerilog~\cite{zagieboylo2023specverilog} further extends this ability to support specifying speculation-related policies.
\cite{tan2023security} formally verifies that a low-trust architecture with a specialized ISA and hardware is free of timing side-channel leakage.
% Their designalso uses semantics of hardware signals to specify timing information leakage as information flow properties~\cite{tan2023security} because a secret-dependent execution time can be reflected as information flow from the secret to certain control signals.}


% \paragraph{RTL Security Verification for Data-oblivious Hardware}
% \mengjia{I am happy with the related work up until now, because I do not fully understand what the work below...}
% \yuhengtext{
% % Researchers have also proposed verification schemes against the timing side channels that are not only introduced by speculative execution.
% Clepsydra~\cite{ardeshiricham2017clepsydra} defines a data-obliviousness property for hardware, stating that hardware should take a same amount of time when executing on different input data, and verifies this property for hardware modules such as ALUs and Caches.
% IODINE~\cite{gleissenthall2019iodine}, Xenon~\cite{v2021solver}, and UPEC-DIT~\cite{deutschmann2023scalable} further extend the verification to in-order and out-of-order processors.
% % However, all of these schemes allow processors to execute arbitrary program and cannot provide precise security assessment for processors that is designed to be secure only under well-written program (i.e., program that passes our contract assumption check).
% These schemes evaluate processors while executing arbitrary programs, while our scheme evaluates processors while executing programs that pass the contract assumption check as we are only targeting at speculative vulnerabilities.
% Knox~\cite{athalye2022verifying} builds a framework to verify when a specific program is running on a hardware, its execution time does not leak extra information beyond the functional specification of the program.
% \yuheng{Knox is a slightly different property, allowing timing depend on public data (i.e., data included in the interface specification of the program)}
% }



